CEFHRI: A Communication Efficient Federated Learning Framework for Recognizing Industrial Human-Robot Interaction

Human-robot interaction (HRI) is a rapidly growing field that encompasses social and industrial applications. Machine learning plays a vital role in industrial HRI by enhancing the adaptability and autonomy of robots in complex environments. However, data privacy is a crucial concern in the interaction between humans and robots, as companies need to protect sensitive data while machine learning algorithms require access to large datasets. Federated Learning (FL) offers a solution by enabling the distributed training of models without sharing raw data. Despite extensive research on Federated learning (FL) for tasks such as natural language processing (NLP) and image classification, the question of how to use FL for HRI remains an open research problem. The traditional FL approach involves transmitting large neural network parameter matrices between the server and clients, which can lead to high communication costs and often becomes a bottleneck in FL. This paper proposes a communication-efficient FL framework for human-robot interaction (CEFHRI) to address the challenges of data heterogeneity and communication costs. The framework leverages pre-trained models and introduces a trainable spatiotemporal adapter for video understanding tasks in HRI. Experimental results on three human-robot interaction benchmark datasets: HRI30, InHARD, and COIN demonstrate the superiority of CEFHRI over full fine-tuning in terms of communication costs. The proposed methodology provides a secure and efficient approach to HRI federated learning, particularly in industrial environments with data privacy concerns and limited communication bandwidth. Our code is available at https://github.com/umarkhalidAI/CEFHRI-Efficient-Federated-Learning.

==> fig/representative.tex <==
 \begin{figure}[t!]
\centering
    \hfill
    \begin{subfigure}[h]{0.45\columnwidth}
		\centering
		  \framebox[\linewidth]{\raisebox{0}[0.5\linewidth][0]{{\small CareAvatars.}}}
	\end{subfigure}
	\hfill
	\begin{subfigure}[h]{0.45\columnwidth}
		\centering
		 \includegraphics[width=\linewidth]{fig/matterport.png}
	\end{subfigure}
	\hfill 
	\\
	\vspace{0.25cm}
	\begin{subfigure}[h]{\columnwidth}
		\centering
		  \includegraphics[width=0.99\linewidth]{fig/teaser.png}
	\end{subfigure}
    % \vspace{-0.25cm}
    \caption{We propose \textbf{RCareWorld}, a \textit{high-fidelity} human-centered simulation world for robotic caregiving.}
    \label{fig:teaser}
    \vspace{-0.8cm}
\end{figure}

==> fig/system_overview.tex <==
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.95\linewidth]{fig/rcareworld_system_overview_new.pdf}
\end{center}
\vspace{-2mm}
\centering
*\scriptsize{\textbf{P}hysX, \textbf{B}ullet, \textbf{O}bi, \textbf{F}lex, \textbf{C}loth \textbf{D}ynamics, \textbf{Z}ibra Liquids, and \textbf{S}OFA}
\vspace{-1mm}
\caption{System overview of RCareWorld.
% : It uses Unity as server for visual rendering and physics simulation, and provides Python, ROS, and VR interfaces. With CareAvatars for human modeling, and CareHomes for assistive environment modeling, RCareWorld provides realistic human modeling and environment modeling. 
}
\label{fig:components}
\vspace{-8mm}
\end{figure}

==> references.tex <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})

@inproceedings{feichtenhofer2020x3d,
  title={X3d: Expanding architectures for efficient video recognition},
  author={Feichtenhofer, Christoph},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={203--213},
  year={2020}
}
@article{tam2022parameter,
  title={Parameter-Efficient Prompt Tuning Makes Generalized and Calibrated Neural Text Retrievers},
  author={Tam, Weng Lam and Liu, Xiao and Ji, Kaixuan and Xue, Lilong and Zhang, Xingjian and Dong, Yuxiao and Liu, Jiahua and Hu, Maodi and Tang, Jie},
  journal={arXiv preprint arXiv:2207.07087},
  year={2022}
}
@inproceedings{mcmahan2017communication,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial intelligence and statistics},
  pages={1273--1282},
  year={2017},
  organization={PMLR}
}
@article{pan2022st,
  title={ST-Adapter: Parameter-Efficient Image-to-Video Transfer Learning for Action Recognition},
  author={Pan, Junting and Lin, Ziyi and Zhu, Xiatian and Shao, Jing and Li, Hongsheng},
  journal={arXiv preprint arXiv:2206.13559},
  year={2022}
}

@inproceedings{wei2022masked,
  title={Masked feature prediction for self-supervised visual pre-training},
  author={Wei, Chen and Fan, Haoqi and Xie, Saining and Wu, Chao-Yuan and Yuille, Alan and Feichtenhofer, Christoph},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14668--14678},
  year={2022}
}
@inproceedings{bertasius2021space,
  title={Is space-time attention all you need for video understanding?},
  author={Bertasius, Gedas and Wang, Heng and Torresani, Lorenzo},
  booktitle={ICML},
  volume={2},
  number={3},
  pages={4},
  year={2021}
}
@inproceedings{thoker2022severe,
  title={How Severe is Benchmark-Sensitivity in Video Self-Supervised Learning?},
  author={Thoker, Fida Mohammad and Doughty, Hazel and Bagad, Piyush and Snoek, Cees GM},
  booktitle={European Conference on Computer Vision},
  pages={632--652},
  year={2022},
  organization={Springer}
}
@inproceedings{shao2020finegym,
  title={Finegym: A hierarchical video dataset for fine-grained action understanding},
  author={Shao, Dian and Zhao, Yue and Dai, Bo and Lin, Dahua},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2616--2625},
  year={2020}
}

@article{yang2023aim,
  title={Aim: Adapting image models for efficient video action recognition},
  author={Yang, Taojiannan and Zhu, Yi and Xie, Yusheng and Zhang, Aston and Chen, Chen and Li, Mu},
  journal={arXiv preprint arXiv:2302.03024},
  year={2023}
}
@inproceedings{jia2022visual,
  title={Visual prompt tuning},
  author={Jia, Menglin and Tang, Luming and Chen, Bor-Chun and Cardie, Claire and Belongie, Serge and Hariharan, Bharath and Lim, Ser-Nam},
  booktitle={European Conference on Computer Vision},
  pages={709--727},
  year={2022},
  organization={Springer}
}
@article{ajoudani2018progress,
  title={Progress and prospects of the human--robot collaboration},
  author={Ajoudani, Arash and Zanchettin, Andrea Maria and Ivaldi, Serena and Albu-Sch{\"a}ffer, Alin and Kosuge, Kazuhiro and Khatib, Oussama},
  journal={Autonomous Robots},
  volume={42},
  pages={957--975},
  year={2018},
  publisher={Springer}
}
@inproceedings{roitberg2014human,
  title={Human activity recognition in the context of industrial human-robot interaction},
  author={Roitberg, Alina and Perzylo, Alexander and Somani, Nikhil and Giuliani, Manuel and Rickert, Markus and Knoll, Alois},
  booktitle={Signal and Information Processing Association Annual Summit and Conference (APSIPA), 2014 Asia-Pacific},
  pages={1--10},
  year={2014},
  organization={IEEE}
}
@article{GAMBOAMONTERO2023118510,
title = {Asynchronous federated learning system for human–robot touch interaction},
journal = {Expert Systems with Applications},
volume = {211},
pages = {118510},
year = {2023},
issn = {0957-4174},
doi = {https://doi.org/10.1016/j.eswa.2022.118510},
url = {https://www.sciencedirect.com/science/article/pii/S0957417422015901},
author = {Juan Jose Gamboa-Montero and Fernando Alonso-Martin and Sara Marques-Villarroya and Joao Sequeira and Miguel A. Salichs},
keywords = {Machine learning applications, Federated learning, Human–robot interaction, Social robots, Acoustic sensing, Touch recognition},
abstract = {Artificial intelligence and robotics are advancing at an incredible pace; however, there is a risk associated with the data privacy and personal information of users interacting with these systems and platforms. In this context, the federated learning approach emerged to enable large-scale, distributed learning without the need to transmit or store any information necessary to train the learning models. In a previous paper, we presented a system capable of detecting, locating, and classifying what kind of contact occurs between humans and one of our robots using innovative contact microphone technology. In this work we go further, improving the previously presented touch system with a multi-user, multi-robot, distributed, and scalable learning approach that is able to learn in a collaborative and incremental way while respecting the privacy of the user’s information. The system has been successfully evaluated in a real environment with 28 different users divided in 7 different groups. To assess the performance of our system with this federated learning approach, we compared it to the same distributed learning system without federated learning. That is, the control group for this comparison is a central node directly receiving all the training examples obtained by each robot locally. We found that in this context the inclusion of federated learning improves the results concerning traditional distributed learning.}
}
@article{hentout2019human,
  title={Human--robot interaction in industrial collaborative robotics: a literature review of the decade 2008--2017},
  author={Hentout, Abdelfetah and Aouache, Mustapha and Maoudj, Abderraouf and Akli, Isma},
  journal={Advanced Robotics},
  volume={33},
  number={15-16},
  pages={764--799},
  year={2019},
  publisher={Taylor \& Francis}
}
@inproceedings{mendieta2022local,
  title={Local learning matters: Rethinking data heterogeneity in federated learning},
  author={Mendieta, Matias and Yang, Taojiannan and Wang, Pu and Lee, Minwoo and Ding, Zhengming and Chen, Chen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8397--8406},
  year={2022}
}
@INPROCEEDINGS{9857233,
  author={Karim, Nazmul and Khalid, Umar and Esmaeili, Ashkan and Rahnavard, Nazanin},
  booktitle={2022 IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (CVPRW)}, 
  title={CNLL: A Semi-supervised Approach For Continual Noisy Label Learning}, 
  year={2022},
  volume={},
  number={},
  pages={3877-3887},
  doi={10.1109/CVPRW56347.2022.00433}}
@INPROCEEDINGS{6725318,
  author={Zareen, Muhammad Sharjeel and Akhlaq, Monis and Tariq, Muhammad and Khalid, Umar},
  booktitle={2013 2nd National Conference on Information Assurance (NCIA)}, 
  title={Cyber security challenges and wayforward for developing countries}, 
  year={2013},
  volume={},
  number={},
  pages={7-14},
  doi={10.1109/NCIA.2013.6725318}}
@inproceedings{choudhury2019utility,
  title={On the utility of model learning in hri},
  author={Choudhury, Rohan and Swamy, Gokul and Hadfield-Menell, Dylan and Dragan, Anca D},
  booktitle={2019 14th ACM/IEEE International Conference on Human-Robot Interaction (HRI)},
  pages={317--325},
  year={2019},
  organization={IEEE}
}
@ARTICLE{9433648,
  author={De Cristofaro, Emiliano},
  journal={IEEE Security & Privacy}, 
  title={A Critical Overview of Privacy in Machine Learning}, 
  year={2021},
  volume={19},
  number={4},
  pages={19-27},
  doi={10.1109/MSEC.2021.3076443}}
@INPROCEEDINGS{9983628,
  author={Su, Xiaowen and Yuan, Fengpei and Zhang, Ran and Liu, Jian and Boltz, Marie and Zhao, Xiaopeng},
  booktitle={2022 IEEE/ACM Conference on Connected Health: Applications, Systems and Engineering Technologies (CHASE)}, 
  title={Deploying a Human Robot Interaction Model for Dementia Care in Federated Learning}, 
  year={2022},
  volume={},
  number={},
  pages={184-185},
  doi={}}
@inproceedings{Bitfit-2022,
  author    = {Elad Ben Zaken and
               Yoav Goldberg and
               Shauli Ravfogel},
  title     = {BitFit: Simple Parameter-efficient Fine-tuning for Transformer-based
               Masked Language-models},
  booktitle = {Proceedings of the 60th Annual Meeting of the Association for Computational
               Linguistics (Volume 2: Short Papers), {ACL} 2022, Dublin, Ireland,
               May 22-27, 2022},
  pages     = {1--9},
  publisher = {Association for Computational Linguistics},
  year      = {2022},
}
@inproceedings{ioffe2015batch,
  title={Batch normalization: Accelerating deep network training by reducing internal covariate shift},
  author={Ioffe, Sergey and Szegedy, Christian},
  booktitle={International conference on machine learning},
  pages={448--456},
  year={2015},
  organization={PMLR}
}
@article{wu2022communication,
  title={Communication-efficient federated learning via knowledge distillation},
  author={Wu, Chuhan and Wu, Fangzhao and Lyu, Lingjuan and Huang, Yongfeng and Xie, Xing},
  journal={Nature communications},
  volume={13},
  number={1},
  pages={1--8},
  year={2022},
  publisher={Nature Publishing Group}
}
@article{qu2021feddq,
  title={FedDQ: Communication-Efficient Federated Learning with Descending Quantization},
  author={Qu, Linping and Song, Shenghui and Tsui, Chi-Ying},
  journal={arXiv preprint arXiv:2110.02291},
  year={2021}
}
@article{aji2017sparse,
  title={Sparse communication for distributed gradient descent},
  author={Aji, Alham Fikri and Heafield, Kenneth},
  journal={arXiv preprint arXiv:1704.05021},
  year={2017}
}
@inproceedings{prompt2021,
  author    = {Brian Lester and
               Rami Al{-}Rfou and
               Noah Constant},
  title     = {The Power of Scale for Parameter-Efficient Prompt Tuning},
  booktitle = {Proceedings of the 2021 Conference on Empirical Methods in Natural
               Language Processing, {EMNLP} 2021, Virtual Event / Punta Cana, Dominican
               Republic, 7-11 November, 2021},
  pages     = {3045--3059},
  publisher = {Association for Computational Linguistics},
  year      = {2021},
}



@inproceedings{li-liang-2021-prefix,
    title = "Prefix-Tuning: Optimizing Continuous Prompts for Generation",
    author = "Li, Xiang Lisa  and
      Liang, Percy",
    booktitle = "Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
}
@INPROCEEDINGS{9981793,
  author={Kumar, Aakash and Kini, Jyoti and Mian, Ajmal and Shah, Mubarak},
  booktitle={2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}, 
  title={Self Supervised Learning for Multiple Object Tracking in 3D Point Clouds}, 
  year={2022},
  volume={},
  number={},
  pages={3754-3761},
  doi={10.1109/IROS47612.2022.9981793}}

@misc{kumar2021pcdan,
      title={PC-DAN: Point Cloud based Deep Affinity Network for 3D Multi-Object Tracking (Accepted as an extended abstract in JRDB-ACT Workshop at CVPR21)}, 
      author={Aakash Kumar and Jyoti Kini and Mubarak Shah and Ajmal Mian},
      year={2021},
      eprint={2106.07552},
      archivePrefix={https://arxiv.org/abs/2106.07552},
      primaryClass={cs.CV}
}
@inproceedings{Adaptive-Federated-Optimization-2021,
  author    = {Sashank J. Reddi and
               Zachary Charles and
               Manzil Zaheer and
               Zachary Garrett and
               Keith Rush and
               Jakub Kone{\v{c}}n{\'y} and
               Sanjiv Kumar and
               Hugh Brendan McMahan},
  title     = {Adaptive Federated Optimization},
  booktitle = {9th International Conference on Learning Representations, {ICLR} 2021, Virtual Event, Austria, May 3-7, 2021},
  year      = {2021},
}


@article{Transfer-Learning-for-NLP-2019,
  author    = {Neil Houlsby and
               Andrei Giurgiu and
               Stanislaw Jastrzebski and
               Bruna Morrone and
               Quentin de Laroussilhe and
               Andrea Gesmundo and
               Mona Attariyan and
               Sylvain Gelly},
  title     = {Parameter-Efficient Transfer Learning for {NLP}},
  journal   = {Proceedings of the 36th International Conference on Machine},
  volume    = {abs/1902.00751},
  year      = {2019},
}
@article{xiao2023offsite,
  title={Offsite-Tuning: Transfer Learning without Full Model},
  author={Xiao, Guangxuan and Lin, Ji and Han, Song},
  journal={arXiv preprint arXiv:2302.04870},
  year={2023}
}
@misc{Fedprog-2021,
  author = {Wang, Hui-Po and Stich, Sebastian U. and He, Yang and Fritz, Mario},
  title = {ProgFed: Effective, Communication, and Computation Efficient Federated Learning by Progressive Training},
    booktitle={Proceedings of the 39 th International Conference on Machine
Learning, Baltimore, Maryland, USA},
  year = {2021},
}


@inproceedings{mendieta2022local,
  title={Local learning matters: Rethinking data heterogeneity in federated learning},
  author={Mendieta, Matias and Yang, Taojiannan and Wang, Pu and Lee, Minwoo and Ding, Zhengming and Chen, Chen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8397--8406},
  year={2022}
}





@inproceedings{goyal2017something,
  title={The" something something" video database for learning and evaluating visual common sense},
  author={Goyal, Raghav and Ebrahimi Kahou, Samira and Michalski, Vincent and Materzynska, Joanna and Westphal, Susanne and Kim, Heuna and Haenel, Valentin and Fruend, Ingo and Yianilos, Peter and Mueller-Freitag, Moritz and others},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5842--5850},
  year={2017}
}
@article{li2021survey,
  title={A survey on federated learning systems: vision, hype and reality for data privacy and protection},
  author={Li, Qinbin and Wen, Zeyi and Wu, Zhaomin and Hu, Sixu and Wang, Naibo and Li, Yuan and Liu, Xu and He, Bingsheng},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2021},
  publisher={IEEE}
}
@inproceedings{rehman2022federated,
  title={Federated Self-supervised Learning for Video Understanding},
  author={Rehman, Yasar Abbas Ur and Gao, Yan and Shen, Jiajun and de Gusm{\~a}o, Pedro Porto Buarque and Lane, Nicholas},
  booktitle={European Conference on Computer Vision},
  pages={506--522},
  year={2022},
  organization={Springer}
}
@inproceedings{zhao2017spatio,
  title={Spatio-temporal autoencoder for video anomaly detection},
  author={Zhao, Yiru and Deng, Bing and Shen, Chen and Liu, Yao and Lu, Hongtao and Hua, Xian-Sheng},
  booktitle={Proceedings of the 25th ACM international conference on Multimedia},
  pages={1933--1941},
  year={2017}
}
@article{xiang2008video,
  title={Video behavior profiling for anomaly detection},
  author={Xiang, Tao and Gong, Shaogang},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={30},
  number={5},
  pages={893--908},
  year={2008},
  publisher={IEEE}
}
@article{nayak2021comprehensive,
  title={A comprehensive review on deep learning-based methods for video anomaly detection},
  author={Nayak, Rashmiranjan and Pati, Umesh Chandra and Das, Santos Kumar},
  journal={Image and Vision Computing},
  volume={106},
  pages={104078},
  year={2021},
  publisher={Elsevier}
}
@article{van2008visualizing,
  title={Visualizing data using t-SNE.},
  author={Van der Maaten, Laurens and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={11},
  year={2008}
}
@article{zaken2021bitfit,
  title={Bitfit: Simple parameter-efficient fine-tuning for transformer-based masked language-models},
  author={Zaken, Elad Ben and Ravfogel, Shauli and Goldberg, Yoav},
  journal={arXiv preprint arXiv:2106.10199},
  year={2021}
}
@article{chen2022adaptformer,
  title={AdaptFormer: Adapting Vision Transformers for Scalable Visual Recognition},
  author={Chen, Shoufa and Ge, Chongjian and Tong, Zhan and Wang, Jiangliu and Song, Yibing and Wang, Jue and Luo, Ping},
  journal={arXiv preprint arXiv:2205.13535},
  year={2022}
}
@inproceedings{sultani2018real,
  title={Real-world anomaly detection in surveillance videos},
  author={Sultani, Waqas and Chen, Chen and Shah, Mubarak},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={6479--6488},
  year={2018}
}

@inproceedings{zhang_shufflenet_2017,
  title={Shufflenet v2: Practical guidelines for efficient cnn architecture design},
  author={Ma, Ningning and Zhang, Xiangyu and Zheng, Hai-Tao and Sun, Jian},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={116--131},
  year={2018}
}
@article{dai2022toyota,
  title={Toyota smarthome untrimmed: Real-world untrimmed videos for activity detection},
  author={Dai, Rui and Das, Srijan and Sharma, Saurav and Minciullo, Luca and Garattoni, Lorenzo and Bremond, Francois and Francesca, Gianpiero},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2022},
  publisher={IEEE}
}






@article{soomro2012ucf101,
  title={UCF101: A dataset of 101 human actions classes from videos in the wild},
  author={Soomro, Khurram and Zamir, Amir Roshan and Shah, Mubarak},
  journal={arXiv preprint arXiv:1212.0402},
  year={2012}
}
@inproceedings{kuehne2011hmdb,
  title={HMDB: a large video database for human motion recognition},
  author={Kuehne, Hildegard and Jhuang, Hueihan and Garrote, Est{\'\i}baliz and Poggio, Tomaso and Serre, Thomas},
  booktitle={2011 International conference on computer vision},
  pages={2556--2563},
  year={2011},
  organization={IEEE}
}
@article{imagenet15russakovsky,
    Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
    Title = { {ImageNet Large Scale Visual Recognition Challenge} },
    Year = {2015},
    journal   = {International Journal of Computer Vision (IJCV)},
    doi = {10.1007/s11263-015-0816-y},
    volume={115},
    number={3},
    pages={211-252}
}
@incollection{NEURIPS2019_9015,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf}
}
@article{tong2022videomae,
  title={Videomae: Masked autoencoders are data-efficient learners for self-supervised video pre-training},
  author={Tong, Zhan and Song, Yibing and Wang, Jue and Wang, Limin},
  journal={arXiv preprint arXiv:2203.12602},
  year={2022}
}
@inproceedings{he2015delving,
  title={Delving deep into rectifiers: Surpassing human-level performance on imagenet classification},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1026--1034},
  year={2015}
}
@article{kay2017kinetics,
  title={The kinetics human action video dataset},
  author={Kay, Will and Carreira, Joao and Simonyan, Karen and Zhang, Brian and Hillier, Chloe and Vijayanarasimhan, Sudheendra and Viola, Fabio and Green, Tim and Back, Trevor and Natsev, Paul and others},
  journal={arXiv preprint arXiv:1705.06950},
  year={2017}
}

@article{wang2020tackling,
  title={Tackling the objective inconsistency problem in heterogeneous federated optimization},
  author={Wang, Jianyu and Liu, Qinghua and Liang, Hao and Joshi, Gauri and Poor, H Vincent},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={7611--7623},
  year={2020}
}

@article{acar2021federated,
  title={Federated learning based on dynamic regularization},
  author={Acar, Durmus Alp Emre and Zhao, Yue and Navarro, Ramon Matas and Mattina, Matthew and Whatmough, Paul N and Saligrama, Venkatesh},
  journal={arXiv preprint arXiv:2111.04263},
  year={2021}
}





@misc{fed-video-2022,
  author = {Rehman, Yasar Abbas Ur and Gao, Yan and Shen, Jiajun and de Gusmao, Pedro Porto Buarque and Lane, Nicholas},
  title = {Federated Self-supervised Learning for Video Understanding}
  ,publisher =  {10.48550/ARXIV.2207.01975},
  year = {2022},
}





@misc{shen_partial_2021,
	title = {Partial {Is} {Better} {Than} {All}: {Revisiting} {Fine}-tuning {Strategy} for {Few}-shot {Learning}},
	shorttitle = {Partial {Is} {Better} {Than} {All}},
	url = {http://arxiv.org/abs/2102.03983},
	abstract = {The goal of few-shot learning is to learn a classifier that can recognize unseen classes from limited support data with labels. A common practice for this task is to train a model on the base set first and then transfer to novel classes through fine-tuning (Here fine-tuning procedure is defined as transferring knowledge from base to novel data, i.e. learning to transfer in few-shot scenario.) or meta-learning. However, as the base classes have no overlap to the novel set, simply transferring whole knowledge from base data is not an optimal solution since some knowledge in the base model may be biased or even harmful to the novel class. In this paper, we propose to transfer partial knowledge by freezing or fine-tuning particular layer(s) in the base model. Specifically, layers will be imposed different learning rates if they are chosen to be fine-tuned, to control the extent of preserved transferability. To determine which layers to be recast and what values of learning rates for them, we introduce an evolutionary search based method that is efficient to simultaneously locate the target layers and determine their individual learning rates. We conduct extensive experiments on CUB and mini-ImageNet to demonstrate the effectiveness of our proposed method. It achieves the state-of-the-art performance on both meta-learning and non-meta based frameworks. Furthermore, we extend our method to the conventional pre-training + fine-tuning paradigm and obtain consistent improvement.},
	urldate = {2022-09-27},
	publisher = {arXiv},
	author = {Shen, Zhiqiang and Liu, Zechun and Qin, Jie and Savvides, Marios and Cheng, Kwang-Ting},
	month = feb,
	year = {2021},
	note = {arXiv:2102.03983 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@misc{suresh_distributed_2017,
	title = {Distributed {Mean} {Estimation} with {Limited} {Communication}},
	url = {http://arxiv.org/abs/1611.00429},
	doi = {10.48550/arXiv.1611.00429},
	abstract = {Motivated by the need for distributed learning and optimization algorithms with low communication cost, we study communication efficient algorithms for distributed mean estimation. Unlike previous works, we make no probabilistic assumptions on the data. We first show that for \$d\$ dimensional data with \$n\$ clients, a naive stochastic binary rounding approach yields a mean squared error (MSE) of \${\textbackslash}Theta(d/n)\$ and uses a constant number of bits per dimension per client. We then extend this naive algorithm in two ways: we show that applying a structured random rotation before quantization reduces the error to \${\textbackslash}mathcal\{O\}(({\textbackslash}log d)/n)\$ and a better coding strategy further reduces the error to \${\textbackslash}mathcal\{O\}(1/n)\$ and uses a constant number of bits per dimension per client. We also show that the latter coding strategy is optimal up to a constant in the minimax sense i.e., it achieves the best MSE for a given communication cost. We finally demonstrate the practicality of our algorithms by applying them to distributed Lloyd's algorithm for k-means and power iteration for PCA.},
	urldate = {2022-09-26},
	publisher = {arXiv},
	author = {Suresh, Ananda Theertha and Yu, Felix X. and Kumar, Sanjiv and McMahan, H. Brendan},
	month = sep,
	year = {2017},
	note = {arXiv:1611.00429 [cs]},
	keywords = {Computer Science - Machine Learning},
}

@misc{konecny_federated_2017,
	title = {Federated {Learning}: {Strategies} for {Improving} {Communication} {Efficiency}},
	shorttitle = {Federated {Learning}},
	url = {http://arxiv.org/abs/1610.05492},
	doi = {10.48550/arXiv.1610.05492},
	abstract = {Federated Learning is a machine learning setting where the goal is to train a high-quality centralized model while training data remains distributed over a large number of clients each with unreliable and relatively slow network connections. We consider learning algorithms for this setting where on each round, each client independently computes an update to the current model based on its local data, and communicates this update to a central server, where the client-side updates are aggregated to compute a new global model. The typical clients in this setting are mobile phones, and communication efficiency is of the utmost importance. In this paper, we propose two ways to reduce the uplink communication costs: structured updates, where we directly learn an update from a restricted space parametrized using a smaller number of variables, e.g. either low-rank or a random mask; and sketched updates, where we learn a full model update and then compress it using a combination of quantization, random rotations, and subsampling before sending it to the server. Experiments on both convolutional and recurrent networks show that the proposed methods can reduce the communication cost by two orders of magnitude.},
	urldate = {2022-09-26},
	publisher = {arXiv},
	author = {Konečný, Jakub and McMahan, H. Brendan and Yu, Felix X. and Richtárik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
	month = oct,
	year = {2017},
	note = {arXiv:1610.05492 [cs]},
	keywords = {Computer Science - Machine Learning},
}

@misc{han_deep_2016,
	title = {Deep {Compression}: {Compressing} {Deep} {Neural} {Networks} with {Pruning}, {Trained} {Quantization} and {Huffman} {Coding}},
	shorttitle = {Deep {Compression}},
	url = {http://arxiv.org/abs/1510.00149},
	doi = {10.48550/arXiv.1510.00149},
	abstract = {Neural networks are both computationally intensive and memory intensive, making them difficult to deploy on embedded systems with limited hardware resources. To address this limitation, we introduce "deep compression", a three stage pipeline: pruning, trained quantization and Huffman coding, that work together to reduce the storage requirement of neural networks by 35x to 49x without affecting their accuracy. Our method first prunes the network by learning only the important connections. Next, we quantize the weights to enforce weight sharing, finally, we apply Huffman coding. After the first two steps we retrain the network to fine tune the remaining connections and the quantized centroids. Pruning, reduces the number of connections by 9x to 13x; Quantization then reduces the number of bits that represent each connection from 32 to 5. On the ImageNet dataset, our method reduced the storage required by AlexNet by 35x, from 240MB to 6.9MB, without loss of accuracy. Our method reduced the size of VGG-16 by 49x from 552MB to 11.3MB, again with no loss of accuracy. This allows fitting the model into on-chip SRAM cache rather than off-chip DRAM memory. Our compression method also facilitates the use of complex neural networks in mobile applications where application size and download bandwidth are constrained. Benchmarked on CPU, GPU and mobile GPU, compressed network has 3x to 4x layerwise speedup and 3x to 7x better energy efficiency.},
	urldate = {2022-09-26},
	publisher = {arXiv},
	author = {Han, Song and Mao, Huizi and Dally, William J.},
	month = feb,
	year = {2016},
	note = {arXiv:1510.00149 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Neural and Evolutionary Computing},
}

@inproceedings{hamer_fedboost_2020,
	title = {{FedBoost}: {A} {Communication}-{Efficient} {Algorithm} for {Federated} {Learning}},
	shorttitle = {{FedBoost}},
	url = {https://proceedings.mlr.press/v119/hamer20a.html},
	abstract = {Communication cost is often a bottleneck in federated learning and other client-based distributed learning scenarios. To overcome this, several gradient compression and model compression algorithms have been proposed. In this work, we propose an alternative approach whereby an ensemble of pre-trained base predictors is trained via federated learning. This method allows for training a model which may otherwise surpass the communication bandwidth and storage capacity of the clients to be learned with on-device data through federated learning. Motivated by language modeling, we prove the optimality of ensemble methods for density estimation for standard empirical risk minimization and agnostic risk minimization. We provide communication-efficient ensemble algorithms for federated learning, where per-round communication cost is independent of the size of the ensemble. Furthermore, unlike works on gradient compression, our proposed approach reduces the communication cost of both server-to-client and client-to-server communication.},
	language = {en},
	urldate = {2022-09-26},
	booktitle = {Proceedings of the 37th {International} {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Hamer, Jenny and Mohri, Mehryar and Suresh, Ananda Theertha},
	month = nov,
	year = {2020},
	note = {ISSN: 2640-3498},
	pages = {3973--3983},
}

@misc{konecny_federated_2017-1,
	title = {Federated {Learning}: {Strategies} for {Improving} {Communication} {Efficiency}},
	shorttitle = {Federated {Learning}},
	url = {http://arxiv.org/abs/1610.05492},
	abstract = {Federated Learning is a machine learning setting where the goal is to train a high-quality centralized model while training data remains distributed over a large number of clients each with unreliable and relatively slow network connections. We consider learning algorithms for this setting where on each round, each client independently computes an update to the current model based on its local data, and communicates this update to a central server, where the client-side updates are aggregated to compute a new global model. The typical clients in this setting are mobile phones, and communication efficiency is of the utmost importance. In this paper, we propose two ways to reduce the uplink communication costs: structured updates, where we directly learn an update from a restricted space parametrized using a smaller number of variables, e.g. either low-rank or a random mask; and sketched updates, where we learn a full model update and then compress it using a combination of quantization, random rotations, and subsampling before sending it to the server. Experiments on both convolutional and recurrent networks show that the proposed methods can reduce the communication cost by two orders of magnitude.},
	urldate = {2022-09-26},
	publisher = {arXiv},
	author = {Konečný, Jakub and McMahan, H. Brendan and Yu, Felix X. and Richtárik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
	month = oct,
	year = {2017},
	note = {arXiv:1610.05492 [cs]},
	keywords = {Computer Science - Machine Learning},
}



@misc{wightman_pytorch_2019,
	title = {{PyTorch} {Image} {Models}},
	url = {https://github.com/rwightman/pytorch-image-models},
	publisher = {GitHub},
	author = {Wightman, Ross},
	year = {2019},
	doi = {10.5281/zenodo.4414861},
	note = {Publication Title: GitHub repository},
}

@article{wang_generalizing_2019,
	title = {Generalizing from a {Few} {Examples}: {A} {Survey} on {Few}-{Shot} {Learning}},
	shorttitle = {Generalizing from a {Few} {Examples}},
	url = {https://arxiv.org/abs/1904.05046v3},
	doi = {10.48550/arXiv.1904.05046},
	abstract = {Machine learning has been highly successful in data-intensive applications but is often hampered when the data set is small. Recently, Few-Shot Learning (FSL) is proposed to tackle this problem. Using prior knowledge, FSL can rapidly generalize to new tasks containing only a few samples with supervised information. In this paper, we conduct a thorough survey to fully understand FSL. Starting from a formal definition of FSL, we distinguish FSL from several relevant machine learning problems. We then point out that the core issue in FSL is that the empirical risk minimized is unreliable. Based on how prior knowledge can be used to handle this core issue, we categorize FSL methods from three perspectives: (i) data, which uses prior knowledge to augment the supervised experience; (ii) model, which uses prior knowledge to reduce the size of the hypothesis space; and (iii) algorithm, which uses prior knowledge to alter the search for the best hypothesis in the given hypothesis space. With this taxonomy, we review and discuss the pros and cons of each category. Promising directions, in the aspects of the FSL problem setups, techniques, applications and theories, are also proposed to provide insights for future research.},
	language = {en},
	urldate = {2022-09-26},
	author = {Wang, Yaqing and Yao, Quanming and Kwok, James and Ni, Lionel M.},
	month = apr,
	year = {2019},
}

@article{wang_generalizing_2021,
	title = {Generalizing from a {Few} {Examples}: {A} {Survey} on {Few}-shot {Learning}},
	volume = {53},
	issn = {0360-0300, 1557-7341},
	shorttitle = {Generalizing from a {Few} {Examples}},
	url = {https://dl.acm.org/doi/10.1145/3386252},
	doi = {10.1145/3386252},
	abstract = {Machine learning has been highly successful in data-intensive applications but is often hampered when the data set is small. Recently, Few-shot Learning (FSL) is proposed to tackle this problem. Using prior knowledge, FSL can rapidly generalize to new tasks containing only a few samples with supervised information. In this article, we conduct a thorough survey to fully understand FSL. Starting from a formal definition of FSL, we distinguish FSL from several relevant machine learning problems. We then point out that the core issue in FSL is that the empirical risk minimizer is unreliable. Based on how prior knowledge can be used to handle this core issue, we categorize FSL methods from three perspectives: (i) data, which uses prior knowledge to augment the supervised experience; (ii) model, which uses prior knowledge to reduce the size of the hypothesis space; and (iii) algorithm, which uses prior knowledge to alter the search for the best hypothesis in the given hypothesis space. With this taxonomy, we review and discuss the pros and cons of each category. Promising directions, in the aspects of the FSL problem setups, techniques, applications, and theories, are also proposed to provide insights for future research.
              1},
	language = {en},
	number = {3},
	urldate = {2022-09-26},
	journal = {ACM Computing Surveys},
	author = {Wang, Yaqing and Yao, Quanming and Kwok, James T. and Ni, Lionel M.},
	month = may,
	year = {2021},
	pages = {1--34},
}



@inproceedings{CCNET-ICCV-2019,
  author    = {Zilong Huang and
               Xinggang Wang and
               Lichao Huang and
               Chang Huang and
               Yunchao Wei and
               Wenyu Liu},
  title     = {CCNet: Criss-Cross Attention for Semantic Segmentation},
  booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
               2019, Seoul, Korea (South), October 27 - November 2, 2019},
  pages     = {603--612},
  publisher = {{IEEE}},
  year      = {2019},
}


@inproceedings{partial-better-than-all-2021,
  author    = {Zhiqiang Shen and
               Zechun Liu and
               Jie Qin and
               Marios Savvides and
               Kwang{-}Ting Cheng},
  title     = {Partial Is Better Than All: Revisiting Fine-tuning Strategy for Few-shot
               Learning},
  booktitle = {Thirty-Fifth {AAAI} Conference on Artificial Intelligence, {AAAI}},
  pages     = {9594--9602},
  publisher = {{AAAI} Press},
  year      = {2021},
}




@inproceedings{bonawitz2017practical,
  title={Practical secure aggregation for privacy-preserving machine learning},
  author={Bonawitz, Keith and Ivanov, Vladimir and Kreuter, Ben and Marcedone, Antonio and McMahan, H Brendan and Patel, Sarvar and Ramage, Daniel and Segal, Aaron and Seth, Karn},
  booktitle={Proceedings of the 2017 ACM SIGSAC Conference on Computer and Communications Security},
  pages={1175--1191},
  year={2017}
}


@article{speedtest,
  title={speedtest.net. Speedtest market report.},
  journal={http://www.speedtest.net/reports/united-states/},
  year={2016}
}



@article{veeling_rotation_2018,
	title = {Rotation {Equivariant} {CNNs} for {Digital} {Pathology}},
	author = {Veeling, Bastiaan S and Linmans, Jasper and Winkens, Jim and Cohen, Taco and Welling, Max},
	month = jun,
	year = {2018},
	note = {\_eprint: 1806.03962},
}

@misc{tan_federated_2022,
	title = {Federated {Learning} from {Pre}-{Trained} {Models}: {A} {Contrastive} {Learning} {Approach}},
	shorttitle = {Federated {Learning} from {Pre}-{Trained} {Models}},
	url = {http://arxiv.org/abs/2209.10083},
	abstract = {Federated Learning (FL) is a machine learning paradigm that allows decentralized clients to learn collaboratively without sharing their private data. However, excessive computation and communication demands pose challenges to current FL frameworks, especially when training large-scale models. To prevent these issues from hindering the deployment of FL systems, we propose a lightweight framework where clients jointly learn to fuse the representations generated by multiple fixed pre-trained models rather than training a large-scale model from scratch. This leads us to a more practical FL problem by considering how to capture more client-specific and class-relevant information from the pre-trained models and jointly improve each client's ability to exploit those off-the-shelf models. In this work, we design a Federated Prototype-wise Contrastive Learning (FedPCL) approach which shares knowledge across clients through their class prototypes and builds client-specific representations in a prototype-wise contrastive manner. Sharing prototypes rather than learnable model parameters allows each client to fuse the representations in a personalized way while keeping the shared knowledge in a compact form for efficient communication. We perform a thorough evaluation of the proposed FedPCL in the lightweight framework, measuring and visualizing its ability to fuse various pre-trained models on popular FL datasets.},
	urldate = {2022-09-23},
	publisher = {arXiv},
	author = {Tan, Yue and Long, Guodong and Ma, Jie and Liu, Lu and Zhou, Tianyi and Jiang, Jing},
	month = sep,
	year = {2022},
	note = {arXiv:2209.10083 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Cryptography and Security, Computer Science - Machine Learning},
}


@misc{ruder_overview_2017,
	title = {An overview of gradient descent optimization algorithms},
	url = {http://arxiv.org/abs/1609.04747},
	doi = {10.48550/arXiv.1609.04747},
	abstract = {Gradient descent optimization algorithms, while increasingly popular, are often used as black-box optimizers, as practical explanations of their strengths and weaknesses are hard to come by. This article aims to provide the reader with intuitions with regard to the behaviour of different algorithms that will allow her to put them to use. In the course of this overview, we look at different variants of gradient descent, summarize challenges, introduce the most common optimization algorithms, review architectures in a parallel and distributed setting, and investigate additional strategies for optimizing gradient descent.},
	urldate = {2022-09-22},
	publisher = {arXiv},
	author = {Ruder, Sebastian},
	month = jun,
	year = {2017},
	note = {arXiv:1609.04747 [cs]},
	keywords = {Computer Science - Machine Learning},
}


@inproceedings{shokri2015privacy,
  title={Privacy-preserving deep learning},
  author={Shokri, Reza and Shmatikov, Vitaly},
  booktitle={Proceedings of the 22nd ACM SIGSAC conference on computer and communications security},
  pages={1310--1321},
  year={2015}
}

@article{konevcny2016federated,
  title={Federated learning: Strategies for improving communication efficiency},
  author={Kone{\v{c}}n{\`y}, Jakub and McMahan, H Brendan and Yu, Felix X and Richt{\'a}rik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
  journal={arXiv preprint arXiv:1610.05492},
  year={2016}
}









@misc{ridnik_imagenet-21k_2021,
	title = {{ImageNet}-{21K} {Pretraining} for the {Masses}},
	url = {http://arxiv.org/abs/2104.10972},
	doi = {10.48550/arXiv.2104.10972},
	abstract = {ImageNet-1K serves as the primary dataset for pretraining deep learning models for computer vision tasks. ImageNet-21K dataset, which is bigger and more diverse, is used less frequently for pretraining, mainly due to its complexity, low accessibility, and underestimation of its added value. This paper aims to close this gap, and make high-quality efficient pretraining on ImageNet-21K available for everyone. Via a dedicated preprocessing stage, utilization of WordNet hierarchical structure, and a novel training scheme called semantic softmax, we show that various models significantly benefit from ImageNet-21K pretraining on numerous datasets and tasks, including small mobile-oriented models. We also show that we outperform previous ImageNet-21K pretraining schemes for prominent new models like ViT and Mixer. Our proposed pretraining pipeline is efficient, accessible, and leads to SoTA reproducible results, from a publicly available dataset. The training code and pretrained models are available at: https://github.com/Alibaba-MIIL/ImageNet21K},
	urldate = {2022-09-22},
	publisher = {arXiv},
	author = {Ridnik, Tal and Ben-Baruch, Emanuel and Noy, Asaf and Zelnik-Manor, Lihi},
	month = aug,
	year = {2021},
	note = {arXiv:2104.10972 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@techreport{krizhevsky_learning_2009,
	title = {Learning multiple layers of features from tiny images},
	abstract = {Groups at MIT and NYU have collected a dataset of millions of tiny colour images from the web. It is, in principle, an excellent dataset for unsupervised training of deep generative models, but previous researchers who have tried this have found it difficult to learn a good set of filters from the images. We show how to train a multi-layer generative model that learns to extract meaningful features which resemble those found in the human visual cortex. Using a novel parallelization algorithm to distribute the work among multiple machines connected on a network, we show how training such a model can be done in reasonable time. A second problematic aspect of the tiny images dataset is that there are no reliable class labels which makes it hard to use for object recognition experiments. We created two sets of reliable labels. The CIFAR-10 set has 6000 examples of each of 10 classes and the CIFAR-100 set has 600 examples of each of 100 non-overlapping classes. Using these labels, we show that object recognition is significantly},
	author = {Krizhevsky, Alex},
	year = {2009},
}

@misc{liu_few-shot_2022,
	title = {Few-{Shot} {Parameter}-{Efficient} {Fine}-{Tuning} is {Better} and {Cheaper} than {In}-{Context} {Learning}},
	url = {http://arxiv.org/abs/2205.05638},
	abstract = {Few-shot in-context learning (ICL) enables pre-trained language models to perform a previously-unseen task without any gradient-based training by feeding a small number of training examples as part of the input. ICL incurs substantial computational, memory, and storage costs because it involves processing all of the training examples every time a prediction is made. Parameter-efficient fine-tuning (PEFT) (e.g. adapter modules, prompt tuning, sparse update methods, etc.) offers an alternative paradigm where a small set of parameters are trained to enable a model to perform the new task. In this paper, we rigorously compare few-shot ICL and PEFT and demonstrate that the latter offers better accuracy as well as dramatically lower computational costs. Along the way, we introduce a new PEFT method called (IA)\${\textasciicircum}3\$ that scales activations by learned vectors, attaining stronger performance while only introducing a relatively tiny amount of new parameters. We also propose a simple recipe based on the T0 model called T-Few that can be applied to new tasks without task-specific tuning or modifications. We validate the effectiveness of T-Few on completely unseen tasks by applying it to the RAFT benchmark, attaining super-human performance for the first time and outperforming the state-of-the-art by 6\% absolute. All of the code used in our experiments is publicly available.},
	urldate = {2022-09-18},
	publisher = {arXiv},
	author = {Liu, Haokun and Tam, Derek and Muqeeth, Mohammed and Mohta, Jay and Huang, Tenghao and Bansal, Mohit and Raffel, Colin},
	month = aug,
	year = {2022},
	note = {arXiv:2205.05638 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
}

@misc{wang_tackling_2020,
	title = {Tackling the {Objective} {Inconsistency} {Problem} in {Heterogeneous} {Federated} {Optimization}},
	url = {http://arxiv.org/abs/2007.07481},
	doi = {10.48550/arXiv.2007.07481},
	abstract = {In federated optimization, heterogeneity in the clients' local datasets and computation speeds results in large variations in the number of local updates performed by each client in each communication round. Naive weighted aggregation of such models causes objective inconsistency, that is, the global model converges to a stationary point of a mismatched objective function which can be arbitrarily different from the true objective. This paper provides a general framework to analyze the convergence of federated heterogeneous optimization algorithms. It subsumes previously proposed methods such as FedAvg and FedProx and provides the first principled understanding of the solution bias and the convergence slowdown due to objective inconsistency. Using insights from this analysis, we propose FedNova, a normalized averaging method that eliminates objective inconsistency while preserving fast error convergence.},
	urldate = {2022-09-18},
	publisher = {arXiv},
	author = {Wang, Jianyu and Liu, Qinghua and Liang, Hao and Joshi, Gauri and Poor, H. Vincent},
	month = jul,
	year = {2020},
	note = {arXiv:2007.07481 [cs, stat]},
	keywords = {Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning, Statistics - Machine Learning},
}

@misc{yurochkin_bayesian_2019,
	title = {Bayesian {Nonparametric} {Federated} {Learning} of {Neural} {Networks}},
	url = {http://arxiv.org/abs/1905.12022},
	doi = {10.48550/arXiv.1905.12022},
	abstract = {In federated learning problems, data is scattered across different servers and exchanging or pooling it is often impractical or prohibited. We develop a Bayesian nonparametric framework for federated learning with neural networks. Each data server is assumed to provide local neural network weights, which are modeled through our framework. We then develop an inference approach that allows us to synthesize a more expressive global network without additional supervision, data pooling and with as few as a single communication round. We then demonstrate the efficacy of our approach on federated learning problems simulated from two popular image classification datasets.},
	urldate = {2022-09-18},
	publisher = {arXiv},
	author = {Yurochkin, Mikhail and Agarwal, Mayank and Ghosh, Soumya and Greenewald, Kristjan and Hoang, Trong Nghia and Khazaeni, Yasaman},
	month = may,
	year = {2019},
	note = {arXiv:1905.12022 [cs, stat]},
	keywords = {Computer Science - Machine Learning, Statistics - Machine Learning},
}


@article{mendieta_local_2022,
    author    = {Mendieta, Matias and Yang, Taojiannan and Wang, Pu and Lee, Minwoo and Ding, Zhengming and Chen, Chen},
    title     = {Local Learning Matters: Rethinking Data Heterogeneity in Federated Learning},
    journal = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {8397-8406}
}

@article{li_model-contrastive_2021,
	author = {Li, Qinbin and He, Bingsheng and Song, Dawn},
		title = {Model-{Contrastive} {Federated} {Learning}},
journal = {IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
	year = {2021},
}

@misc{li_federated_2020,
	title = {Federated {Optimization} in {Heterogeneous} {Networks}},
	url = {http://arxiv.org/abs/1812.06127},
	doi = {10.48550/arXiv.1812.06127},
	abstract = {Federated Learning is a distributed learning paradigm with two key challenges that differentiate it from traditional distributed optimization: (1) significant variability in terms of the systems characteristics on each device in the network (systems heterogeneity), and (2) non-identically distributed data across the network (statistical heterogeneity). In this work, we introduce a framework, FedProx, to tackle heterogeneity in federated networks. FedProx can be viewed as a generalization and re-parametrization of FedAvg, the current state-of-the-art method for federated learning. While this re-parameterization makes only minor modifications to the method itself, these modifications have important ramifications both in theory and in practice. Theoretically, we provide convergence guarantees for our framework when learning over data from non-identical distributions (statistical heterogeneity), and while adhering to device-level systems constraints by allowing each participating device to perform a variable amount of work (systems heterogeneity). Practically, we demonstrate that FedProx allows for more robust convergence than FedAvg across a suite of realistic federated datasets. In particular, in highly heterogeneous settings, FedProx demonstrates significantly more stable and accurate convergence behavior relative to FedAvg---improving absolute test accuracy by 22\% on average.},
	urldate = {2022-09-18},
	publisher = {arXiv},
	author = {Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
	month = apr,
	year = {2020},
	note = {arXiv:1812.06127 [cs, stat]},
	keywords = {Computer Science - Machine Learning, Statistics - Machine Learning},
}

@article{dwork_algorithmic_2014,
	title = {The algorithmic foundations of differential privacy},
	volume = {9},
	number = {3–4},
	journal = {Foundations and Trends® in Theoretical Computer Science},
	author = {Dwork, Cynthia and Roth, Aaron and {others}},
	year = {2014},
	note = {Publisher: Now Publishers, Inc.},
	pages = {211--407},
}

@inproceedings{dwork_differential_2008,
	address = {Berlin, Heidelberg},
	series = {Lecture {Notes} in {Computer} {Science}},
	title = {Differential {Privacy}: {A} {Survey} of {Results}},
	isbn = {978-3-540-79228-4},
	shorttitle = {Differential {Privacy}},
	doi = {10.1007/978-3-540-79228-4_1},
	abstract = {Over the past five years a new approach to privacy-preserving data analysis has born fruit [13, 18, 7, 19, 5, 37, 35, 8, 32]. This approach differs from much (but not all!) of the related literature in the statistics, databases, theory, and cryptography communities, in that a formal and ad omnia privacy guarantee is defined, and the data analysis techniques presented are rigorously proved to satisfy the guarantee. The key privacy guarantee that has emerged is differential privacy. Roughly speaking, this ensures that (almost, and quantifiably) no risk is incurred by joining a statistical database.},
	language = {en},
	booktitle = {Theory and {Applications} of {Models} of {Computation}},
	publisher = {Springer},
	author = {Dwork, Cynthia},
	editor = {Agrawal, Manindra and Du, Dingzhu and Duan, Zhenhua and Li, Angsheng},
	year = {2008},
	keywords = {Differential Privacy, Privacy Mechanism, Statistical Database, Statistical Query, True Answer},
	pages = {1--19},
}

@inproceedings{dwork_calibrating_2006,
	address = {Berlin, Heidelberg},
	series = {Lecture {Notes} in {Computer} {Science}},
	title = {Calibrating {Noise} to {Sensitivity} in {Private} {Data} {Analysis}},
	isbn = {978-3-540-32732-5},
	doi = {10.1007/11681878_14},
	abstract = {We continue a line of research initiated in [10,11]on privacy-preserving statistical databases. Consider a trusted server that holds a database of sensitive information. Given a query function f mapping databases to reals, the so-called true answer is the result of applying f to the database. To protect privacy, the true answer is perturbed by the addition of random noise generated according to a carefully chosen distribution, and this response, the true answer plus noise, is returned to the user.},
	language = {en},
	booktitle = {Theory of {Cryptography}},
	publisher = {Springer},
	author = {Dwork, Cynthia and McSherry, Frank and Nissim, Kobbi and Smith, Adam},
	editor = {Halevi, Shai and Rabin, Tal},
	year = {2006},
	keywords = {Laplace Distribution, Privacy Breach, Query Function, Semantic Security, True Answer},
	pages = {265--284},
}

@misc{hatamizadeh_gradvit_2022,
	title = {{GradViT}: {Gradient} {Inversion} of {Vision} {Transformers}},
	shorttitle = {{GradViT}},
	url = {http://arxiv.org/abs/2203.11894},
	doi = {10.48550/arXiv.2203.11894},
	abstract = {In this work we demonstrate the vulnerability of vision transformers (ViTs) to gradient-based inversion attacks. During this attack, the original data batch is reconstructed given model weights and the corresponding gradients. We introduce a method, named GradViT, that optimizes random noise into naturally looking images via an iterative process. The optimization objective consists of (i) a loss on matching the gradients, (ii) image prior in the form of distance to batch-normalization statistics of a pretrained CNN model, and (iii) a total variation regularization on patches to guide correct recovery locations. We propose a unique loss scheduling function to overcome local minima during optimization. We evaluate GadViT on ImageNet1K and MS-Celeb-1M datasets, and observe unprecedentedly high fidelity and closeness to the original (hidden) data. During the analysis we find that vision transformers are significantly more vulnerable than previously studied CNNs due to the presence of the attention mechanism. Our method demonstrates new state-of-the-art results for gradient inversion in both qualitative and quantitative metrics. Project page at https://gradvit.github.io/.},
	urldate = {2022-09-18},
	publisher = {arXiv},
	author = {Hatamizadeh, Ali and Yin, Hongxu and Roth, Holger and Li, Wenqi and Kautz, Jan and Xu, Daguang and Molchanov, Pavlo},
	month = mar,
	year = {2022},
	note = {arXiv:2203.11894 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Cryptography and Security, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
}

@article{zhu_r-gap_2021,
	title = {R-{GAP}: {RECURSIVE} {GRADIENT} {ATTACK} {ON} {PRIVACY}},
	abstract = {Federated learning frameworks have been regarded as a promising approach to break the dilemma between demands on privacy and the promise of learning from large collections of distributed data. Many such frameworks only ask collaborators to share their local update of a common model, i.e. gradients, instead of exposing their raw data to other collaborators. However, recent optimization-based gradient attacks show that raw data can often be accurately recovered from gradients. It has been shown that minimizing the Euclidean distance between true gradients and those calculated from estimated data is often effective in fully recovering private data. However, there is a fundamental lack of theoretical understanding of how and when gradients can lead to unique recovery of original data. Our research ﬁlls this gap by providing a closed-form recursive procedure to recover data from gradients in deep neural networks. We name it Recursive Gradient Attack on Privacy (R-GAP). Experimental results demonstrate that R-GAP works as well as or even better than optimization-based approaches at a fraction of the computation under certain conditions. Additionally, we propose a Rank Analysis method, which can be used to estimate the risk of gradient attacks inherent in certain network architectures, regardless of whether an optimization-based or closed-form-recursive attack is used. Experimental results demonstrate the utility of the rank analysis towards improving the network’s security. Source code is available for download from https://github.com/JunyiZhu-AI/R-GAP.},
	language = {en},
	author = {Zhu, Junyi and Blaschko, Matthew},
	year = {2021},
	pages = {17},
}

@misc{liu_few-shot_2022-1,
	title = {Few-{Shot} {Parameter}-{Efficient} {Fine}-{Tuning} is {Better} and {Cheaper} than {In}-{Context} {Learning}},
	url = {http://arxiv.org/abs/2205.05638},
	abstract = {Few-shot in-context learning (ICL) enables pre-trained language models to perform a previously-unseen task without any gradient-based training by feeding a small number of training examples as part of the input. ICL incurs substantial computational, memory, and storage costs because it involves processing all of the training examples every time a prediction is made. Parameter-efficient fine-tuning (PEFT) (e.g. adapter modules, prompt tuning, sparse update methods, etc.) offers an alternative paradigm where a small set of parameters are trained to enable a model to perform the new task. In this paper, we rigorously compare few-shot ICL and PEFT and demonstrate that the latter offers better accuracy as well as dramatically lower computational costs. Along the way, we introduce a new PEFT method called (IA)\${\textasciicircum}3\$ that scales activations by learned vectors, attaining stronger performance while only introducing a relatively tiny amount of new parameters. We also propose a simple recipe based on the T0 model called T-Few that can be applied to new tasks without task-specific tuning or modifications. We validate the effectiveness of T-Few on completely unseen tasks by applying it to the RAFT benchmark, attaining super-human performance for the first time and outperforming the state-of-the-art by 6\% absolute. All of the code used in our experiments is publicly available.},
	urldate = {2022-09-17},
	publisher = {arXiv},
	author = {Liu, Haokun and Tam, Derek and Muqeeth, Mohammed and Mohta, Jay and Huang, Tenghao and Bansal, Mohit and Raffel, Colin},
	month = aug,
	year = {2022},
	note = {arXiv:2205.05638 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Machine Learning},
}

@misc{liu_p-tuning_2022,
	title = {P-{Tuning} v2: {Prompt} {Tuning} {Can} {Be} {Comparable} to {Fine}-tuning {Universally} {Across} {Scales} and {Tasks}},
	shorttitle = {P-{Tuning} v2},
	url = {http://arxiv.org/abs/2110.07602},
	doi = {10.48550/arXiv.2110.07602},
	abstract = {Prompt tuning, which only tunes continuous prompts with a frozen language model, substantially reduces per-task storage and memory usage at training. However, in the context of NLU, prior work reveals that prompt tuning does not perform well for normal-sized pretrained models. We also find that existing methods of prompt tuning cannot handle hard sequence labeling tasks, indicating a lack of universality. We present a novel empirical finding that properly optimized prompt tuning can be universally effective across a wide range of model scales and NLU tasks. It matches the performance of finetuning while having only 0.1\%-3\% tuned parameters. Our method P-Tuning v2 is an implementation of Deep Prompt Tuning {\textbackslash}cite\{li2021prefix,qin2021learning\} optimized and adapted for NLU. Given the universality and simplicity of P-Tuning v2, we believe it can serve as an alternative to finetuning and a strong baseline for future research.Our code and data are released at https://github.com/THUDM/P-tuning-v2.},
	urldate = {2022-09-17},
	publisher = {arXiv},
	author = {Liu, Xiao and Ji, Kaixuan and Fu, Yicheng and Tam, Weng Lam and Du, Zhengxiao and Yang, Zhilin and Tang, Jie},
	month = mar,
	year = {2022},
	note = {arXiv:2110.07602 [cs]},
	keywords = {Computer Science - Computation and Language},
}

@inproceedings{pfeiffer_adapterhub_2020,
	address = {Online},
	title = {{AdapterHub}: {A} {Framework} for {Adapting} {Transformers}},
	shorttitle = {{AdapterHub}},
	url = {https://aclanthology.org/2020.emnlp-demos.7},
	doi = {10.18653/v1/2020.emnlp-demos.7},
	abstract = {The current modus operandi in NLP involves downloading and fine-tuning pre-trained models consisting of millions or billions of parameters. Storing and sharing such large trained models is expensive, slow, and time-consuming, which impedes progress towards more general and versatile NLP methods that learn from and for many tasks. Adapters—small learnt bottleneck layers inserted within each layer of a pre-trained model— ameliorate this issue by avoiding full fine-tuning of the entire model. However, sharing and integrating adapter layers is not straightforward. We propose AdapterHub, a framework that allows dynamic “stiching-in” of pre-trained adapters for different tasks and languages. The framework, built on top of the popular HuggingFace Transformers library, enables extremely easy and quick adaptations of state-of-the-art pre-trained models (e.g., BERT, RoBERTa, XLM-R) across tasks and languages. Downloading, sharing, and training adapters is as seamless as possible using minimal changes to the training scripts and a specialized infrastructure. Our framework enables scalable and easy access to sharing of task-specific models, particularly in low-resource scenarios. AdapterHub includes all recent adapter architectures and can be found at AdapterHub.ml},
	urldate = {2022-09-17},
	booktitle = {Proceedings of the 2020 {Conference} on {Empirical} {Methods} in {Natural} {Language} {Processing}: {System} {Demonstrations}},
	publisher = {Association for Computational Linguistics},
	author = {Pfeiffer, Jonas and Rücklé, Andreas and Poth, Clifton and Kamath, Aishwarya and Vulić, Ivan and Ruder, Sebastian and Cho, Kyunghyun and Gurevych, Iryna},
	year = {2020},
	pages = {46--54},
}

@inproceedings{cai_tinytl_2020,
	title = {{TinyTL}: {Reduce} {Memory}, {Not} {Parameters} for {Efficient} {On}-{Device} {Learning}},
	volume = {33},
	shorttitle = {{TinyTL}},
	url = {https://proceedings.neurips.cc/paper/2020/hash/81f7acabd411274fcf65ce2070ed568a-Abstract.html},
	abstract = {Efficient on-device learning requires a small memory footprint at training time to fit the tight memory constraint. Existing work solves this problem by reducing the number of trainable parameters. However, this doesn't directly translate to memory saving since the major bottleneck is the activations, not parameters.
In this work, we present Tiny-Transfer-Learning (TinyTL) for memory-efficient on-device learning. TinyTL freezes the weights while only learns the memory-efficient bias modules, thus no need to store the intermediate activations. To maintain the adaptation capacity, we introduce a new memory-efficient bias module, the lite residual module, to refine the feature extractor by learning small residual feature maps adding only 3.8\% memory overhead. Extensive experiments show that TinyTL significantly saves the memory (up to 6.5x) with little accuracy loss compared to fine-tuning the full network. Compared to fine-tuning the last layer, TinyTL provides significant accuracy improvements (up to 33.8\%) with little memory overhead. Furthermore, combined with feature extractor adaptation, TinyTL provides 7.5-12.9x memory saving without sacrificing accuracy compared to fine-tuning the full Inception-V3. Code is released at https://github.com/mit-han-lab/tinyML/tree/master/tinyTL.},
	urldate = {2022-09-17},
	booktitle = {Advances in {Neural} {Information} {Processing} {Systems}},
	publisher = {Curran Associates, Inc.},
	author = {Cai, Han and Gan, Chuang and Zhu, Ligeng and Han, Song},
	year = {2020},
	pages = {11285--11297},
}
@article{naseer2021intriguing,
  title={Intriguing properties of vision transformers},
  author={Naseer, Muhammad Muzammal and Ranasinghe, Kanchana and Khan, Salman H and Hayat, Munawar and Shahbaz Khan, Fahad and Yang, Ming-Hsuan},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={23296--23308},
  year={2021}
}
@misc{dosovitskiy_image_2021,
	title = {An {Image} is {Worth} 16x16 {Words}: {Transformers} for {Image} {Recognition} at {Scale}},
	shorttitle = {An {Image} is {Worth} 16x16 {Words}},
	url = {http://arxiv.org/abs/2010.11929},
	doi = {10.48550/arXiv.2010.11929},
	abstract = {While the Transformer architecture has become the de-facto standard for natural language processing tasks, its applications to computer vision remain limited. In vision, attention is either applied in conjunction with convolutional networks, or used to replace certain components of convolutional networks while keeping their overall structure in place. We show that this reliance on CNNs is not necessary and a pure transformer applied directly to sequences of image patches can perform very well on image classification tasks. When pre-trained on large amounts of data and transferred to multiple mid-sized or small image recognition benchmarks (ImageNet, CIFAR-100, VTAB, etc.), Vision Transformer (ViT) attains excellent results compared to state-of-the-art convolutional networks while requiring substantially fewer computational resources to train.},
	urldate = {2022-09-17},
	publisher = {arXiv},
	author = {Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and Uszkoreit, Jakob and Houlsby, Neil},
	month = jun,
	year = {2021},
	note = {arXiv:2010.11929 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}


@misc{bommasani_opportunities_2022,
	title = {On the {Opportunities} and {Risks} of {Foundation} {Models}},
	url = {http://arxiv.org/abs/2108.07258},
	abstract = {AI is undergoing a paradigm shift with the rise of models (e.g., BERT, DALL-E, GPT-3) that are trained on broad data at scale and are adaptable to a wide range of downstream tasks. We call these models foundation models to underscore their critically central yet incomplete character. This report provides a thorough account of the opportunities and risks of foundation models, ranging from their capabilities (e.g., language, vision, robotics, reasoning, human interaction) and technical principles(e.g., model architectures, training procedures, data, systems, security, evaluation, theory) to their applications (e.g., law, healthcare, education) and societal impact (e.g., inequity, misuse, economic and environmental impact, legal and ethical considerations). Though foundation models are based on standard deep learning and transfer learning, their scale results in new emergent capabilities,and their effectiveness across so many tasks incentivizes homogenization. Homogenization provides powerful leverage but demands caution, as the defects of the foundation model are inherited by all the adapted models downstream. Despite the impending widespread deployment of foundation models, we currently lack a clear understanding of how they work, when they fail, and what they are even capable of due to their emergent properties. To tackle these questions, we believe much of the critical research on foundation models will require deep interdisciplinary collaboration commensurate with their fundamentally sociotechnical nature.},
	urldate = {2022-09-16},
	publisher = {arXiv},
	author = {Bommasani, Rishi and others},
	month = jul,
	year = {2022},
	note = {arXiv:2108.07258 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computers and Society, Computer Science - Machine Learning},
}

@misc{devlin_bert_2019,
	title = {{BERT}: {Pre}-training of {Deep} {Bidirectional} {Transformers} for {Language} {Understanding}},
	shorttitle = {{BERT}},
	url = {http://arxiv.org/abs/1810.04805},
	doi = {10.48550/arXiv.1810.04805},
	abstract = {We introduce a new language representation model called BERT, which stands for Bidirectional Encoder Representations from Transformers. Unlike recent language representation models, BERT is designed to pre-train deep bidirectional representations from unlabeled text by jointly conditioning on both left and right context in all layers. As a result, the pre-trained BERT model can be fine-tuned with just one additional output layer to create state-of-the-art models for a wide range of tasks, such as question answering and language inference, without substantial task-specific architecture modifications. BERT is conceptually simple and empirically powerful. It obtains new state-of-the-art results on eleven natural language processing tasks, including pushing the GLUE score to 80.5\% (7.7\% point absolute improvement), MultiNLI accuracy to 86.7\% (4.6\% absolute improvement), SQuAD v1.1 question answering Test F1 to 93.2 (1.5 point absolute improvement) and SQuAD v2.0 Test F1 to 83.1 (5.1 point absolute improvement).},
	urldate = {2022-09-16},
	publisher = {arXiv},
	author = {Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
	month = may,
	year = {2019},
	note = {arXiv:1810.04805 [cs]},
	keywords = {Computer Science - Computation and Language},
}

@inproceedings{brown_language_2020,
	title = {Language {Models} are {Few}-{Shot} {Learners}},
	volume = {33},
	url = {https://papers.nips.cc/paper/2020/hash/1457c0d6bfcb4967418bfb8ac142f64a-Abstract.html},
	abstract = {We demonstrate that scaling up language models greatly improves task-agnostic, few-shot performance, sometimes even becoming competitive with prior state-of-the-art fine-tuning approaches. Specifically, we train GPT-3, an autoregressive language model with 175 billion parameters, 10x more than any previous non-sparse language model, and test its performance in the few-shot setting.  For all tasks, GPT-3 is applied without any gradient updates or fine-tuning, with tasks and few-shot demonstrations specified purely via text interaction with the model.  GPT-3 achieves strong performance on many NLP datasets, including translation, question-answering, and cloze tasks. We also identify some datasets where GPT-3's few-shot learning still struggles, as well as some datasets where GPT-3 faces methodological issues related to training on large web corpora.},
	urldate = {2022-09-16},
	booktitle = {Advances in {Neural} {Information} {Processing} {Systems}},
	publisher = {Curran Associates, Inc.},
	author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel and Wu, Jeffrey and Winter, Clemens and Hesse, Chris and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
	year = {2020},
	pages = {1877--1901},
}

@misc{radford_learning_2021,
	title = {Learning {Transferable} {Visual} {Models} {From} {Natural} {Language} {Supervision}},
	url = {http://arxiv.org/abs/2103.00020},
	doi = {10.48550/arXiv.2103.00020},
	abstract = {State-of-the-art computer vision systems are trained to predict a fixed set of predetermined object categories. This restricted form of supervision limits their generality and usability since additional labeled data is needed to specify any other visual concept. Learning directly from raw text about images is a promising alternative which leverages a much broader source of supervision. We demonstrate that the simple pre-training task of predicting which caption goes with which image is an efficient and scalable way to learn SOTA image representations from scratch on a dataset of 400 million (image, text) pairs collected from the internet. After pre-training, natural language is used to reference learned visual concepts (or describe new ones) enabling zero-shot transfer of the model to downstream tasks. We study the performance of this approach by benchmarking on over 30 different existing computer vision datasets, spanning tasks such as OCR, action recognition in videos, geo-localization, and many types of fine-grained object classification. The model transfers non-trivially to most tasks and is often competitive with a fully supervised baseline without the need for any dataset specific training. For instance, we match the accuracy of the original ResNet-50 on ImageNet zero-shot without needing to use any of the 1.28 million training examples it was trained on. We release our code and pre-trained model weights at https://github.com/OpenAI/CLIP.},
	urldate = {2022-09-16},
	publisher = {arXiv},
	author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
	month = feb,
	year = {2021},
	note = {arXiv:2103.00020 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{chamikara_local_2020,
	title = {Local {Differential} {Privacy} for {Deep} {Learning}},
	volume = {7},
	issn = {2327-4662, 2372-2541},
	url = {http://arxiv.org/abs/1908.02997},
	doi = {10.1109/JIOT.2019.2952146},
	abstract = {The internet of things (IoT) is transforming major industries including but not limited to healthcare, agriculture, finance, energy, and transportation. IoT platforms are continually improving with innovations such as the amalgamation of software-defined networks (SDN) and network function virtualization (NFV) in the edge-cloud interplay. Deep learning (DL) is becoming popular due to its remarkable accuracy when trained with a massive amount of data, such as generated by IoT. However, DL algorithms tend to leak privacy when trained on highly sensitive crowd-sourced data such as medical data. Existing privacy-preserving DL algorithms rely on the traditional server-centric approaches requiring high processing powers. We propose a new local differentially private (LDP) algorithm named LATENT that redesigns the training process. LATENT enables a data owner to add a randomization layer before data leave the data owners' devices and reach a potentially untrusted machine learning service. This feature is achieved by splitting the architecture of a convolutional neural network (CNN) into three layers: (1) convolutional module, (2) randomization module, and (3) fully connected module. Hence, the randomization module can operate as an NFV privacy preservation service in an SDN-controlled NFV, making LATENT more practical for IoT-driven cloud-based environments compared to existing approaches. The randomization module employs a newly proposed LDP protocol named utility enhancing randomization, which allows LATENT to maintain high utility compared to existing LDP protocols. Our experimental evaluation of LATENT on convolutional deep neural networks demonstrates excellent accuracy (e.g. 91\%- 96\%) with high model quality even under low privacy budgets (e.g. \${\textbackslash}varepsilon=0.5\$).},
	number = {7},
	urldate = {2022-09-14},
	journal = {IEEE Internet of Things Journal},
	author = {Chamikara, M. A. P. and Bertok, P. and Khalil, I. and Liu, D. and Camtepe, S. and Atiquzzaman, M.},
	month = jul,
	year = {2020},
	note = {arXiv:1908.02997 [cs]},
	keywords = {Computer Science - Cryptography and Security, Computer Science - Machine Learning},
	pages = {5827--5842},
}

@misc{li_model-contrastive_2021-1,
	title = {Model-{Contrastive} {Federated} {Learning}},
	url = {http://arxiv.org/abs/2103.16257},
	abstract = {Federated learning enables multiple parties to collaboratively train a machine learning model without communicating their local data. A key challenge in federated learning is to handle the heterogeneity of local data distribution across parties. Although many studies have been proposed to address this challenge, we find that they fail to achieve high performance in image datasets with deep learning models. In this paper, we propose MOON: model-contrastive federated learning. MOON is a simple and effective federated learning framework. The key idea of MOON is to utilize the similarity between model representations to correct the local training of individual parties, i.e., conducting contrastive learning in model-level. Our extensive experiments show that MOON significantly outperforms the other state-of-the-art federated learning algorithms on various image classification tasks.},
	urldate = {2022-09-09},
	publisher = {arXiv},
	author = {Li, Qinbin and He, Bingsheng and Song, Dawn},
	month = mar,
	year = {2021},
	note = {arXiv:2103.16257 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@misc{zhao_reduce_2022,
	title = {Reduce {Communication} {Costs} and {Preserve} {Privacy}: {Prompt} {Tuning} {Method} in {Federated} {Learning}},
	shorttitle = {Reduce {Communication} {Costs} and {Preserve} {Privacy}},
	url = {http://arxiv.org/abs/2208.12268},
	abstract = {Federated learning (FL) has enabled global model training on decentralized data in a privacy-preserving way by aggregating model updates. However, for many natural language processing (NLP) tasks that utilize pre-trained language models (PLMs) with large numbers of parameters, there are considerable communication costs associated with FL. Recently, prompt tuning, which tunes some soft prompts without modifying PLMs, has achieved excellent performance as a new learning paradigm. Therefore we want to combine the two methods and explore the effect of prompt tuning under FL. In this paper, we propose "FedPrompt" as the first work study prompt tuning in a model split learning way using FL, and prove that split learning greatly reduces the communication cost, only 0.01\% of the PLMs' parameters, with little decrease on accuracy both on IID and Non-IID data distribution. This improves the efficiency of FL method while also protecting the data privacy in prompt tuning.In addition, like PLMs, prompts are uploaded and downloaded between public platforms and personal users, so we try to figure out whether there is still a backdoor threat using only soft prompt in FL scenarios. We further conduct backdoor attacks by data poisoning on FedPrompt. Our experiments show that normal backdoor attack can not achieve a high attack success rate, proving the robustness of FedPrompt.We hope this work can promote the application of prompt in FL and raise the awareness of the possible security threats.},
	urldate = {2022-09-07},
	publisher = {arXiv},
	author = {Zhao, Haodong and Du, Wei and Li, Fangqi and Li, Peixuan and Liu, Gongshen},
	month = aug,
	year = {2022},
	note = {arXiv:2208.12268 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Cryptography and Security, Computer Science - Machine Learning},
}

@misc{nguyen_where_2022,
	title = {Where to {Begin}? {Exploring} the {Impact} of {Pre}-{Training} and {Initialization} in {Federated} {Learning}},
	shorttitle = {Where to {Begin}?},
	url = {http://arxiv.org/abs/2206.15387},
	doi = {10.48550/arXiv.2206.15387},
	abstract = {An oft-cited challenge of federated learning is the presence of data heterogeneity -- the data at different clients may follow very different distributions. Several federated optimization methods have been proposed to address these challenges. In the literature, empirical evaluations usually start federated training from a random initialization. However, in many practical applications of federated learning, the server has access to proxy data for the training task which can be used to pre-train a model before starting federated training. We empirically study the impact of starting from a pre-trained model in federated learning using four common federated learning benchmark datasets. Unsurprisingly, starting from a pre-trained model reduces the training time required to reach a target error rate and enables training more accurate models (by up to 40{\textbackslash}\%) than is possible than when starting from a random initialization. Surprisingly, we also find that the effect of data heterogeneity is much less significant when starting federated training from a pre-trained initialization. Rather, when starting from a pre-trained model, using an adaptive optimizer at the server, such as {\textbackslash}textsc\{FedAdam\}, consistently leads to the best accuracy. We recommend that future work proposing and evaluating federated optimization methods consider the performance when starting both random and pre-trained initializations. We also believe this study raises several questions for further work on understanding the role of heterogeneity in federated optimization.},
	urldate = {2022-09-05},
	publisher = {arXiv},
	author = {Nguyen, John and Malik, Kshitiz and Sanjabi, Maziar and Rabbat, Michael},
	month = jun,
	year = {2022},
	note = {arXiv:2206.15387 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
}

@misc{huang_evaluating_2021,
	title = {Evaluating {Gradient} {Inversion} {Attacks} and {Defenses} in {Federated} {Learning}},
	url = {http://arxiv.org/abs/2112.00059},
	abstract = {Gradient inversion attack (or input recovery from gradient) is an emerging threat to the security and privacy preservation of Federated learning, whereby malicious eavesdroppers or participants in the protocol can recover (partially) the clients' private data. This paper evaluates existing attacks and defenses. We find that some attacks make strong assumptions about the setup. Relaxing such assumptions can substantially weaken these attacks. We then evaluate the benefits of three proposed defense mechanisms against gradient inversion attacks. We show the trade-offs of privacy leakage and data utility of these defense methods, and find that combining them in an appropriate manner makes the attack less effective, even under the original strong assumptions. We also estimate the computation cost of end-to-end recovery of a single image under each evaluated defense. Our findings suggest that the state-of-the-art attacks can currently be defended against with minor data utility loss, as summarized in a list of potential strategies. Our code is available at: https://github.com/Princeton-SysML/GradAttack.},
	urldate = {2022-09-05},
	publisher = {arXiv},
	author = {Huang, Yangsibo and Gupta, Samyak and Song, Zhao and Li, Kai and Arora, Sanjeev},
	month = nov,
	year = {2021},
	note = {arXiv:2112.00059 [cs]
version: 1},
	keywords = {Computer Science - Cryptography and Security, Computer Science - Machine Learning},
}

@article{abnar_exploring_2022,
	title = {{EXPLORING} {THE} {LIMITS} {OF} {LARGE} {SCALE} {PRE}-{TRAINING}},
	abstract = {Recent developments in large-scale machine learning suggest that by scaling up data, model size and training time properly, one might observe that improvements in pre-training would transfer favorably to most downstream tasks. In this work we systematically study this phenomena and establish that, as we increase the upstream accuracy, performance of downstream tasks saturates. In particular, we investigate more than 4800 experiments on Vision Transformers, MLP-Mixers and ResNets with number of parameters ranging from ten million to ten billion, trained on the largest scale of available image data (JFT, ImageNet21K) and evaluated on more than 20 downstream image recognition tasks. We propose a model for downstream performance that reﬂects the saturation phenomena and captures the nonlinear relationship in performance of upstream and downstream tasks. Delving deeper to understand the reasons that give rise to these phenomena, we show that the observed saturation behavior is closely related to the way that representations evolve through the layers of the models. We showcase an even more extreme scenario where performance on upstream and downstream are at odds with each other. That is, in order to have a better downstream performance, we need to hurt upstream accuracy.},
	language = {en},
	author = {Abnar, Samira and Dehghani, Mostafa and Neyshabur, Behnam and Sedghi, Hanie},
	year = {2022},
	pages = {46},
}

@misc{taher_systematic_2021,
	title = {A {Systematic} {Benchmarking} {Analysis} of {Transfer} {Learning} for {Medical} {Image} {Analysis}},
	url = {http://arxiv.org/abs/2108.05930},
	abstract = {Transfer learning from supervised ImageNet models has been frequently used in medical image analysis. Yet, no large-scale evaluation has been conducted to benchmark the efficacy of newly-developed pre-training techniques for medical image analysis, leaving several important questions unanswered. As the first step in this direction, we conduct a systematic study on the transferability of models pre-trained on iNat2021, the most recent large-scale fine-grained dataset, and 14 top self-supervised ImageNet models on 7 diverse medical tasks in comparison with the supervised ImageNet model. Furthermore, we present a practical approach to bridge the domain gap between natural and medical images by continually (pre-)training supervised ImageNet models on medical images. Our comprehensive evaluation yields new insights: (1) pre-trained models on fine-grained data yield distinctive local representations that are more suitable for medical segmentation tasks, (2) self-supervised ImageNet models learn holistic features more effectively than supervised ImageNet models, and (3) continual pre-training can bridge the domain gap between natural and medical images. We hope that this large-scale open evaluation of transfer learning can direct the future research of deep learning for medical imaging. As open science, all codes and pre-trained models are available on our GitHub page https://github.com/JLiangLab/BenchmarkTransferLearning.},
	urldate = {2022-09-01},
	publisher = {arXiv},
	author = {Taher, Mohammad Reza Hosseinzadeh and Haghighi, Fatemeh and Feng, Ruibin and Gotway, Michael B. and Liang, Jianming},
	month = aug,
	year = {2021},
	note = {arXiv:2108.05930 [cs, eess]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Electrical Engineering and Systems Science - Image and Video Processing},
}

@article{lu_prompt_nodate,
	title = {Prompt {Distribution} {Learning}},
	abstract = {We present prompt distribution learning for effectively adapting a pre-trained vision-language model to address downstream recognition tasks. Our method not only learns low-bias prompts from a few samples but also captures the distribution of diverse prompts to handle the varying visual representations. In this way, we provide high-quality taskrelated content for facilitating recognition. This prompt distribution learning is realized by an efficient approach that learns the output embeddings of prompts instead of the input embeddings. Thus, we can employ a Gaussian distribution to model them effectively and derive a surrogate loss for efficient training. Extensive experiments on 12 datasets demonstrate that our method consistently and significantly outperforms existing methods. For example, with 1 sample per category, it relatively improves the average result by 9.1\% compared to human-crafted prompts.},
	language = {en},
	author = {Lu, Yuning and Liu, Jianzhuang and Zhang, Yonggang and Liu, Yajing and Tian, Xinmei},
	pages = {10},
}

@misc{chen_adaptformer_2022,
	title = {{AdaptFormer}: {Adapting} {Vision} {Transformers} for {Scalable} {Visual} {Recognition}},
	shorttitle = {{AdaptFormer}},
	url = {http://arxiv.org/abs/2205.13535},
	doi = {10.48550/arXiv.2205.13535},
	abstract = {Although the pre-trained Vision Transformers (ViTs) achieved great success in computer vision, adapting a ViT to various image and video tasks is challenging because of its heavy computation and storage burdens, where each model needs to be independently and comprehensively fine-tuned to different tasks, limiting its transferability in different domains. To address this challenge, we propose an effective adaptation approach for Transformer, namely AdaptFormer, which can adapt the pre-trained ViTs into many different image and video tasks efficiently. It possesses several benefits more appealing than prior arts. Firstly, AdaptFormer introduces lightweight modules that only add less than 2\% extra parameters to a ViT, while it is able to increase the ViT's transferability without updating its original pre-trained parameters, significantly outperforming the existing 100\% fully fine-tuned models on action recognition benchmarks. Secondly, it can be plug-and-play in different Transformers and scalable to many visual tasks. Thirdly, extensive experiments on five image and video datasets show that AdaptFormer largely improves ViTs in the target domains. For example, when updating just 1.5\% extra parameters, it achieves about 10\% and 19\% relative improvement compared to the fully fine-tuned models on Something-Something{\textasciitilde}v2 and HMDB51, respectively. Project page: http://www.shoufachen.com/adaptformer-page.},
	urldate = {2022-08-30},
	publisher = {arXiv},
	author = {Chen, Shoufa and Ge, Chongjian and Tong, Zhan and Wang, Jiangliu and Song, Yibing and Wang, Jue and Luo, Ping},
	month = may,
	year = {2022},
	note = {arXiv:2205.13535 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@misc{yao_cpt_2022,
	title = {{CPT}: {Colorful} {Prompt} {Tuning} for {Pre}-trained {Vision}-{Language} {Models}},
	shorttitle = {{CPT}},
	url = {http://arxiv.org/abs/2109.11797},
	abstract = {Pre-Trained Vision-Language Models (VL-PTMs) have shown promising capabilities in grounding natural language in image data, facilitating a broad variety of cross-modal tasks. However, we note that there exists a signiﬁcant gap between the objective forms of model pre-training and ﬁne-tuning, resulting in a need for large amounts of labeled data to stimulate the visual grounding capability of VL-PTMs for downstream tasks. To address the challenge, we present Cross-modal Prompt Tuning (CPT, alternatively, Colorful Prompt Tuning), a novel paradigm for tuning VL-PTMs, which reformulates visual grounding into a ﬁll-in-the-blank problem with color-based co-referential markers in image and text, maximally mitigating the gap. In this way, CPT enables strong few-shot and even zero-shot visual grounding capabilities of VL-PTMs. Comprehensive experimental results show that the prompt-tuned VL-PTMs outperform their ﬁnetuned counterparts by a large margin (e.g., 17.3\% absolute accuracy improvement, and 73.8\% relative standard deviation reduction on average with one shot in RefCOCO evaluation). We make the data and code for this paper publicly available at https://github.com/thunlp/CPT.},
	language = {en},
	urldate = {2022-08-30},
	publisher = {arXiv},
	author = {Yao, Yuan and Zhang, Ao and Zhang, Zhengyan and Liu, Zhiyuan and Chua, Tat-Seng and Sun, Maosong},
	month = may,
	year = {2022},
	note = {arXiv:2109.11797 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition},
}

@misc{jia_visual_2022,
	title = {Visual {Prompt} {Tuning}},
	url = {http://arxiv.org/abs/2203.12119},
	abstract = {The current modus operandi in adapting pre-trained models involves updating all the backbone parameters, ie, full fine-tuning. This paper introduces Visual Prompt Tuning (VPT) as an efficient and effective alternative to full fine-tuning for large-scale Transformer models in vision. Taking inspiration from recent advances in efficiently tuning large language models, VPT introduces only a small amount (less than 1\% of model parameters) of trainable parameters in the input space while keeping the model backbone frozen. Via extensive experiments on a wide variety of downstream recognition tasks, we show that VPT achieves significant performance gains compared to other parameter efficient tuning protocols. Most importantly, VPT even outperforms full fine-tuning in many cases across model capacities and training data scales, while reducing per-task storage cost.},
	urldate = {2022-08-30},
	publisher = {arXiv},
	author = {Jia, Menglin and Tang, Luming and Chen, Bor-Chun and Cardie, Claire and Belongie, Serge and Hariharan, Bharath and Lim, Ser-Nam},
	month = jul,
	year = {2022},
	note = {arXiv:2203.12119 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{Fair-Federated-Learning-2021,
  author    = {Weituo Hao and
               Mostafa El{-}Khamy and
               Jungwon Lee and
               Jianyi Zhang and
               Kevin J. Liang and
               Changyou Chen and
               Lawrence Carin},
  title     = {Towards Fair Federated Learning with Zero-Shot Data Augmentation},
  journal   = {CoRR},
  volume    = {abs/2104.13417},
  year      = {2021},
}
@inproceedings{guliani2021training,
  title={Training speech recognition models with federated learning: A quality/cost framework},
  author={Guliani, Dhruv and Beaufays, Fran{\c{c}}oise and Motta, Giovanni},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3080--3084},
  year={2021},
  organization={IEEE}
}

@article{zhao2022reduce,
  title={Reduce Communication Costs and Preserve Privacy: Prompt Tuning Method in Federated Learning},
  author={Zhao, Haodong and Du, Wei and Li, Fangqi and Li, Peixuan and Liu, Gongshen},
  journal={arXiv preprint arXiv:2208.12268},
  year={2022}
}
@article{wang2020generalizing,
  title={Generalizing from a few examples: A survey on few-shot learning},
  author={Wang, Yaqing and Yao, Quanming and Kwok, James T and Ni, Lionel M},
  journal={ACM computing surveys (csur)},
  volume={53},
  number={3},
  pages={1--34},
  year={2020},
  publisher={ACM New York, NY, USA}
}
@article{pan2022st,
  title={ST-Adapter: Parameter-Efficient Image-to-Video Transfer Learning for Action Recognition},
  author={Pan, Junting and Lin, Ziyi and Zhu, Xiatian and Shao, Jing and Li, Hongsheng},
  journal={arXiv preprint arXiv:2206.13559},
  year={2022}
}
@inproceedings{lin2022frozen,
  title={Frozen CLIP Models are Efficient Video Learners},
  author={Lin, Ziyi and Geng, Shijie and Zhang, Renrui and Gao, Peng and de Melo, Gerard and Wang, Xiaogang and Dai, Jifeng and Qiao, Yu and Li, Hongsheng},
  booktitle={European Conference on Computer Vision},
  pages={388--404},
  year={2022},
  organization={Springer}
}

@article{zhao2018-non-iid,
  title={Federated learning with non-iid data},
  author={Zhao, Yue and Li, Meng and Lai, Liangzhen and Suda, Naveen and Civin, Damon and Chandra, Vikas},
  journal={arXiv preprint arXiv:1806.00582},
  year={2018}
}




@inproceedings{matched-averaging-2020,
  author    = {Hongyi Wang and
               Mikhail Yurochkin and
               Yuekai Sun and
               Dimitris S. Papailiopoulos and
               Yasaman Khazaeni},
  title     = {Federated Learning with Matched Averaging},
  booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
               Addis Ababa, Ethiopia, April 26-30, 2020},
  publisher = {OpenReview.net},
  year      = {2020},
}



@article{fallah2020personalized,
  title={Personalized federated learning with theoretical guarantees: A model-agnostic meta-learning approach},
  author={Fallah, Alireza and Mokhtari, Aryan and Ozdaglar, Asuman},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={3557--3568},
  year={2020}
}

@article{haddadpour2019convergence,
  title={On the convergence of local descent methods in federated learning},
  author={Haddadpour, Farzin and Mahdavi, Mehrdad},
  journal={arXiv preprint arXiv:1910.14425},
  year={2019}
}




@inproceedings{vahidian-pacfl-2022,
  title = {Efficient Distribution Similarity Identification in Clustered Federated Learning via Principal Angles Between Client Data Subspaces},
    author = {Vahidian, Saeed and Morafah, Mahdi and Wang, Weijia and Kungurtsev, Vyacheslav and Chen, Chen and Shah, Mubarak and Lin, Bill},
  journal      = {CoRR},
  volume       = {abs/2209.10526},
  year         = {2022},
  url          = {https://doi.org/10.48550/arXiv.2209.10526},
  doi          = {10.48550/arXiv.2209.10526},
}

@article{ghosh2020efficient,
  title={An Efficient Framework for Clustered Federated Learning},
  author={Ghosh, Avishek and Chung, Jichan and Yin, Dong and Ramchandran, Kannan},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  year={2020}
}



@ARTICLE{Vahidian-FLIS-2022,
  author={Morafah, Mahdi and Vahidian, Saeed and Wang, Weijia and Lin, Bill},
  journal={IEEE Open Journal of the Computer Society}, 
  title={{FLIS}: Clustered Federated Learning Via Inference Similarity for Non-IID Data Distribution}, 
  year={2023},
  volume={4},
  number={},
  pages={109-120},
  doi={10.1109/OJCS.2023.3262203}}





@article{mahdavi2020-APFL,
  author    = {Yuyang Deng and
               Mohammad Mahdi Kamani and
               Mehrdad Mahdavi},
  title     = {Adaptive Personalized Federated Learning},
  journal   = {CoRR},
  volume    = {abs/2003.13461},
  year      = {2020},
  url       = {https://arxiv.org/abs/2003.13461},
}




@article{Navarro-ICLR-2021,
  author    = {Durmus Alp Emre Acar and
               Yue Zhao and
               Ramon Matas Navarro and
               Matthew Mattina and
               Paul N. Whatmough and
               Venkatesh Saligrama},
  title     = {Federated Learning Based on Dynamic Regularization},
  journal   = {International Conference on Learning Representations},
  year      = {2021},
}




@article{li2018federated,
  title={Federated optimization in heterogeneous networks},
  author={Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
  journal={arXiv preprint arXiv:1812.06127},
  year={2018}
}







@article{Federated-Distillation-2018,
  author    = {Eunjeong Jeong and
               Seungeun Oh and
               Hyesung Kim and
               Jihong Park and
               Mehdi Bennis and
               Seong{-}Lyun Kim},
  title     = {Communication-Efficient On-Device Machine Learning: Federated Distillation
               and Augmentation under Non-IID Private Data},
  journal   = {CoRR},
  volume    = {abs/1811.11479},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.11479},
}


@article{Federated-Learning-via-Synthetic-Data-2020,
  author    = {Jack Goetz and
               Ambuj Tewari},
  title     = {Federated Learning via Synthetic Data},
  journal   = {CoRR},
  volume    = {abs/2008.04489},
  year      = {2020},
  url       = {https://arxiv.org/abs/2008.04489},

}






























@article{Brown-2019,
  author    = {Tzu{-}Ming Harry Hsu and
               Hang Qi and
               Matthew Brown},
  title     = {Measuring the Effects of Non-Identical Data Distribution for Federated
               Visual Classification},
  journal   = {CoRR},
  volume    = {abs/1909.06335},
  year      = {2019},
}










@misc{chen_conv-adapter_2022,
	title = {Conv-{Adapter}: {Exploring} {Parameter} {Efficient} {Transfer} {Learning} for {ConvNets}},
	shorttitle = {Conv-{Adapter}},
	url = {http://arxiv.org/abs/2208.07463},
	abstract = {While parameter efficient tuning (PET) methods have shown great potential with transformer architecture on Natural Language Processing (NLP) tasks, their effectiveness is still under-studied with large-scale ConvNets on Computer Vision (CV) tasks. This paper proposes Conv-Adapter, a PET module designed for ConvNets. Conv-Adapter is light-weight, domain-transferable, and architecture-agnostic with generalized performance on different tasks. When transferring on downstream tasks, Conv-Adapter learns tasks-specific feature modulation to the intermediate representations of backbone while keeping the pre-trained parameters frozen. By introducing only a tiny amount of learnable parameters, e.g., only 3.5\% full fine-tuning parameters of ResNet50, Conv-Adapter outperforms previous PET baseline methods and achieves comparable or surpasses the performance of full fine-tuning on 23 classification tasks of various domains. It also presents superior performance on few-shot classifications, with an average margin of 3.39\%. Beyond classification, Conv-Adapter can generalize to detection and segmentation tasks with more than 50\% reduction of parameters but comparable performance to the traditional full fine-tuning.},
	urldate = {2022-08-30},
	publisher = {arXiv},
	author = {Chen, Hao and Tao, Ran and Zhang, Han and Wang, Yidong and Ye, Wei and Wang, Jindong and Hu, Guosheng and Savvides, Marios},
	month = aug,
	year = {2022},
	note = {arXiv:2208.07463 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@misc{zheng_prompt_2022,
	title = {Prompt {Vision} {Transformer} for {Domain} {Generalization}},
	url = {http://arxiv.org/abs/2208.08914},
	abstract = {Though vision transformers (ViTs) have exhibited impressive ability for representation learning, we empirically find that they cannot generalize well to unseen domains with previous domain generalization algorithms. In this paper, we propose a novel approach DoPrompt based on prompt learning to embed the knowledge of source domains in domain prompts for target domain prediction. Specifically, domain prompts are prepended before ViT input tokens from the corresponding source domain. Each domain prompt learns domain-specific knowledge efficiently since it is optimized only for one domain. Meanwhile, we train a prompt adapter to produce a suitable prompt for each input image based on the learned source domain prompts. At test time, the adapted prompt generated by the prompt adapter can exploit the similarity between the feature of the out-of-domain image and source domains to properly integrate the source domain knowledge. Extensive experiments are conducted on four benchmark datasets. Our approach achieves 1.4\% improvements in the averaged accuracy, which is 3.5 times the improvement of the state-of-the-art algorithm with a ViT backbone.},
	urldate = {2022-08-30},
	publisher = {arXiv},
	author = {Zheng, Zangwei and Yue, Xiangyu and Wang, Kai and You, Yang},
	month = aug,
	year = {2022},
	note = {arXiv:2208.08914 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@misc{bahng_exploring_2022,
	title = {Exploring {Visual} {Prompts} for {Adapting} {Large}-{Scale} {Models}},
	url = {http://arxiv.org/abs/2203.17274},
	abstract = {We investigate the efficacy of visual prompting to adapt large-scale models in vision. Following the recent approach from prompt tuning and adversarial reprogramming, we learn a single image perturbation such that a frozen model prompted with this perturbation performs a new task. Through comprehensive experiments, we demonstrate that visual prompting is particularly effective for CLIP and robust to distribution shift, achieving performance competitive with standard linear probes. We further analyze properties of the downstream dataset, prompt design, and output transformation in regard to adaptation performance. The surprising effectiveness of visual prompting provides a new perspective on adapting pre-trained models in vision. Code is available at http://hjbahng.github.io/visual\_prompting .},
	urldate = {2022-08-30},
	publisher = {arXiv},
	author = {Bahng, Hyojin and Jahanian, Ali and Sankaranarayanan, Swami and Isola, Phillip},
	month = jun,
	year = {2022},
	note = {arXiv:2203.17274 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@techreport{guo_promptfl_2022,
	title = {{PromptFL}: {Let} {Federated} {Participants} {Cooperatively} {Learn} {Prompts} {Instead} of {Models} -- {Federated} {Learning} in {Age} of {Foundation} {Model}},
	shorttitle = {{PromptFL}},
	url = {http://arxiv.org/abs/2208.11625},
	abstract = {Quick global aggregation of effective distributed parameters is crucial to federated learning (FL), which requires adequate bandwidth for parameters communication and sufficient user data for local training. Otherwise, FL may cost excessive training time for convergence and produce inaccurate models. In this paper, we propose a brand-new FL framework, PromptFL, that replaces the federated model training with the federated prompt training, i.e., let federated participants train prompts instead of a shared model, to simultaneously achieve the efficient global aggregation and local training on insufficient data by exploiting the power of foundation models (FM) in a distributed way. PromptFL ships an off-the-shelf FM, i.e., CLIP, to distributed clients who would cooperatively train shared soft prompts based on very few local data. Since PromptFL only needs to update the prompts instead of the whole model, both the local training and the global aggregation can be significantly accelerated. And FM trained over large scale data can provide strong adaptation capability to distributed users tasks with the trained soft prompts. We empirically analyze the PromptFL via extensive experiments, and show its superiority in terms of system feasibility, user privacy, and performance.},
	urldate = {2022-08-27},
	author = {Guo, Tao and Guo, Song and Wang, Junxiao and Xu, Wenchao},
	month = aug,
	year = {2022},
	note = {arXiv:2208.11625 [cs]
type: article},
	keywords = {Computer Science - Machine Learning},
}

@misc{xing_class-aware_2022,
	title = {Class-{Aware} {Visual} {Prompt} {Tuning} for {Vision}-{Language} {Pre}-{Trained} {Model}},
	url = {http://arxiv.org/abs/2208.08340},
	abstract = {With the emergence of large pre-trained vison-language model like CLIP, transferrable representations can be adapted to a wide range of downstream tasks via prompt tuning. Prompt tuning tries to probe the beneficial information for downstream tasks from the general knowledge stored in both the image and text encoders of the pre-trained vision-language model. A recently proposed method named Context Optimization (CoOp) introduces a set of learnable vectors as text prompt from the language side, while tuning the text prompt alone can not affect the computed visual features of the image encoder, thus leading to sub-optimal. In this paper, we propose a dual modality prompt tuning paradigm through learning text prompts and visual prompts for both the text and image encoder simultaneously. In addition, to make the visual prompt concentrate more on the target visual concept, we propose Class-Aware Visual Prompt Tuning (CAVPT), which is generated dynamically by performing the cross attention between language descriptions of template prompts and visual class token embeddings. Our method provides a new paradigm for tuning the large pre-trained vision-language model and extensive experimental results on 8 datasets demonstrate the effectiveness of the proposed method. Our code is available in the supplementary materials.},
	urldate = {2022-08-18},
	publisher = {arXiv},
	author = {Xing, Yinghui and Wu, Qirui and Cheng, De and Zhang, Shizhou and Liang, Guoqiang and Zhang, Yanning},
	month = aug,
	year = {2022},
	note = {arXiv:2208.08340 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@misc{bahng_exploring_2022-1,
	title = {Exploring {Visual} {Prompts} for {Adapting} {Large}-{Scale} {Models}},
	url = {http://arxiv.org/abs/2203.17274},
	abstract = {We investigate the efficacy of visual prompting to adapt large-scale models in vision. Following the recent approach from prompt tuning and adversarial reprogramming, we learn a single image perturbation such that a frozen model prompted with this perturbation performs a new task. Through comprehensive experiments, we demonstrate that visual prompting is particularly effective for CLIP and robust to distribution shift, achieving performance competitive with standard linear probes. We further analyze properties of the downstream dataset, prompt design, and output transformation in regard to adaptation performance. The surprising effectiveness of visual prompting provides a new perspective on adapting pre-trained models in vision. Code is available at http://hjbahng.github.io/visual\_prompting .},
	urldate = {2022-08-11},
	publisher = {arXiv},
	author = {Bahng, Hyojin and Jahanian, Ali and Sankaranarayanan, Swami and Isola, Phillip},
	month = jun,
	year = {2022},
	note = {arXiv:2203.17274 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}


@article{Rethinking-vahid-2023,
  author       = {Mahdi Morafah and
                  Saeed Vahidian and
                  Chen Chen and
                  Mubarak Shah and
                  Bill Lin},
  title        = {Rethinking Data Heterogeneity in Federated Learning: Introducing a
                  New Notion and Standard Benchmarks},
  journal      = {CoRR},
  volume       = {abs/2209.15595},
  year         = {2022},
  url          = {https://doi.org/10.48550/arXiv.2209.15595},
  doi          = {10.48550/arXiv.2209.15595},
}



@misc{kim_ocr-free_2022,
	title = {{OCR}-free {Document} {Understanding} {Transformer}},
	url = {http://arxiv.org/abs/2111.15664},
	abstract = {Understanding document images (e.g., invoices) is a core but challenging task since it requires complex functions such as reading text and a holistic understanding of the document. Current Visual Document Understanding (VDU) methods outsource the task of reading text to off-the-shelf Optical Character Recognition (OCR) engines and focus on the understanding task with the OCR outputs. Although such OCR-based approaches have shown promising performance, they suffer from 1) high computational costs for using OCR; 2) inflexibility of OCR models on languages or types of document; 3) OCR error propagation to the subsequent process. To address these issues, in this paper, we introduce a novel OCR-free VDU model named Donut, which stands for Document understanding transformer. As the first step in OCR-free VDU research, we propose a simple architecture (i.e., Transformer) with a pre-training objective (i.e., cross-entropy loss). Donut is conceptually simple yet effective. Through extensive experiments and analyses, we show a simple OCR-free VDU model, Donut, achieves state-of-the-art performances on various VDU tasks in terms of both speed and accuracy. In addition, we offer a synthetic data generator that helps the model pre-training to be flexible in various languages and domains. The code, trained model and synthetic data are available at https://github.com/clovaai/donut.},
	urldate = {2022-08-10},
	publisher = {arXiv},
	author = {Kim, Geewook and Hong, Teakgyu and Yim, Moonbin and Nam, Jeongyeon and Park, Jinyoung and Yim, Jinyeong and Hwang, Wonseok and Yun, Sangdoo and Han, Dongyoon and Park, Seunghyun},
	month = jul,
	year = {2022},
	note = {arXiv:2111.15664 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
}

@misc{qu_rethinking_2022,
	title = {Rethinking {Architecture} {Design} for {Tackling} {Data} {Heterogeneity} in {Federated} {Learning}},
	url = {http://arxiv.org/abs/2106.06047},
	abstract = {Federated learning is an emerging research paradigm enabling collaborative training of machine learning models among different organizations while keeping data private at each institution. Despite recent progress, there remain fundamental challenges such as the lack of convergence and the potential for catastrophic forgetting across real-world heterogeneous devices. In this paper, we demonstrate that self-attention-based architectures (e.g., Transformers) are more robust to distribution shifts and hence improve federated learning over heterogeneous data. Concretely, we conduct the first rigorous empirical investigation of different neural architectures across a range of federated algorithms, real-world benchmarks, and heterogeneous data splits. Our experiments show that simply replacing convolutional networks with Transformers can greatly reduce catastrophic forgetting of previous devices, accelerate convergence, and reach a better global model, especially when dealing with heterogeneous data. We release our code and pretrained models at https://github.com/Liangqiong/ViT-FL-main to encourage future exploration in robust architectures as an alternative to current research efforts on the optimization front.},
	urldate = {2022-07-25},
	publisher = {arXiv},
	author = {Qu, Liangqiong and Zhou, Yuyin and Liang, Paul Pu and Xia, Yingda and Wang, Feifei and Adeli, Ehsan and Fei-Fei, Li and Rubin, Daniel},
	month = apr,
	year = {2022},
	note = {arXiv:2106.06047 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@inproceedings{pfeiffer_adapterfusion_2021,
	address = {Online},
	title = {{AdapterFusion}: {Non}-{Destructive} {Task} {Composition} for {Transfer} {Learning}},
	shorttitle = {{AdapterFusion}},
	url = {https://aclanthology.org/2021.eacl-main.39},
	doi = {10.18653/v1/2021.eacl-main.39},
	abstract = {Sequential fine-tuning and multi-task learning are methods aiming to incorporate knowledge from multiple tasks; however, they suffer from catastrophic forgetting and difficulties in dataset balancing. To address these shortcomings, we propose AdapterFusion, a new two stage learning algorithm that leverages knowledge from multiple tasks. First, in the knowledge extraction stage we learn task specific parameters called adapters, that encapsulate the task-specific information. We then combine the adapters in a separate knowledge composition step. We show that by separating the two stages, i.e., knowledge extraction and knowledge composition, the classifier can effectively exploit the representations learned from multiple tasks in a non-destructive manner. We empirically evaluate AdapterFusion on 16 diverse NLU tasks, and find that it effectively combines various types of knowledge at different layers of the model. We show that our approach outperforms traditional strategies such as full fine-tuning as well as multi-task learning. Our code and adapters are available at AdapterHub.ml.},
	urldate = {2022-07-20},
	booktitle = {Proceedings of the 16th {Conference} of the {European} {Chapter} of the {Association} for {Computational} {Linguistics}: {Main} {Volume}},
	publisher = {Association for Computational Linguistics},
	author = {Pfeiffer, Jonas and Kamath, Aishwarya and Rücklé, Andreas and Cho, Kyunghyun and Gurevych, Iryna},
	year = {2021},
	pages = {487--503},
}

@misc{xu_layoutlmv2_2022,
	title = {{LayoutLMv2}: {Multi}-modal {Pre}-training for {Visually}-{Rich} {Document} {Understanding}},
	shorttitle = {{LayoutLMv2}},
	url = {http://arxiv.org/abs/2012.14740},
	doi = {10.48550/arXiv.2012.14740},
	abstract = {Pre-training of text and layout has proved effective in a variety of visually-rich document understanding tasks due to its effective model architecture and the advantage of large-scale unlabeled scanned/digital-born documents. We propose LayoutLMv2 architecture with new pre-training tasks to model the interaction among text, layout, and image in a single multi-modal framework. Specifically, with a two-stream multi-modal Transformer encoder, LayoutLMv2 uses not only the existing masked visual-language modeling task but also the new text-image alignment and text-image matching tasks, which make it better capture the cross-modality interaction in the pre-training stage. Meanwhile, it also integrates a spatial-aware self-attention mechanism into the Transformer architecture so that the model can fully understand the relative positional relationship among different text blocks. Experiment results show that LayoutLMv2 outperforms LayoutLM by a large margin and achieves new state-of-the-art results on a wide variety of downstream visually-rich document understanding tasks, including FUNSD (0.7895 \${\textbackslash}to\$ 0.8420), CORD (0.9493 \${\textbackslash}to\$ 0.9601), SROIE (0.9524 \${\textbackslash}to\$ 0.9781), Kleister-NDA (0.8340 \${\textbackslash}to\$ 0.8520), RVL-CDIP (0.9443 \${\textbackslash}to\$ 0.9564), and DocVQA (0.7295 \${\textbackslash}to\$ 0.8672). We made our model and code publicly available at {\textbackslash}url\{https://aka.ms/layoutlmv2\}.},
	urldate = {2022-07-11},
	publisher = {arXiv},
	author = {Xu, Yang and Xu, Yiheng and Lv, Tengchao and Cui, Lei and Wei, Furu and Wang, Guoxin and Lu, Yijuan and Florencio, Dinei and Zhang, Cha and Che, Wanxiang and Zhang, Min and Zhou, Lidong},
	month = jan,
	year = {2022},
	note = {arXiv:2012.14740 [cs]},
	keywords = {Computer Science - Computation and Language},
}

@inproceedings{xu_layoutlm_2020,
	title = {{LayoutLM}: {Pre}-training of {Text} and {Layout} for {Document} {Image} {Understanding}},
	shorttitle = {{LayoutLM}},
	url = {http://arxiv.org/abs/1912.13318},
	doi = {10.1145/3394486.3403172},
	abstract = {Pre-training techniques have been verified successfully in a variety of NLP tasks in recent years. Despite the widespread use of pre-training models for NLP applications, they almost exclusively focus on text-level manipulation, while neglecting layout and style information that is vital for document image understanding. In this paper, we propose the {\textbackslash}textbf\{LayoutLM\} to jointly model interactions between text and layout information across scanned document images, which is beneficial for a great number of real-world document image understanding tasks such as information extraction from scanned documents. Furthermore, we also leverage image features to incorporate words' visual information into LayoutLM. To the best of our knowledge, this is the first time that text and layout are jointly learned in a single framework for document-level pre-training. It achieves new state-of-the-art results in several downstream tasks, including form understanding (from 70.72 to 79.27), receipt understanding (from 94.02 to 95.24) and document image classification (from 93.07 to 94.42). The code and pre-trained LayoutLM models are publicly available at {\textbackslash}url\{https://aka.ms/layoutlm\}.},
	urldate = {2022-07-11},
	booktitle = {Proceedings of the 26th {ACM} {SIGKDD} {International} {Conference} on {Knowledge} {Discovery} \& {Data} {Mining}},
	author = {Xu, Yiheng and Li, Minghao and Cui, Lei and Huang, Shaohan and Wei, Furu and Zhou, Ming},
	month = aug,
	year = {2020},
	note = {arXiv:1912.13318 [cs]},
	keywords = {Computer Science - Computation and Language},
	pages = {1192--1200},
}

@misc{pan_parameter-efficient_2022,
	title = {Parameter-{Efficient} {Image}-to-{Video} {Transfer} {Learning}},
	url = {http://arxiv.org/abs/2206.13559},
	abstract = {Capitalizing on large pre-trained models for various downstream tasks of interest have recently emerged with promising performance. Due to the ever-growing model size, the standard full fine-tuning based task adaptation strategy becomes prohibitively costly in terms of model training and storage. This has led to a new research direction in parameter-efficient transfer learning. However, existing attempts typically focus on downstream tasks from the same modality (e.g., image understanding) of the pre-trained model. This creates a limit because in some specific modalities, (e.g., video understanding) such a strong pre-trained model with sufficient knowledge is less or not available. In this work, we investigate such a novel cross-modality transfer learning setting, namely parameter-efficient image-to-video transfer learning. To solve this problem, we propose a new Spatio-Temporal Adapter (ST-Adapter) for parameter-efficient fine-tuning per video task. With a built-in spatio-temporal reasoning capability in a compact design, ST-Adapter enables a pre-trained image model without temporal knowledge to reason about dynamic video content at a small ({\textasciitilde}8\%) per-task parameter cost, requiring approximately 20 times fewer updated parameters compared to previous work. Extensive experiments on video action recognition tasks show that our ST-Adapter can match or even outperform the strong full fine-tuning strategy and state-of-the-art video models, whilst enjoying the advantage of parameter efficiency.},
	urldate = {2022-07-01},
	publisher = {arXiv},
	author = {Pan, Junting and Lin, Ziyi and Zhu, Xiatian and Shao, Jing and Li, Hongsheng},
	month = jun,
	year = {2022},
	note = {arXiv:2206.13559 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}


@inproceedings{fine-tuning-nlp-2022,
  author    = {Da Yu and
               Saurabh Naik and
               Arturs Backurs and
               Sivakanth Gopi and
               Huseyin A. Inan and
               Gautam Kamath and
               Janardhan Kulkarni and
               Yin Tat Lee and
               Andre Manoel and
               Lukas Wutschitz and
               Sergey Yekhanin and
               Huishuai Zhang},
  title     = {Differentially Private Fine-tuning of Language Models},
  booktitle = {The Tenth International Conference on Learning Representations, {ICLR}
               2022, Virtual Event, April 25-29, 2022},
  publisher = {OpenReview.net},
  year      = {2022},
}




@inproceedings{No-fear-heterogeneity-2021,
  author    = {Mi Luo and
               Fei Chen and
               Dapeng Hu and
               Yifan Zhang and
               Jian Liang and
               Jiashi Feng},
  title     = {No Fear of Heterogeneity: Classifier Calibration for Federated Learning with Non-IID Data},
  booktitle = {Advances in Neural Information Processing Systems, NeurIPS 2021, December 6-14},
  pages     = {5972--5984},
  year      = {2021},
}

@inproceedings{LORA-2022,
  author    = {Edward J. Hu and
               Yelong Shen and
               Phillip Wallis and
               Zeyuan Allen{-}Zhu and
               Yuanzhi Li and
               Shean Wang and
               Lu Wang and
               Weizhu Chen},
  title     = {LoRA: Low-Rank Adaptation of Large Language Models},
  booktitle = {The Tenth International Conference on Learning Representations, {ICLR}
               2022, Virtual Event, April 25-29, 2022},
  year      = {2022},
}



@misc{chen_pre-training_2022,
	title = {On {Pre}-{Training} for {Federated} {Learning}},
	url = {http://arxiv.org/abs/2206.11488},
	doi = {10.48550/arXiv.2206.11488},
	abstract = {In most of the literature on federated learning (FL), neural networks are initialized with random weights. In this paper, we present an empirical study on the effect of pre-training on FL. Specifically, we aim to investigate if pre-training can alleviate the drastic accuracy drop when clients' decentralized data are non-IID. We focus on FedAvg, the fundamental and most widely used FL algorithm. We found that pre-training does largely close the gap between FedAvg and centralized learning under non-IID data, but this does not come from alleviating the well-known model drifting problem in FedAvg's local training. Instead, how pre-training helps FedAvg is by making FedAvg's global aggregation more stable. When pre-training using real data is not feasible for FL, we propose a novel approach to pre-train with synthetic data. On various image datasets (including one for segmentation), our approach with synthetic pre-training leads to a notable gain, essentially a critical step toward scaling up federated learning for real-world applications.},
	urldate = {2022-06-29},
	publisher = {arXiv},
	author = {Chen, Hong-You and Tu, Cheng-Hao and Li, Ziwei and Shen, Han-Wei and Chao, Wei-Lun},
	month = jun,
	year = {2022},
	note = {arXiv:2206.11488 [cs]},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@misc{li_dit_2022,
	title = {{DiT}: {Self}-supervised {Pre}-training for {Document} {Image} {Transformer}},
	shorttitle = {{DiT}},
	url = {http://arxiv.org/abs/2203.02378},
	doi = {10.48550/arXiv.2203.02378},
	abstract = {Image Transformer has recently achieved significant progress for natural image understanding, either using supervised (ViT, DeiT, etc.) or self-supervised (BEiT, MAE, etc.) pre-training techniques. In this paper, we propose DiT, a self-supervised pre-trained Document Image Transformer model using large-scale unlabeled text images for Document AI tasks, which is essential since no supervised counterparts ever exist due to the lack of human labeled document images. We leverage DiT as the backbone network in a variety of vision-based Document AI tasks, including document image classification, document layout analysis, table detection as well as text detection for OCR. Experiment results have illustrated that the self-supervised pre-trained DiT model achieves new state-of-the-art results on these downstream tasks, e.g. document image classification (91.11 \${\textbackslash}rightarrow\$ 92.69), document layout analysis (91.0 \${\textbackslash}rightarrow\$ 94.9), table detection (94.23 \${\textbackslash}rightarrow\$ 96.55) and text detection for OCR (93.07 \${\textbackslash}rightarrow\$ 94.29). The code and pre-trained models are publicly available at {\textbackslash}url\{https://aka.ms/msdit\}.},
	urldate = {2022-06-28},
	publisher = {arXiv},
	author = {Li, Junlong and Xu, Yiheng and Lv, Tengchao and Cui, Lei and Zhang, Cha and Wei, Furu},
	month = apr,
	year = {2022},
	note = {arXiv:2203.02378 [cs]},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@misc{huang_layoutlmv3_2022,
	title = {{LayoutLMv3}: {Pre}-training for {Document} {AI} with {Unified} {Text} and {Image} {Masking}},
	shorttitle = {{LayoutLMv3}},
	url = {http://arxiv.org/abs/2204.08387},
	doi = {10.48550/arXiv.2204.08387},
	abstract = {Self-supervised pre-training techniques have achieved remarkable progress in Document AI. Most multimodal pre-trained models use a masked language modeling objective to learn bidirectional representations on the text modality, but they differ in pre-training objectives for the image modality. This discrepancy adds difficulty to multimodal representation learning. In this paper, we propose LayoutLMv3 to pre-train multimodal Transformers for Document AI with unified text and image masking. Additionally, LayoutLMv3 is pre-trained with a word-patch alignment objective to learn cross-modal alignment by predicting whether the corresponding image patch of a text word is masked. The simple unified architecture and training objectives make LayoutLMv3 a general-purpose pre-trained model for both text-centric and image-centric Document AI tasks. Experimental results show that LayoutLMv3 achieves state-of-the-art performance not only in text-centric tasks, including form understanding, receipt understanding, and document visual question answering, but also in image-centric tasks such as document image classification and document layout analysis. The code and models are publicly available at https://aka.ms/layoutlmv3.},
	urldate = {2022-06-28},
	publisher = {arXiv},
	author = {Huang, Yupan and Lv, Tengchao and Cui, Lei and Lu, Yutong and Wei, Furu},
	month = apr,
	year = {2022},
	note = {arXiv:2204.08387 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition},
}

@misc{luo_bi-vldoc_2022,
	title = {Bi-{VLDoc}: {Bidirectional} {Vision}-{Language} {Modeling} for {Visually}-{Rich} {Document} {Understanding}},
	shorttitle = {Bi-{VLDoc}},
	url = {http://arxiv.org/abs/2206.13155},
	abstract = {Multi-modal document pre-trained models have proven to be very effective in a variety of visually-rich document understanding (VrDU) tasks. Though existing document pre-trained models have achieved excellent performance on standard benchmarks for VrDU, the way they model and exploit the interactions between vision and language on documents has hindered them from better generalization ability and higher accuracy. In this work, we investigate the problem of vision-language joint representation learning for VrDU mainly from the perspective of supervisory signals. Specifically, a pre-training paradigm called Bi-VLDoc is proposed, in which a bidirectional vision-language supervision strategy and a vision-language hybrid-attention mechanism are devised to fully explore and utilize the interactions between these two modalities, to learn stronger cross-modal document representations with richer semantics. Benefiting from the learned informative cross-modal document representations, Bi-VLDoc significantly advances the state-of-the-art performance on three widely-used document understanding benchmarks, including Form Understanding (from 85.14\% to 93.44\%), Receipt Information Extraction (from 96.01\% to 97.84\%), and Document Classification (from 96.08\% to 97.12\%). On Document Visual QA, Bi-VLDoc achieves the state-of-the-art performance compared to previous single model methods.},
	urldate = {2022-06-28},
	publisher = {arXiv},
	author = {Luo, Chuwei and Tang, Guozhi and Zheng, Qi and Yao, Cong and Jin, Lianwen and Li, Chenliang and Xue, Yang and Si, Luo},
	month = jun,
	year = {2022},
	note = {arXiv:2206.13155 [cs]},
	keywords = {Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Multimedia},
}

@misc{zhang_dino_2022,
	title = {{DINO}: {DETR} with {Improved} {DeNoising} {Anchor} {Boxes} for {End}-to-{End} {Object} {Detection}},
	shorttitle = {{DINO}},
	url = {http://arxiv.org/abs/2203.03605},
	abstract = {We present DINO ({\textbackslash}textbf\{D\}ETR with {\textbackslash}textbf\{I\}mproved de{\textbackslash}textbf\{N\}oising anch{\textbackslash}textbf\{O\}r boxes), a state-of-the-art end-to-end object detector. \% in this paper. DINO improves over previous DETR-like models in performance and efficiency by using a contrastive way for denoising training, a mixed query selection method for anchor initialization, and a look forward twice scheme for box prediction. DINO achieves \$48.3\$AP in \$12\$ epochs and \$51.0\$AP in \$36\$ epochs on COCO with a ResNet-50 backbone and multi-scale features, yielding a significant improvement of \${\textbackslash}textbf\{+4.9\}\${\textbackslash}textbf\{AP\} and \${\textbackslash}textbf\{+2.4\}\${\textbackslash}textbf\{AP\}, respectively, compared to DN-DETR, the previous best DETR-like model. DINO scales well in both model size and data size. Without bells and whistles, after pre-training on the Objects365 dataset with a SwinL backbone, DINO obtains the best results on both COCO {\textbackslash}texttt\{val2017\} (\${\textbackslash}textbf\{63.2\}\${\textbackslash}textbf\{AP\}) and {\textbackslash}texttt\{test-dev\} ({\textbackslash}textbf\{\${\textbackslash}textbf\{63.3\}\$AP\}). Compared to other models on the leaderboard, DINO significantly reduces its model size and pre-training data size while achieving better results. Our code will be available at {\textbackslash}url\{https://github.com/IDEACVR/DINO\}.},
	urldate = {2022-06-27},
	publisher = {arXiv},
	author = {Zhang, Hao and Li, Feng and Liu, Shilong and Zhang, Lei and Su, Hang and Zhu, Jun and Ni, Lionel M. and Shum, Heung-Yeung},
	month = apr,
	year = {2022},
	note = {arXiv:2203.03605 [cs]
version: 3},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@inproceedings{li_selfdoc_2021,
	address = {Nashville, TN, USA},
	title = {{SelfDoc}: {Self}-{Supervised} {Document} {Representation} {Learning}},
	isbn = {978-1-66544-509-2},
	shorttitle = {{SelfDoc}},
	url = {https://ieeexplore.ieee.org/document/9578856/},
	doi = {10.1109/CVPR46437.2021.00560},
	abstract = {We propose SelfDoc, a task-agnostic pre-training framework for document image understanding. Because documents are multimodal and are intended for sequential reading, our framework exploits the positional, textual, and visual information of every semantically meaningful component in a document, and it models the contextualization between each block of content. Unlike existing document pre-training models, our model is coarse-grained instead of treating individual words as input, therefore avoiding an overly ﬁne-grained with excessive contextualization. Beyond that, we introduce cross-modal learning in the model pre-training phase to fully leverage multimodal information from unlabeled documents. For downstream usage, we propose a novel modality-adaptive attention mechanism for multimodal feature fusion by adaptively emphasizing language and vision signals. Our framework beneﬁts from self-supervised pre-training on documents without requiring annotations by a feature masking training strategy. It achieves superior performance on multiple downstream tasks with signiﬁcantly fewer document images used in the pre-training stage compared to previous works.},
	language = {en},
	urldate = {2022-06-21},
	booktitle = {2021 {IEEE}/{CVF} {Conference} on {Computer} {Vision} and {Pattern} {Recognition} ({CVPR})},
	publisher = {IEEE},
	author = {Li, Peizhao and Gu, Jiuxiang and Kuen, Jason and Morariu, Vlad I. and Zhao, Handong and Jain, Rajiv and Manjunatha, Varun and Liu, Hongfu},
	month = jun,
	year = {2021},
	pages = {5648--5656},
}

@techreport{gu_unified_2022,
	title = {Unified {Pretraining} {Framework} for {Document} {Understanding}},
	url = {http://arxiv.org/abs/2204.10939},
	abstract = {Document intelligence automates the extraction of information from documents and supports many business applications. Recent self-supervised learning methods on large-scale unlabeled document datasets have opened up promising directions towards reducing annotation efforts by training models with self-supervised objectives. However, most of the existing document pretraining methods are still language-dominated. We present UDoc, a new unified pretraining framework for document understanding. UDoc is designed to support most document understanding tasks, extending the Transformer to take multimodal embeddings as input. Each input element is composed of words and visual features from a semantic region of the input document image. An important feature of UDoc is that it learns a generic representation by making use of three self-supervised losses, encouraging the representation to model sentences, learn similarities, and align modalities. Extensive empirical analysis demonstrates that the pretraining procedure learns better joint representations and leads to improvements in downstream tasks.},
	urldate = {2022-06-08},
	author = {Gu, Jiuxiang and Kuen, Jason and Morariu, Vlad I. and Zhao, Handong and Barmpalios, Nikolaos and Jain, Rajiv and Nenkova, Ani and Sun, Tong},
	month = apr,
	year = {2022},
	note = {arXiv:2204.10939 [cs]
type: article},
	keywords = {Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition},
}



@article{he_ssfl_2021,
	title = {{SSFL}: {Tackling} {Label} {Deficiency} in {Federated} {Learning} via {Personalized} {Self}-{Supervision}},
	shorttitle = {{SSFL}},
	url = {http://arxiv.org/abs/2110.02470},
	abstract = {Federated Learning (FL) is transforming the ML training ecosystem from a centralized over-the-cloud setting to distributed training over edge devices in order to strengthen data privacy. An essential but rarely studied challenge in FL is label deficiency at the edge. This problem is even more pronounced in FL compared to centralized training due to the fact that FL users are often reluctant to label their private data. Furthermore, due to the heterogeneous nature of the data at edge devices, it is crucial to develop personalized models. In this paper we propose self-supervised federated learning (SSFL), a unified self-supervised and personalized federated learning framework, and a series of algorithms under this framework which work towards addressing these challenges. First, under the SSFL framework, we demonstrate that the standard FedAvg algorithm is compatible with recent breakthroughs in centralized self-supervised learning such as SimSiam networks. Moreover, to deal with data heterogeneity at the edge devices in this framework, we have innovated a series of algorithms that broaden existing supervised personalization algorithms into the setting of self-supervised learning. We further propose a novel personalized federated self-supervised learning algorithm, Per-SSFL, which balances personalization and consensus by carefully regulating the distance between the local and global representations of data. To provide a comprehensive comparative analysis of all proposed algorithms, we also develop a distributed training system and related evaluation protocol for SSFL. Our findings show that the gap of evaluation accuracy between supervised learning and unsupervised learning in FL is both small and reasonable. The performance comparison indicates the representation regularization-based personalization method is able to outperform other variants.},
	urldate = {2022-05-05},
	journal = {arXiv:2110.02470 [cs]},
	author = {He, Chaoyang and Yang, Zhengyu and Mushtaq, Erum and Lee, Sunwoo and Soltanolkotabi, Mahdi and Avestimehr, Salman},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.02470},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Machine Learning},
}

@inproceedings{shome_fedaffect_2021,
	address = {Montreal, BC, Canada},
	title = {{FedAffect}: {Few}-shot federated learning for facial expression recognition},
	isbn = {978-1-66540-191-3},
	shorttitle = {{FedAffect}},
	url = {https://ieeexplore.ieee.org/document/9607387/},
	doi = {10.1109/ICCVW54120.2021.00463},
	abstract = {Annotation of large-scale facial expression datasets in the real world is a major challenge because of privacy concerns of the individuals due to which traditional supervised learning approaches won’t scale. Moreover, training models on large curated datasets often leads to dataset bias which reduces generalizability for real world use. Federated learning is a recent paradigm for training models collaboratively with decentralized private data on user devices. In this paper, we propose a few-shot federated learning framework which utilizes few samples of labeled private facial expression data to train local models in each training round and aggregates all the local model weights in the central server to get a globally optimal model. In addition, as the user devices are a large source of unlabeled data, we design a federated learning based self-supervised method to disjointly update the feature extractor network on unlabeled private facial data in order to learn robust and diverse face representations. Experimental results by testing the globally trained model on benchmark datasets (FER-2013 and FERG) show comparable performance with state of the art centralized approaches. To the best of author’s knowledge, this is the first work on few-shot federated learning for facial expression recognition.},
	language = {en},
	urldate = {2022-05-04},
	booktitle = {2021 {IEEE}/{CVF} {International} {Conference} on {Computer} {Vision} {Workshops} ({ICCVW})},
	publisher = {IEEE},
	author = {Shome, Debaditya and Kar, T.},
	month = oct,
	year = {2021},
	pages = {4151--4158},
}

@article{varno_minimizing_2022,
	title = {Minimizing {Client} {Drift} in {Federated} {Learning} via {Adaptive} {Bias} {Estimation}},
	url = {http://arxiv.org/abs/2204.13170},
	abstract = {In Federated Learning a number of clients collaborate to train a model without sharing their data. Client models are optimized locally and are communicated through a central hub called server. A major challenge is to deal with heterogeneity among clients' data which causes the local optimization to drift away with respect to the global objective. In order to estimate and therefore remove this drift, variance reduction techniques have been incorporated into Federated Learning optimization recently. However, the existing solutions propagate the error of their estimations, throughout the optimization trajectory which leads to inaccurate approximations of the clients' drift and ultimately failure to remove them properly. In this paper, we address this issue by introducing an adaptive algorithm that efficiently reduces clients' drift. Compared to the previous works on adapting variance reduction to Federated Learning, our approach uses less or the same level of communication bandwidth, computation or memory. Additionally, it addresses the instability problem--prevalent in prior work, caused by increasing norm of the estimates which makes our approach a much more practical solution for large scale Federated Learning settings. Our experimental results demonstrate that the proposed algorithm converges significantly faster and achieves higher accuracy compared to the baselines in an extensive set of Federated Learning benchmarks.},
	urldate = {2022-05-04},
	journal = {arXiv:2204.13170 [cs]},
	author = {Varno, Farshid and Saghayi, Marzie and Rafiee, Laya and Gupta, Sharut and Matwin, Stan and Havaei, Mohammad},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.13170},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning, Computer Science - Multiagent Systems},
}

@article{danecek_emoca_2022,
	title = {{EMOCA}: {Emotion} {Driven} {Monocular} {Face} {Capture} and {Animation}},
	shorttitle = {{EMOCA}},
	url = {http://arxiv.org/abs/2204.11312},
	abstract = {As 3D facial avatars become more widely used for communication, it is critical that they faithfully convey emotion. Unfortunately, the best recent methods that regress parametric 3D face models from monocular images are unable to capture the full spectrum of facial expression, such as subtle or extreme emotions. We find the standard reconstruction metrics used for training (landmark reprojection error, photometric error, and face recognition loss) are insufficient to capture high-fidelity expressions. The result is facial geometries that do not match the emotional content of the input image. We address this with EMOCA (EMOtion Capture and Animation), by introducing a novel deep perceptual emotion consistency loss during training, which helps ensure that the reconstructed 3D expression matches the expression depicted in the input image. While EMOCA achieves 3D reconstruction errors that are on par with the current best methods, it significantly outperforms them in terms of the quality of the reconstructed expression and the perceived emotional content. We also directly regress levels of valence and arousal and classify basic expressions from the estimated 3D face parameters. On the task of in-the-wild emotion recognition, our purely geometric approach is on par with the best image-based methods, highlighting the value of 3D geometry in analyzing human behavior. The model and code are publicly available at https://emoca.is.tue.mpg.de.},
	urldate = {2022-04-27},
	journal = {arXiv:2204.11312 [cs]},
	author = {Danecek, Radek and Black, Michael J. and Bolkart, Timo},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.11312},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{rame_fishr_2021,
	title = {Fishr: {Invariant} {Gradient} {Variances} for {Out}-of-distribution {Generalization}},
	shorttitle = {Fishr},
	url = {http://arxiv.org/abs/2109.02934},
	abstract = {Learning robust models that generalize well under changes in the data distribution is critical for real-world applications. To this end, there has been a growing surge of interest to learn simultaneously from multiple training domains -- while enforcing different types of invariance across those domains. Yet, all existing approaches fail to show systematic benefits under controlled evaluation protocols. In this paper, we introduce a new regularization -- named Fishr -- that enforces domain invariance in the space of the gradients of the loss: specifically, the domain-level variances of gradients are matched across training domains. Our approach is based on the close relations between the gradient covariance, the Fisher Information and the Hessian of the loss: in particular, we show that Fishr eventually aligns the domain-level loss landscapes locally around the final weights. Extensive experiments demonstrate the effectiveness of Fishr for out-of-distribution generalization. Notably, Fishr improves the state of the art on the DomainBed benchmark and performs consistently better than Empirical Risk Minimization. The code is released at https://github.com/alexrame/fishr.},
	urldate = {2022-04-20},
	journal = {arXiv:2109.02934 [cs]},
	author = {Rame, Alexandre and Dancette, Corentin and Cord, Matthieu},
	month = oct,
	year = {2021},
	note = {arXiv: 2109.02934},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{zheng_poster_2022,
	title = {{POSTER}: {A} {Pyramid} {Cross}-{Fusion} {Transformer} {Network} for {Facial} {Expression} {Recognition}},
	shorttitle = {{POSTER}},
	url = {http://arxiv.org/abs/2204.04083},
	abstract = {Facial Expression Recognition (FER) has received increasing interest in the computer vision community. As a challenging task, there are three key issues especially prevalent in FER: inter-class similarity, intra-class discrepancy, and scale sensitivity. Existing methods typically address some of these issues, but do not tackle them all in a unified framework. Therefore, in this paper, we propose a two-stream Pyramid crOss-fuSion TransformER network (POSTER) that aims to holistically solve these issues. Specifically, we design a transformer-based cross-fusion paradigm that enables effective collaboration of facial landmark and direct image features to maximize proper attention to salient facial regions. Furthermore, POSTER employs a pyramid structure to promote scale invariance. Extensive experimental results demonstrate that our POSTER outperforms SOTA methods on RAF-DB with 92.05\%, FERPlus with 91.62\%, AffectNet (7 cls) with 67.31\%, and AffectNet (8 cls) with 63.34\%, respectively.},
	language = {en},
	urldate = {2022-04-20},
	journal = {arXiv:2204.04083 [cs]},
	author = {Zheng, Ce and Mendieta, Matias and Chen, Chen},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.04083},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@article{zheng_poster_2022-1,
	title = {{POSTER}: {A} {Pyramid} {Cross}-{Fusion} {Transformer} {Network} for {Facial} {Expression} {Recognition}},
	shorttitle = {{POSTER}},
	url = {http://arxiv.org/abs/2204.04083},
	abstract = {Facial Expression Recognition (FER) has received increasing interest in the computer vision community. As a challenging task, there are three key issues especially prevalent in FER: inter-class similarity, intra-class discrepancy, and scale sensitivity. Existing methods typically address some of these issues, but do not tackle them all in a unified framework. Therefore, in this paper, we propose a two-stream Pyramid crOss-fuSion TransformER network (POSTER) that aims to holistically solve these issues. Specifically, we design a transformer-based cross-fusion paradigm that enables effective collaboration of facial landmark and direct image features to maximize proper attention to salient facial regions. Furthermore, POSTER employs a pyramid structure to promote scale invariance. Extensive experimental results demonstrate that our POSTER outperforms SOTA methods on RAF-DB with 92.05\%, FERPlus with 91.62\%, AffectNet (7 cls) with 67.31\%, and AffectNet (8 cls) with 63.34\%, respectively.},
	language = {en},
	urldate = {2022-04-20},
	journal = {arXiv:2204.04083 [cs]},
	author = {Zheng, Ce and Mendieta, Matias and Chen, Chen},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.04083},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@misc{noauthor_exit_nodate,
	title = {Exit {Exam}},
	url = {https://www.overleaf.com/project/624a5b9b3873854a45b15d80},
	abstract = {An online LaTeX editor that’s easy to use. No installation, real-time collaboration, version control, hundreds of LaTeX templates, and more.},
	language = {en},
	urldate = {2022-04-14},
}

@article{li_universal_2022,
	title = {Universal {Representations}: {A} {Unified} {Look} at {Multiple} {Task} and {Domain} {Learning}},
	shorttitle = {Universal {Representations}},
	url = {http://arxiv.org/abs/2204.02744},
	abstract = {We propose a unified look at jointly learning multiple vision tasks and visual domains through universal representations, a single deep neural network. Learning multiple problems simultaneously involves minimizing a weighted sum of multiple loss functions with different magnitudes and characteristics and thus results in unbalanced state of one loss dominating the optimization and poor results compared to learning a separate model for each problem. To this end, we propose distilling knowledge of multiple task/domain-specific networks into a single deep neural network after aligning its representations with the task/domain-specific ones through small capacity adapters. We rigorously show that universal representations achieve state-of-the-art performances in learning of multiple dense prediction problems in NYU-v2 and Cityscapes, multiple image classification problems from diverse domains in Visual Decathlon Dataset and cross-domain few-shot learning in MetaDataset. Finally we also conduct multiple analysis through ablation and qualitative studies.},
	urldate = {2022-04-13},
	journal = {arXiv:2204.02744 [cs]},
	author = {Li, Wei-Hong and Liu, Xialei and Bilen, Hakan},
	month = apr,
	year = {2022},
	note = {arXiv: 2204.02744},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}




@article{wang_field_2021,
	title = {A {Field} {Guide} to {Federated} {Optimization}},
	url = {http://arxiv.org/abs/2107.06917},
	abstract = {Federated learning and analytics are a distributed approach for collaboratively learning models (or statistics) from decentralized data, motivated by and designed for privacy protection. The distributed learning process can be formulated as solving federated optimization problems, which emphasize communication eﬃciency, data heterogeneity, compatibility with privacy and system requirements, and other constraints that are not primary considerations in other problem settings. This paper provides recommendations and guidelines on formulating, designing, evaluating and analyzing federated optimization algorithms through concrete examples and practical implementation, with a focus on conducting eﬀective simulations to infer real-world performance. The goal of this work is not to survey the current literature, but to inspire researchers and practitioners to design federated learning algorithms that can be used in various practical applications.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2107.06917 [cs]},
	author = {Wang, Jianyu and Charles, Zachary and Xu, Zheng and Joshi, Gauri and McMahan, H. Brendan and Arcas, Blaise Aguera y and Al-Shedivat, Maruan and Andrew, Galen and Avestimehr, Salman and Daly, Katharine and Data, Deepesh and Diggavi, Suhas and Eichner, Hubert and Gadhikar, Advait and Garrett, Zachary and Girgis, Antonious M. and Hanzely, Filip and Hard, Andrew and He, Chaoyang and Horvath, Samuel and Huo, Zhouyuan and Ingerman, Alex and Jaggi, Martin and Javidi, Tara and Kairouz, Peter and Kale, Satyen and Karimireddy, Sai Praneeth and Konecny, Jakub and Koyejo, Sanmi and Li, Tian and Liu, Luyang and Mohri, Mehryar and Qi, Hang and Reddi, Sashank J. and Richtarik, Peter and Singhal, Karan and Smith, Virginia and Soltanolkotabi, Mahdi and Song, Weikang and Suresh, Ananda Theertha and Stich, Sebastian U. and Talwalkar, Ameet and Wang, Hongyi and Woodworth, Blake and Wu, Shanshan and Yu, Felix X. and Yuan, Honglin and Zaheer, Manzil and Zhang, Mi and Zhang, Tong and Zheng, Chunxiang and Zhu, Chen and Zhu, Wennan},
	month = jul,
	year = {2021},
	note = {arXiv: 2107.06917},
	keywords = {Computer Science - Machine Learning},
}

@article{yang_federated_2022,
	title = {Federated and {Generalized} {Person} {Re}-identification through {Domain} and {Feature} {Hallucinating}},
	url = {http://arxiv.org/abs/2203.02689},
	abstract = {In this paper, we study the problem of federated domain generalization (FedDG) for person reidentiﬁcation (re-ID), which aims to learn a generalized model with multiple decentralized labeled source domains. An empirical method (FedAvg) trains local models individually and averages them to obtain the global model for further local ﬁne-tuning or deploying in unseen target domains. One drawback of FedAvg is neglecting the data distributions of other clients during local training, making the local model overﬁt local data and producing a poorly-generalized global model. To solve this problem, we propose a novel method, called “Domain and Feature Hallucinating (DFH)”, to produce diverse features for learning generalized local and global models. Speciﬁcally, after each model aggregation process, we share the Domain-level Feature Statistics (DFS) among different clients without violating data privacy. During local training, the DFS are used to synthesize novel domain statistics with the proposed domain hallucinating, which is achieved by re-weighting DFS with random weights. Then, we propose feature hallucinating to diversify local features by scaling and shifting them to the distribution of the obtained novel domain. The synthesized novel features retain the original pair-wise similarities, enabling us to utilize them to optimize the model in a supervised manner. Extensive experiments verify that the proposed DFH can effectively improve the generalization ability of the global model. Our method achieves the state-of-the-art performance for FedDG on four large-scale re-ID benchmarks.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2203.02689 [cs]},
	author = {Yang, Fengxiang and Zhong, Zhun and Luo, Zhiming and Li, Shaozi and Sebe, Nicu},
	month = mar,
	year = {2022},
	note = {arXiv: 2203.02689},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}












@article{zhuang_towards_2021,
	title = {Towards {Unsupervised} {Domain} {Adaptation} for {Deep} {Face} {Recognition} under {Privacy} {Constraints} via {Federated} {Learning}},
	url = {http://arxiv.org/abs/2105.07606},
	abstract = {Unsupervised domain adaptation has been widely adopted to generalize models for unlabeled data in a target domain, given labeled data in a source domain, whose data distributions differ from the target domain. However, existing works are inapplicable to face recognition under privacy constraints because they require sharing sensitive face images between two domains. To address this problem, we propose a novel unsupervised federated face recognition approach (FedFR). FedFR improves the performance in the target domain by iteratively aggregating knowledge from the source domain through federated learning. It protects data privacy by transferring models instead of raw data between domains. Besides, we propose a new domain constraint loss (DCL) to regularize source domain training. DCL suppresses the data volume dominance of the source domain. We also enhance a hierarchical clustering algorithm to predict pseudo labels for the unlabeled target domain accurately. To this end, FedFR forms an end-to-end training pipeline: (1) pre-train in the source domain; (2) predict pseudo labels by clustering in the target domain; (3) conduct domain-constrained federated learning across two domains. Extensive experiments and analysis on two newly constructed benchmarks demonstrate the effectiveness of FedFR. It outperforms the baseline and classic methods in the target domain by over 4\% on the more realistic benchmark. We believe that FedFR will shed light on applying federated learning to more computer vision tasks under privacy constraints.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2105.07606 [cs]},
	author = {Zhuang, Weiming and Gan, Xin and Wen, Yonggang and Zhang, Xuesen and Zhang, Shuai and Yi, Shuai},
	month = may,
	year = {2021},
	note = {arXiv: 2105.07606},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
}

@article{zhuang_performance_2020,
	title = {Performance {Optimization} for {Federated} {Person} {Re}-identification via {Benchmark} {Analysis}},
	url = {http://arxiv.org/abs/2008.11560},
	doi = {10.1145/3394171.3413814},
	abstract = {Federated learning is a privacy-preserving machine learning technique that learns a shared model across decentralized clients. It can alleviate privacy concerns of personal re-identification, an important computer vision task. In this work, we implement federated learning to person re-identification (FedReID) and optimize its performance affected by statistical heterogeneity in the realworld scenario. We first construct a new benchmark to investigate the performance of FedReID. This benchmark consists of (1) nine datasets with different volumes sourced from different domains to simulate the heterogeneous situation in reality, (2) two federated scenarios, and (3) an enhanced federated algorithm for FedReID. The benchmark analysis shows that the client-edge-cloud architecture, represented by the federated-by-dataset scenario, has better performance than client-server architecture in FedReID. It also reveals the bottlenecks of FedReID under the real-world scenario, including poor performance of large datasets caused by unbalanced weights in model aggregation and challenges in convergence. Then we propose two optimization methods: (1) To address the unbalanced weight problem, we propose a new method to dynamically change the weights according to the scale of model changes in clients in each training round; (2) To facilitate convergence, we adopt knowledge distillation to refine the server model with knowledge generated from client models on a public dataset. Experiment results demonstrate that our strategies can achieve much better convergence with superior performance on all datasets. We believe that our work will inspire the community to further explore the implementation of federated learning on more computer vision tasks in real-world scenarios.},
	language = {en},
	urldate = {2022-03-20},
	journal = {Proceedings of the 28th ACM International Conference on Multimedia},
	author = {Zhuang, Weiming and Wen, Yonggang and Zhang, Xuesen and Gan, Xin and Yin, Daiying and Zhou, Dongzhan and Zhang, Shuai and Yi, Shuai},
	month = oct,
	year = {2020},
	note = {arXiv: 2008.11560},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
	pages = {955--963},
}

@article{wu_decentralised_2021,
	title = {Decentralised {Learning} from {Independent} {Multi}-{Domain} {Labels} for {Person} {Re}-{Identification}},
	url = {http://arxiv.org/abs/2006.04150},
	abstract = {Deep learning has been successful for many computer vision tasks due to the availability of shared and centralised large-scale training data. However, increasing awareness of privacy concerns poses new challenges to deep learning, especially for human subject related recognition such as person re-identiﬁcation (Re-ID). In this work, we solve the Re-ID problem by decentralised learning from non-shared private training data distributed at multiple user sites of independent multi-domain label spaces. We propose a novel paradigm called Federated Person Re-Identiﬁcation (FedReID) to construct a generalisable global model (a central server) by simultaneously learning with multiple privacy-preserved local models (local clients). Speciﬁcally, each local client receives global model updates from the server and trains a local model using its local data independent from all the other clients. Then, the central server aggregates transferrable local model updates to construct a generalisable global feature embedding model without accessing local data so to preserve local privacy. This client-server collaborative learning process is iteratively performed under privacy control, enabling FedReID to realise decentralised learning without sharing distributed data nor collecting any centralised data. Extensive experiments on ten Re-ID benchmarks show that FedReID achieves compelling generalisation performance beyond any locally trained models without using shared training data, whilst inherently protects the privacy of each local client. This is uniquely advantageous over contemporary Re-ID methods.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2006.04150 [cs]},
	author = {Wu, Guile and Gong, Shaogang},
	month = jul,
	year = {2021},
	note = {arXiv: 2006.04150},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{raza_lightweight_2021,
	title = {Lightweight {Transformer} in {Federated} {Setting} for {Human} {Activity} {Recognition}},
	url = {http://arxiv.org/abs/2110.00244},
	abstract = {Human Activity Recognition (HAR) has been a challenging problem yet it needs to be solved. It will mainly be used for eldercare and healthcare as an assistive technology when ensemble with other technologies like Internet of Things(IoT). HAR can be achieved with the help of sensors, smartphones or images. Deep neural network techniques like artiﬁcial neural networks, convolutional neural networks and recurrent neural networks have been used in HAR, both in centralized and federated setting. However,these techniques have certain limitations. RNNs have limitation of parallelization, CNNS have the limitation of sequence length and they are computationally expensive. In this paper, to address the state of art challenges, we present a inertial sensors-based novel one patch transformer which gives the best of both RNNs and CNNs for Human activity recognition. We also design a testbed to collect real-time human activity data. The data collected is further used to train and test the proposed transformer. With the help of experiments, we show that the proposed transformer outperforms the state of art CNN and RNN based classiﬁers, both in federated and centralized setting. Moreover, the proposed transformer is computationally inexpensive as it uses very few parameter compared to the existing state of art CNN and RNN based classiﬁer. Thus its more suitable for federated learning as it provides less communication and computational cost.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2110.00244 [cs]},
	author = {Raza, Ali and Tran, Kim Phuc and Koehl, Ludovic and Li, Shujun and Zeng, Xianyi and Benzaidi, Khaled},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.00244},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@article{zhuang_performance_2020-1,
	title = {Performance {Optimization} for {Federated} {Person} {Re}-identification via {Benchmark} {Analysis}},
	url = {http://arxiv.org/abs/2008.11560},
	doi = {10.1145/3394171.3413814},
	abstract = {Federated learning is a privacy-preserving machine learning technique that learns a shared model across decentralized clients. It can alleviate privacy concerns of personal re-identification, an important computer vision task. In this work, we implement federated learning to person re-identification (FedReID) and optimize its performance affected by statistical heterogeneity in the realworld scenario. We first construct a new benchmark to investigate the performance of FedReID. This benchmark consists of (1) nine datasets with different volumes sourced from different domains to simulate the heterogeneous situation in reality, (2) two federated scenarios, and (3) an enhanced federated algorithm for FedReID. The benchmark analysis shows that the client-edge-cloud architecture, represented by the federated-by-dataset scenario, has better performance than client-server architecture in FedReID. It also reveals the bottlenecks of FedReID under the real-world scenario, including poor performance of large datasets caused by unbalanced weights in model aggregation and challenges in convergence. Then we propose two optimization methods: (1) To address the unbalanced weight problem, we propose a new method to dynamically change the weights according to the scale of model changes in clients in each training round; (2) To facilitate convergence, we adopt knowledge distillation to refine the server model with knowledge generated from client models on a public dataset. Experiment results demonstrate that our strategies can achieve much better convergence with superior performance on all datasets. We believe that our work will inspire the community to further explore the implementation of federated learning on more computer vision tasks in real-world scenarios.},
	language = {en},
	urldate = {2022-03-20},
	journal = {Proceedings of the 28th ACM International Conference on Multimedia},
	author = {Zhuang, Weiming and Wen, Yonggang and Zhang, Xuesen and Gan, Xin and Yin, Daiying and Zhou, Dongzhan and Zhang, Shuai and Yi, Shuai},
	month = oct,
	year = {2020},
	note = {arXiv: 2008.11560},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
	pages = {955--963},
}




@article{jaggi-ensemble-2020,
  author    = {Tao Lin and
               Lingjing Kong and
               Sebastian U. Stich and
               Martin Jaggi},
  title     = {Ensemble Distillation for Robust Model Fusion in Federated Learning},
  journal   = {CoRR},
  volume    = {abs/2006.07242},
  year      = {2020},
}






@article{curr-vahid,
  author       = {Saeed Vahidian and
                  Sreevatsank Kadaveru and
                  Woonjoon Baek and
                  Weijia Wang and
                  Vyacheslav Kungurtsev and
                  Chen Chen and
                  Mubarak Shah and
                  Bill Lin},
  title        = {When Do Curricula Work in Federated Learning?},
  journal      = {CoRR},
  volume       = {abs/2212.12712},
  year         = {2022},
  url          = {https://doi.org/10.48550/arXiv.2212.12712},
  doi          = {10.48550/arXiv.2212.12712},
}




@article{bai_federated_2021,
	title = {Federated {Face} {Recognition}},
	url = {http://arxiv.org/abs/2105.02501},
	abstract = {Face recognition has been extensively studied in computer vision and artiﬁcial intelligence communities in recent years. An important issue of face recognition is data privacy, which receives more and more public concerns. As a common privacy-preserving technique, Federated Learning is proposed to train a model cooperatively without sharing data between parties. However, as far as we know, it has not been successfully applied in face recognition. This paper proposes a framework named FedFace to innovate federated learning for face recognition. Speciﬁcally, FedFace relies on two major innovative algorithms, Partially Federated Momentum (PFM) and Federated Validation (FV). PFM locally applies an estimated equivalent global momentum to approximating the centralized momentum-SGD efﬁciently. FV repeatedly searches for better federated aggregating weightings via testing the aggregated models on some private validation datasets, which can improve the model’s generalization ability. The ablation study and extensive experiments validate the effectiveness of the FedFace method and show that it is comparable to or even better than the centralized baseline in performance.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2105.02501 [cs]},
	author = {Bai, Fan and Wu, Jiaxiang and Shen, Pengcheng and Li, Shaoxin and Zhou, Shuigeng},
	month = may,
	year = {2021},
	note = {arXiv: 2105.02501},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}


@article{Vahidian-federated-2021,
  title={Personalized federated learning by structured and unstructured pruning under data heterogeneity},
  author={Vahidian, Saeed and 
  Morafah, Mahdi
  and Lin, Bill},
  journal={IEEE ICDCS},
  year={2021}
}


@article{liu_federated_2022,
	title = {Federated {Remote} {Physiological} {Measurement} with {Imperfect} {Data}},
	url = {http://arxiv.org/abs/2203.05759},
	abstract = {The growing need for technology that supports remote healthcare is being acutely highlighted by an aging population and the COVID-19 pandemic. In health-related machine learning applications the ability to learn predictive models without data leaving a private device is attractive, especially when these data might contain features (e.g., photographs or videos of the body) that make identifying a subject trivial and/or the training data volume is large (e.g., uncompressed video). Camera-based remote physiological sensing facilitates scalable and low-cost measurement, but is a prime example of a task that involves analysing high bit-rate videos containing identiﬁable images and sensitive health information. Federated learning enables privacy-preserving decentralized training which has several properties beneﬁcial for camera-based sensing. We develop the ﬁrst mobile federated learning camera-based sensing system and show that it can perform competitively with traditional state-of-the-art supervised approaches. However, in the presence of corrupted data (e.g., video or label noise) from a few devices the performance of weight averaging quickly degrades. To address this, we leverage knowledge about the expected noise proﬁle within the video to intelligently adjust how the model weights are averaged on the server. Our results show that this signiﬁcantly improves upon the robustness of models even when the signal-to-noise ratio is low.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2203.05759 [cs, eess]},
	author = {Liu, Xin and Zhang, Mingchuan and Jiang, Ziheng and Patel, Shwetak and McDuff, Daniel},
	month = mar,
	year = {2022},
	note = {arXiv: 2203.05759},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Electrical Engineering and Systems Science - Image and Video Processing},
}

@article{zhang_federated_2022,
	title = {Federated {Learning} for {Internet} of {Things}: {Applications}, {Challenges}, and {Opportunities}},
	shorttitle = {Federated {Learning} for {Internet} of {Things}},
	url = {http://arxiv.org/abs/2111.07494},
	abstract = {Billions of IoT devices will be deployed in the near future, taking advantage of faster Internet speed and the possibility of orders of magnitude more endpoints brought by 5G/6G. With the growth of IoT devices, vast quantities of data that may contain users’ private information will be generated. The high communication and storage costs, mixed with privacy concerns, will increasingly challenge the traditional ecosystem of centralized over-the-cloud learning and processing for IoT platforms. Federated Learning (FL) has emerged as the most promising alternative approach to this problem. In FL, training data-driven machine learning models is an act of collaboration between multiple clients without requiring the data to be brought to a central point, hence alleviating communication and storage costs and providing a great degree of user-level privacy. However, there are still some challenges existing in the real FL system implementation on IoT networks. In this paper, we will discuss the opportunities and challenges of FL in IoT platforms, as well as how it can enable diverse IoT applications. In particular, we identify and discuss seven critical challenges of FL in IoT platforms and highlight some recent promising approaches towards addressing them.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2111.07494 [cs]},
	author = {Zhang, Tuo and Gao, Lei and He, Chaoyang and Zhang, Mi and Krishnamachari, Bhaskar and Avestimehr, Salman},
	month = mar,
	year = {2022},
	note = {arXiv: 2111.07494},
	keywords = {Computer Science - Machine Learning},
}

@inproceedings{kim_federated_2021,
	address = {Las Vegas, NV, USA},
	title = {Federated {Learning} for {Face} {Recognition}},
	isbn = {978-1-72819-766-1},
	url = {https://ieeexplore.ieee.org/document/9427748/},
	doi = {10.1109/ICCE50685.2021.9427748},
	abstract = {With the rapid development of deep learning, the accuracy of face recognition has significantly increased. However, training a face recognition model requires the collection of private data to a centralized server to obtain high performance in the desired domain. Since federated learning is a technique to train a model without collecting data to a server, it is a suitable architecture to train a face recognition model with privacysensitive face images held in personal smartphones. This study proposes strategies to apply federated learning to face recognition model training.},
	language = {en},
	urldate = {2022-03-20},
	booktitle = {2021 {IEEE} {International} {Conference} on {Consumer} {Electronics} ({ICCE})},
	publisher = {IEEE},
	author = {Kim, Jaehyeok and Park, Taehyeong and Kim, Hyorin and Kim, Suhyun},
	month = jan,
	year = {2021},
	pages = {1--2},
}

@article{shao_federated_2020,
	title = {Federated {Face} {Presentation} {Attack} {Detection}},
	url = {http://arxiv.org/abs/2005.14638},
	abstract = {Face presentation attack detection (fPAD) plays a critical role in the modern face recognition pipeline. A face presentation attack detection model with good generalization can be obtained when it is trained with face images from different input distributions and different types of spoof attacks. In reality, training data (both real face images and spoof images) are not directly shared between data owners due to legal and privacy issues. In this paper, with the motivation of circumventing this challenge, we propose Federated Face Presentation Attack Detection (FedPAD) framework. FedPAD simultaneously takes advantage of rich fPAD information available at different data owners while preserving data privacy. In the proposed framework, each data owner (referred to as data centers) locally trains its own fPAD model. A server learns a global fPAD model by iteratively aggregating model updates from all data centers without accessing private data in each of them. Once the learned global model converges, it is used for fPAD inference. We introduce the experimental setting to evaluate the proposed FedPAD framework and carry out extensive experiments to provide various insights about federated learning for fPAD.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2005.14638 [cs]},
	author = {Shao, Rui and Perera, Pramuditha and Yuen, Pong C. and Patel, Vishal M.},
	month = sep,
	year = {2020},
	note = {arXiv: 2005.14638},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{fantauzzo_feddrive_2022,
	title = {{FedDrive}: {Generalizing} {Federated} {Learning} to {Semantic} {Segmentation} in {Autonomous} {Driving}},
	shorttitle = {{FedDrive}},
	url = {http://arxiv.org/abs/2202.13670},
	abstract = {Semantic Segmentation is essential to make selfdriving vehicles autonomous, enabling them to understand their surroundings by assigning individual pixels to known categories. However, it operates on sensible data collected from the users’ cars; thus, protecting the clients’ privacy becomes a primary concern. For similar reasons, Federated Learning has been recently introduced as a new machine learning paradigm aiming to learn a global model while preserving privacy and leveraging data on millions of remote devices. Despite several efforts on this topic, no work has explicitly addressed the challenges of federated learning in semantic segmentation for driving so far. To ﬁll this gap, we propose FedDrive, a new benchmark consisting of three settings and two datasets, incorporating the real-world challenges of statistical heterogeneity and domain generalization. We benchmark state-of-the-art algorithms from the federated learning literature through an in-depth analysis, combining them with style transfer methods to improve their generalization ability. We demonstrate that correctly handling normalization statistics is crucial to deal with the aforementioned challenges. Furthermore, style transfer improves performance when dealing with signiﬁcant appearance shifts. We plan to make both the code and the benchmark publicly available to the research community.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2202.13670 [cs]},
	author = {Fantauzzo, Lidia and Fani', Eros and Caldarola, Debora and Tavera, Antonio and Cermelli, Fabio and Ciccone, Marco and Caputo, Barbara},
	month = feb,
	year = {2022},
	note = {arXiv: 2202.13670},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{hu_dynamic-aware_2022,
	title = {Dynamic-aware {Federated} {Learning} for {Face} {Forgery} {Video} {Detection}},
	issn = {2157-6904, 2157-6912},
	url = {https://dl.acm.org/doi/10.1145/3501814},
	doi = {10.1145/3501814},
	abstract = {The spread of face forgery videos causes a serious threat to information credibility, calling for efective detection algorithms to identify them. Most existing methods have assumed a shared or centralized training set. However, in practice, data may be distributed on devices of diferent enterprises that can not be centralized to share due to the security and privacy restrictions. In this paper, we propose a Federated Learning face forgery detection framework to train a global model collboratively while keeping data stay on local devices. In order to make the detection model more robust, we propose a novel InconsistencyCapture module (ICM) to capture the dynamic inconsistencies between adjacent frames of face forgery videos. The ICM contains two parallel branches. The irst branch takes the whole face of adjacent frames as input to calculate a global inconsistency representation. The second branch only focuses on the inter-frame variation of critical regions to capture the local inconsistency. To the best of our knowledge, this is the irst work to apply Federated Learning to face forgery video detection, which is trained with decentralized data. Extensive experiments show that the proposed framework achieves competitive performance compared to existing methods that are trained with centralized data, with higher-level security and privacy guarantee. CCS Concepts: · Security and privacy → Human and societal aspects of security and privacy; · Computing methodologies → Distributed computing methodologies.},
	language = {en},
	urldate = {2022-03-20},
	journal = {ACM Transactions on Intelligent Systems and Technology},
	author = {Hu, Ziheng and Xie, Hongtao and Yu, Lingyun and Gao, Xingyu and Shang, Zhihua and Zhang, Yongdong},
	month = feb,
	year = {2022},
	pages = {3501814},
}

@article{sun_decentralised_2021,
	title = {Decentralised {Person} {Re}-{Identification} with {Selective} {Knowledge} {Aggregation}},
	url = {http://arxiv.org/abs/2110.11384},
	abstract = {Existing person re-identiﬁcation (Re-ID) methods mostly follow a centralised learning paradigm which shares all training data to a collection for model learning. This paradigm is limited when data from different sources cannot be shared due to privacy concerns. To resolve this problem, two recent works [32, 41] have introduced decentralised (federated) Re-ID learning for constructing a globally generalised model (server) without any direct access to local training data nor shared data across different source domains (clients). However, these methods are poor on how to adapt the generalised model to maximise its performance on individual client domain Re-ID tasks having different Re-ID label spaces, due to a lack of understanding of data heterogeneity across domains. We call this poor ‘model personalisation’. In this work, we present a new Selective Knowledge Aggregation approach to decentralised person Re-ID to optimise the trade-off between model personalisation and generalisation. Speciﬁcally, we incorporate attentive normalisation into the normalisation layers in a deep ReID model and propose to learn local normalisation layers speciﬁc to each domain, which are decoupled from the global model aggregation in federated Re-ID learning. This helps to preserve model personalisation knowledge on each local client domain and learn instance-speciﬁc information. Further, we introduce a dual local normalisation mechanism to learn generalised normalisation layers in each local model, which are then transmitted to the global model for central aggregation. This facilitates selective knowledge aggregation on the server to construct a global generalised model for out-of-the-box deployment on unseen novel domains. Extensive experiments on eight person Re-ID datasets show that the proposed approach to decentralised Re-ID signiﬁcantly outperforms the state-of-the-art decentralised methods on both seen client domains and unseen novel domains.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2110.11384 [cs]},
	author = {Sun, Shitong and Wu, Guile and Gong, Shaogang},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.11384},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@article{kairouz_advances_2021,
	title = {Advances and {Open} {Problems} in {Federated} {Learning}},
	url = {http://arxiv.org/abs/1912.04977},
	abstract = {Federated learning (FL) is a machine learning setting where many clients (e.g. mobile devices or whole organizations) collaboratively train a model under the orchestration of a central server (e.g. service provider), while keeping the training data decentralized. FL embodies the principles of focused data collection and minimization, and can mitigate many of the systemic privacy risks and costs resulting from traditional, centralized machine learning and data science approaches. Motivated by the explosive growth in FL research, this paper discusses recent advances and presents an extensive collection of open problems and challenges.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:1912.04977 [cs, stat]},
	author = {Kairouz, Peter and others},
	month = mar,
	year = {2021},
	note = {arXiv: 1912.04977},
	keywords = {Computer Science - Cryptography and Security, Computer Science - Machine Learning, Statistics - Machine Learning},
}

@article{raza_lightweight_2021-1,
	title = {Lightweight {Transformer} in {Federated} {Setting} for {Human} {Activity} {Recognition}},
	url = {http://arxiv.org/abs/2110.00244},
	abstract = {Human Activity Recognition (HAR) has been a challenging problem yet it needs to be solved. It will mainly be used for eldercare and healthcare as an assistive technology when ensemble with other technologies like Internet of Things(IoT). HAR can be achieved with the help of sensors, smartphones or images. Deep neural network techniques like artiﬁcial neural networks, convolutional neural networks and recurrent neural networks have been used in HAR, both in centralized and federated setting. However,these techniques have certain limitations. RNNs have limitation of parallelization, CNNS have the limitation of sequence length and they are computationally expensive. In this paper, to address the state of art challenges, we present a inertial sensors-based novel one patch transformer which gives the best of both RNNs and CNNs for Human activity recognition. We also design a testbed to collect real-time human activity data. The data collected is further used to train and test the proposed transformer. With the help of experiments, we show that the proposed transformer outperforms the state of art CNN and RNN based classiﬁers, both in federated and centralized setting. Moreover, the proposed transformer is computationally inexpensive as it uses very few parameter compared to the existing state of art CNN and RNN based classiﬁer. Thus its more suitable for federated learning as it provides less communication and computational cost.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2110.00244 [cs]},
	author = {Raza, Ali and Tran, Kim Phuc and Koehl, Ludovic and Li, Shujun and Zeng, Xianyi and Benzaidi, Khaled},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.00244},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}






@article{zhang2023building,
  author       = {Jianyi Zhang and
                  Saeed Vahidian and
                  Martin Kuo and
                  Chunyuan Li and
                  Ruiyi Zhang and
                  Guoyin Wang and
                  Yiran Chen},
  title        = {Towards Building the Federated {GPT:} Federated Instruction Tuning},
  journal      = {CoRR},
  volume       = {abs/2305.05644},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2305.05644},
  doi          = {10.48550/arXiv.2305.05644},
}







@article{zhuang_performance_2020-2,
	title = {Performance {Optimization} for {Federated} {Person} {Re}-identification via {Benchmark} {Analysis}},
	url = {http://arxiv.org/abs/2008.11560},
	doi = {10.1145/3394171.3413814},
	abstract = {Federated learning is a privacy-preserving machine learning technique that learns a shared model across decentralized clients. It can alleviate privacy concerns of personal re-identification, an important computer vision task. In this work, we implement federated learning to person re-identification (FedReID) and optimize its performance affected by statistical heterogeneity in the realworld scenario. We first construct a new benchmark to investigate the performance of FedReID. This benchmark consists of (1) nine datasets with different volumes sourced from different domains to simulate the heterogeneous situation in reality, (2) two federated scenarios, and (3) an enhanced federated algorithm for FedReID. The benchmark analysis shows that the client-edge-cloud architecture, represented by the federated-by-dataset scenario, has better performance than client-server architecture in FedReID. It also reveals the bottlenecks of FedReID under the real-world scenario, including poor performance of large datasets caused by unbalanced weights in model aggregation and challenges in convergence. Then we propose two optimization methods: (1) To address the unbalanced weight problem, we propose a new method to dynamically change the weights according to the scale of model changes in clients in each training round; (2) To facilitate convergence, we adopt knowledge distillation to refine the server model with knowledge generated from client models on a public dataset. Experiment results demonstrate that our strategies can achieve much better convergence with superior performance on all datasets. We believe that our work will inspire the community to further explore the implementation of federated learning on more computer vision tasks in real-world scenarios.},
	language = {en},
	urldate = {2022-03-20},
	journal = {Proceedings of the 28th ACM International Conference on Multimedia},
	author = {Zhuang, Weiming and Wen, Yonggang and Zhang, Xuesen and Gan, Xin and Yin, Daiying and Zhou, Dongzhan and Zhang, Shuai and Yi, Shuai},
	month = oct,
	year = {2020},
	note = {arXiv: 2008.11560},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
	pages = {955--963},
}

@article{bai_federated_2021-1,
	title = {Federated {Face} {Recognition}},
	url = {http://arxiv.org/abs/2105.02501},
	abstract = {Face recognition has been extensively studied in computer vision and artiﬁcial intelligence communities in recent years. An important issue of face recognition is data privacy, which receives more and more public concerns. As a common privacy-preserving technique, Federated Learning is proposed to train a model cooperatively without sharing data between parties. However, as far as we know, it has not been successfully applied in face recognition. This paper proposes a framework named FedFace to innovate federated learning for face recognition. Speciﬁcally, FedFace relies on two major innovative algorithms, Partially Federated Momentum (PFM) and Federated Validation (FV). PFM locally applies an estimated equivalent global momentum to approximating the centralized momentum-SGD efﬁciently. FV repeatedly searches for better federated aggregating weightings via testing the aggregated models on some private validation datasets, which can improve the model’s generalization ability. The ablation study and extensive experiments validate the effectiveness of the FedFace method and show that it is comparable to or even better than the centralized baseline in performance.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2105.02501 [cs]},
	author = {Bai, Fan and Wu, Jiaxiang and Shen, Pengcheng and Li, Shaoxin and Zhou, Shuigeng},
	month = may,
	year = {2021},
	note = {arXiv: 2105.02501},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@article{liu_federated_2022-1,
	title = {Federated {Remote} {Physiological} {Measurement} with {Imperfect} {Data}},
	url = {http://arxiv.org/abs/2203.05759},
	abstract = {The growing need for technology that supports remote healthcare is being acutely highlighted by an aging population and the COVID-19 pandemic. In health-related machine learning applications the ability to learn predictive models without data leaving a private device is attractive, especially when these data might contain features (e.g., photographs or videos of the body) that make identifying a subject trivial and/or the training data volume is large (e.g., uncompressed video). Camera-based remote physiological sensing facilitates scalable and low-cost measurement, but is a prime example of a task that involves analysing high bit-rate videos containing identiﬁable images and sensitive health information. Federated learning enables privacy-preserving decentralized training which has several properties beneﬁcial for camera-based sensing. We develop the ﬁrst mobile federated learning camera-based sensing system and show that it can perform competitively with traditional state-of-the-art supervised approaches. However, in the presence of corrupted data (e.g., video or label noise) from a few devices the performance of weight averaging quickly degrades. To address this, we leverage knowledge about the expected noise proﬁle within the video to intelligently adjust how the model weights are averaged on the server. Our results show that this signiﬁcantly improves upon the robustness of models even when the signal-to-noise ratio is low.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2203.05759 [cs, eess]},
	author = {Liu, Xin and Zhang, Mingchuan and Jiang, Ziheng and Patel, Shwetak and McDuff, Daniel},
	month = mar,
	year = {2022},
	note = {arXiv: 2203.05759},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Electrical Engineering and Systems Science - Image and Video Processing},
}

@article{zhang_federated_2022,
	title = {Federated {Learning} for {Internet} of {Things}: {Applications}, {Challenges}, and {Opportunities}},
	shorttitle = {Federated {Learning} for {Internet} of {Things}},
	url = {http://arxiv.org/abs/2111.07494},
	abstract = {Billions of IoT devices will be deployed in the near future, taking advantage of faster Internet speed and the possibility of orders of magnitude more endpoints brought by 5G/6G. With the growth of IoT devices, vast quantities of data that may contain users’ private information will be generated. The high communication and storage costs, mixed with privacy concerns, will increasingly challenge the traditional ecosystem of centralized over-the-cloud learning and processing for IoT platforms. Federated Learning (FL) has emerged as the most promising alternative approach to this problem. In FL, training data-driven machine learning models is an act of collaboration between multiple clients without requiring the data to be brought to a central point, hence alleviating communication and storage costs and providing a great degree of user-level privacy. However, there are still some challenges existing in the real FL system implementation on IoT networks. In this paper, we will discuss the opportunities and challenges of FL in IoT platforms, as well as how it can enable diverse IoT applications. In particular, we identify and discuss seven critical challenges of FL in IoT platforms and highlight some recent promising approaches towards addressing them.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2111.07494 [cs]},
	author = {Zhang, Tuo and Gao, Lei and He, Chaoyang and Zhang, Mi and Krishnamachari, Bhaskar and Avestimehr, Salman},
	month = mar,
	year = {2022},
	note = {arXiv: 2111.07494},
	keywords = {Computer Science - Machine Learning},
}

@inproceedings{kim_federated_2021,
	address = {Las Vegas, NV, USA},
	title = {Federated {Learning} for {Face} {Recognition}},
	isbn = {978-1-72819-766-1},
	url = {https://ieeexplore.ieee.org/document/9427748/},
	doi = {10.1109/ICCE50685.2021.9427748},
	abstract = {With the rapid development of deep learning, the accuracy of face recognition has significantly increased. However, training a face recognition model requires the collection of private data to a centralized server to obtain high performance in the desired domain. Since federated learning is a technique to train a model without collecting data to a server, it is a suitable architecture to train a face recognition model with privacysensitive face images held in personal smartphones. This study proposes strategies to apply federated learning to face recognition model training.},
	language = {en},
	urldate = {2022-03-20},
	booktitle = {2021 {IEEE} {International} {Conference} on {Consumer} {Electronics} ({ICCE})},
	publisher = {IEEE},
	author = {Kim, Jaehyeok and Park, Taehyeong and Kim, Hyorin and Kim, Suhyun},
	month = jan,
	year = {2021},
	pages = {1--2},
}

@article{shao_federated_2020,
	title = {Federated {Face} {Presentation} {Attack} {Detection}},
	url = {http://arxiv.org/abs/2005.14638},
	abstract = {Face presentation attack detection (fPAD) plays a critical role in the modern face recognition pipeline. A face presentation attack detection model with good generalization can be obtained when it is trained with face images from different input distributions and different types of spoof attacks. In reality, training data (both real face images and spoof images) are not directly shared between data owners due to legal and privacy issues. In this paper, with the motivation of circumventing this challenge, we propose Federated Face Presentation Attack Detection (FedPAD) framework. FedPAD simultaneously takes advantage of rich fPAD information available at different data owners while preserving data privacy. In the proposed framework, each data owner (referred to as data centers) locally trains its own fPAD model. A server learns a global fPAD model by iteratively aggregating model updates from all data centers without accessing private data in each of them. Once the learned global model converges, it is used for fPAD inference. We introduce the experimental setting to evaluate the proposed FedPAD framework and carry out extensive experiments to provide various insights about federated learning for fPAD.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2005.14638 [cs]},
	author = {Shao, Rui and Perera, Pramuditha and Yuen, Pong C. and Patel, Vishal M.},
	month = sep,
	year = {2020},
	note = {arXiv: 2005.14638},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{fantauzzo_feddrive_2022,
	title = {{FedDrive}: {Generalizing} {Federated} {Learning} to {Semantic} {Segmentation} in {Autonomous} {Driving}},
	shorttitle = {{FedDrive}},
	url = {http://arxiv.org/abs/2202.13670},
	abstract = {Semantic Segmentation is essential to make selfdriving vehicles autonomous, enabling them to understand their surroundings by assigning individual pixels to known categories. However, it operates on sensible data collected from the users’ cars; thus, protecting the clients’ privacy becomes a primary concern. For similar reasons, Federated Learning has been recently introduced as a new machine learning paradigm aiming to learn a global model while preserving privacy and leveraging data on millions of remote devices. Despite several efforts on this topic, no work has explicitly addressed the challenges of federated learning in semantic segmentation for driving so far. To ﬁll this gap, we propose FedDrive, a new benchmark consisting of three settings and two datasets, incorporating the real-world challenges of statistical heterogeneity and domain generalization. We benchmark state-of-the-art algorithms from the federated learning literature through an in-depth analysis, combining them with style transfer methods to improve their generalization ability. We demonstrate that correctly handling normalization statistics is crucial to deal with the aforementioned challenges. Furthermore, style transfer improves performance when dealing with signiﬁcant appearance shifts. We plan to make both the code and the benchmark publicly available to the research community.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2202.13670 [cs]},
	author = {Fantauzzo, Lidia and Fani', Eros and Caldarola, Debora and Tavera, Antonio and Cermelli, Fabio and Ciccone, Marco and Caputo, Barbara},
	month = feb,
	year = {2022},
	note = {arXiv: 2202.13670},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{hu_dynamic-aware_2022,
	title = {Dynamic-aware {Federated} {Learning} for {Face} {Forgery} {Video} {Detection}},
	issn = {2157-6904, 2157-6912},
	url = {https://dl.acm.org/doi/10.1145/3501814},
	doi = {10.1145/3501814},
	abstract = {The spread of face forgery videos causes a serious threat to information credibility, calling for efective detection algorithms to identify them. Most existing methods have assumed a shared or centralized training set. However, in practice, data may be distributed on devices of diferent enterprises that can not be centralized to share due to the security and privacy restrictions. In this paper, we propose a Federated Learning face forgery detection framework to train a global model collboratively while keeping data stay on local devices. In order to make the detection model more robust, we propose a novel InconsistencyCapture module (ICM) to capture the dynamic inconsistencies between adjacent frames of face forgery videos. The ICM contains two parallel branches. The irst branch takes the whole face of adjacent frames as input to calculate a global inconsistency representation. The second branch only focuses on the inter-frame variation of critical regions to capture the local inconsistency. To the best of our knowledge, this is the irst work to apply Federated Learning to face forgery video detection, which is trained with decentralized data. Extensive experiments show that the proposed framework achieves competitive performance compared to existing methods that are trained with centralized data, with higher-level security and privacy guarantee. CCS Concepts: · Security and privacy → Human and societal aspects of security and privacy; · Computing methodologies → Distributed computing methodologies.},
	language = {en},
	urldate = {2022-03-20},
	journal = {ACM Transactions on Intelligent Systems and Technology},
	author = {Hu, Ziheng and Xie, Hongtao and Yu, Lingyun and Gao, Xingyu and Shang, Zhihua and Zhang, Yongdong},
	month = feb,
	year = {2022},
	pages = {3501814},
}

@article{sun_decentralised_2021,
	title = {Decentralised {Person} {Re}-{Identification} with {Selective} {Knowledge} {Aggregation}},
	url = {http://arxiv.org/abs/2110.11384},
	abstract = {Existing person re-identiﬁcation (Re-ID) methods mostly follow a centralised learning paradigm which shares all training data to a collection for model learning. This paradigm is limited when data from different sources cannot be shared due to privacy concerns. To resolve this problem, two recent works [32, 41] have introduced decentralised (federated) Re-ID learning for constructing a globally generalised model (server) without any direct access to local training data nor shared data across different source domains (clients). However, these methods are poor on how to adapt the generalised model to maximise its performance on individual client domain Re-ID tasks having different Re-ID label spaces, due to a lack of understanding of data heterogeneity across domains. We call this poor ‘model personalisation’. In this work, we present a new Selective Knowledge Aggregation approach to decentralised person Re-ID to optimise the trade-off between model personalisation and generalisation. Speciﬁcally, we incorporate attentive normalisation into the normalisation layers in a deep ReID model and propose to learn local normalisation layers speciﬁc to each domain, which are decoupled from the global model aggregation in federated Re-ID learning. This helps to preserve model personalisation knowledge on each local client domain and learn instance-speciﬁc information. Further, we introduce a dual local normalisation mechanism to learn generalised normalisation layers in each local model, which are then transmitted to the global model for central aggregation. This facilitates selective knowledge aggregation on the server to construct a global generalised model for out-of-the-box deployment on unseen novel domains. Extensive experiments on eight person Re-ID datasets show that the proposed approach to decentralised Re-ID signiﬁcantly outperforms the state-of-the-art decentralised methods on both seen client domains and unseen novel domains.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2110.11384 [cs]},
	author = {Sun, Shitong and Wu, Guile and Gong, Shaogang},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.11384},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}


@article{wang_field_2021,
	title = {A {Field} {Guide} to {Federated} {Optimization}},
	url = {http://arxiv.org/abs/2107.06917},
	abstract = {Federated learning and analytics are a distributed approach for collaboratively learning models (or statistics) from decentralized data, motivated by and designed for privacy protection. The distributed learning process can be formulated as solving federated optimization problems, which emphasize communication eﬃciency, data heterogeneity, compatibility with privacy and system requirements, and other constraints that are not primary considerations in other problem settings. This paper provides recommendations and guidelines on formulating, designing, evaluating and analyzing federated optimization algorithms through concrete examples and practical implementation, with a focus on conducting eﬀective simulations to infer real-world performance. The goal of this work is not to survey the current literature, but to inspire researchers and practitioners to design federated learning algorithms that can be used in various practical applications.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2107.06917 [cs]},
	author = {Wang, Jianyu and Charles, Zachary and Xu, Zheng and Joshi, Gauri and McMahan, H. Brendan and Arcas, Blaise Aguera y and Al-Shedivat, Maruan and Andrew, Galen and Avestimehr, Salman and Daly, Katharine and Data, Deepesh and Diggavi, Suhas and Eichner, Hubert and Gadhikar, Advait and Garrett, Zachary and Girgis, Antonious M. and Hanzely, Filip and Hard, Andrew and He, Chaoyang and Horvath, Samuel and Huo, Zhouyuan and Ingerman, Alex and Jaggi, Martin and Javidi, Tara and Kairouz, Peter and Kale, Satyen and Karimireddy, Sai Praneeth and Konecny, Jakub and Koyejo, Sanmi and Li, Tian and Liu, Luyang and Mohri, Mehryar and Qi, Hang and Reddi, Sashank J. and Richtarik, Peter and Singhal, Karan and Smith, Virginia and Soltanolkotabi, Mahdi and Song, Weikang and Suresh, Ananda Theertha and Stich, Sebastian U. and Talwalkar, Ameet and Wang, Hongyi and Woodworth, Blake and Wu, Shanshan and Yu, Felix X. and Yuan, Honglin and Zaheer, Manzil and Zhang, Mi and Zhang, Tong and Zheng, Chunxiang and Zhu, Chen and Zhu, Wennan},
	month = jul,
	year = {2021},
	note = {arXiv: 2107.06917},
	keywords = {Computer Science - Machine Learning},
}

@article{yang_federated_2022,
	title = {Federated and {Generalized} {Person} {Re}-identification through {Domain} and {Feature} {Hallucinating}},
	url = {http://arxiv.org/abs/2203.02689},
	abstract = {In this paper, we study the problem of federated domain generalization (FedDG) for person reidentiﬁcation (re-ID), which aims to learn a generalized model with multiple decentralized labeled source domains. An empirical method (FedAvg) trains local models individually and averages them to obtain the global model for further local ﬁne-tuning or deploying in unseen target domains. One drawback of FedAvg is neglecting the data distributions of other clients during local training, making the local model overﬁt local data and producing a poorly-generalized global model. To solve this problem, we propose a novel method, called “Domain and Feature Hallucinating (DFH)”, to produce diverse features for learning generalized local and global models. Speciﬁcally, after each model aggregation process, we share the Domain-level Feature Statistics (DFS) among different clients without violating data privacy. During local training, the DFS are used to synthesize novel domain statistics with the proposed domain hallucinating, which is achieved by re-weighting DFS with random weights. Then, we propose feature hallucinating to diversify local features by scaling and shifting them to the distribution of the obtained novel domain. The synthesized novel features retain the original pair-wise similarities, enabling us to utilize them to optimize the model in a supervised manner. Extensive experiments verify that the proposed DFH can effectively improve the generalization ability of the global model. Our method achieves the state-of-the-art performance for FedDG on four large-scale re-ID benchmarks.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2203.02689 [cs]},
	author = {Yang, Fengxiang and Zhong, Zhun and Luo, Zhiming and Li, Shaozi and Sebe, Nicu},
	month = mar,
	year = {2022},
	note = {arXiv: 2203.02689},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{zhuang_towards_2021,
	title = {Towards {Unsupervised} {Domain} {Adaptation} for {Deep} {Face} {Recognition} under {Privacy} {Constraints} via {Federated} {Learning}},
	url = {http://arxiv.org/abs/2105.07606},
	abstract = {Unsupervised domain adaptation has been widely adopted to generalize models for unlabeled data in a target domain, given labeled data in a source domain, whose data distributions differ from the target domain. However, existing works are inapplicable to face recognition under privacy constraints because they require sharing sensitive face images between two domains. To address this problem, we propose a novel unsupervised federated face recognition approach (FedFR). FedFR improves the performance in the target domain by iteratively aggregating knowledge from the source domain through federated learning. It protects data privacy by transferring models instead of raw data between domains. Besides, we propose a new domain constraint loss (DCL) to regularize source domain training. DCL suppresses the data volume dominance of the source domain. We also enhance a hierarchical clustering algorithm to predict pseudo labels for the unlabeled target domain accurately. To this end, FedFR forms an end-to-end training pipeline: (1) pre-train in the source domain; (2) predict pseudo labels by clustering in the target domain; (3) conduct domain-constrained federated learning across two domains. Extensive experiments and analysis on two newly constructed benchmarks demonstrate the effectiveness of FedFR. It outperforms the baseline and classic methods in the target domain by over 4\% on the more realistic benchmark. We believe that FedFR will shed light on applying federated learning to more computer vision tasks under privacy constraints.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2105.07606 [cs]},
	author = {Zhuang, Weiming and Gan, Xin and Wen, Yonggang and Zhang, Xuesen and Zhang, Shuai and Yi, Shuai},
	month = may,
	year = {2021},
	note = {arXiv: 2105.07606},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
}

@article{zhuang_performance_2020,
	title = {Performance {Optimization} for {Federated} {Person} {Re}-identification via {Benchmark} {Analysis}},
	url = {http://arxiv.org/abs/2008.11560},
	doi = {10.1145/3394171.3413814},
	abstract = {Federated learning is a privacy-preserving machine learning technique that learns a shared model across decentralized clients. It can alleviate privacy concerns of personal re-identification, an important computer vision task. In this work, we implement federated learning to person re-identification (FedReID) and optimize its performance affected by statistical heterogeneity in the realworld scenario. We first construct a new benchmark to investigate the performance of FedReID. This benchmark consists of (1) nine datasets with different volumes sourced from different domains to simulate the heterogeneous situation in reality, (2) two federated scenarios, and (3) an enhanced federated algorithm for FedReID. The benchmark analysis shows that the client-edge-cloud architecture, represented by the federated-by-dataset scenario, has better performance than client-server architecture in FedReID. It also reveals the bottlenecks of FedReID under the real-world scenario, including poor performance of large datasets caused by unbalanced weights in model aggregation and challenges in convergence. Then we propose two optimization methods: (1) To address the unbalanced weight problem, we propose a new method to dynamically change the weights according to the scale of model changes in clients in each training round; (2) To facilitate convergence, we adopt knowledge distillation to refine the server model with knowledge generated from client models on a public dataset. Experiment results demonstrate that our strategies can achieve much better convergence with superior performance on all datasets. We believe that our work will inspire the community to further explore the implementation of federated learning on more computer vision tasks in real-world scenarios.},
	language = {en},
	urldate = {2022-03-20},
	journal = {Proceedings of the 28th ACM International Conference on Multimedia},
	author = {Zhuang, Weiming and Wen, Yonggang and Zhang, Xuesen and Gan, Xin and Yin, Daiying and Zhou, Dongzhan and Zhang, Shuai and Yi, Shuai},
	month = oct,
	year = {2020},
	note = {arXiv: 2008.11560},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
	pages = {955--963},
}

@article{wu_decentralised_2021,
	title = {Decentralised {Learning} from {Independent} {Multi}-{Domain} {Labels} for {Person} {Re}-{Identification}},
	url = {http://arxiv.org/abs/2006.04150},
	abstract = {Deep learning has been successful for many computer vision tasks due to the availability of shared and centralised large-scale training data. However, increasing awareness of privacy concerns poses new challenges to deep learning, especially for human subject related recognition such as person re-identiﬁcation (Re-ID). In this work, we solve the Re-ID problem by decentralised learning from non-shared private training data distributed at multiple user sites of independent multi-domain label spaces. We propose a novel paradigm called Federated Person Re-Identiﬁcation (FedReID) to construct a generalisable global model (a central server) by simultaneously learning with multiple privacy-preserved local models (local clients). Speciﬁcally, each local client receives global model updates from the server and trains a local model using its local data independent from all the other clients. Then, the central server aggregates transferrable local model updates to construct a generalisable global feature embedding model without accessing local data so to preserve local privacy. This client-server collaborative learning process is iteratively performed under privacy control, enabling FedReID to realise decentralised learning without sharing distributed data nor collecting any centralised data. Extensive experiments on ten Re-ID benchmarks show that FedReID achieves compelling generalisation performance beyond any locally trained models without using shared training data, whilst inherently protects the privacy of each local client. This is uniquely advantageous over contemporary Re-ID methods.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2006.04150 [cs]},
	author = {Wu, Guile and Gong, Shaogang},
	month = jul,
	year = {2021},
	note = {arXiv: 2006.04150},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{raza_lightweight_2021,
	title = {Lightweight {Transformer} in {Federated} {Setting} for {Human} {Activity} {Recognition}},
	url = {http://arxiv.org/abs/2110.00244},
	abstract = {Human Activity Recognition (HAR) has been a challenging problem yet it needs to be solved. It will mainly be used for eldercare and healthcare as an assistive technology when ensemble with other technologies like Internet of Things(IoT). HAR can be achieved with the help of sensors, smartphones or images. Deep neural network techniques like artiﬁcial neural networks, convolutional neural networks and recurrent neural networks have been used in HAR, both in centralized and federated setting. However,these techniques have certain limitations. RNNs have limitation of parallelization, CNNS have the limitation of sequence length and they are computationally expensive. In this paper, to address the state of art challenges, we present a inertial sensors-based novel one patch transformer which gives the best of both RNNs and CNNs for Human activity recognition. We also design a testbed to collect real-time human activity data. The data collected is further used to train and test the proposed transformer. With the help of experiments, we show that the proposed transformer outperforms the state of art CNN and RNN based classiﬁers, both in federated and centralized setting. Moreover, the proposed transformer is computationally inexpensive as it uses very few parameter compared to the existing state of art CNN and RNN based classiﬁer. Thus its more suitable for federated learning as it provides less communication and computational cost.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2110.00244 [cs]},
	author = {Raza, Ali and Tran, Kim Phuc and Koehl, Ludovic and Li, Shujun and Zeng, Xianyi and Benzaidi, Khaled},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.00244},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@article{zhuang_performance_2020-1,
	title = {Performance {Optimization} for {Federated} {Person} {Re}-identification via {Benchmark} {Analysis}},
	url = {http://arxiv.org/abs/2008.11560},
	doi = {10.1145/3394171.3413814},
	abstract = {Federated learning is a privacy-preserving machine learning technique that learns a shared model across decentralized clients. It can alleviate privacy concerns of personal re-identification, an important computer vision task. In this work, we implement federated learning to person re-identification (FedReID) and optimize its performance affected by statistical heterogeneity in the realworld scenario. We first construct a new benchmark to investigate the performance of FedReID. This benchmark consists of (1) nine datasets with different volumes sourced from different domains to simulate the heterogeneous situation in reality, (2) two federated scenarios, and (3) an enhanced federated algorithm for FedReID. The benchmark analysis shows that the client-edge-cloud architecture, represented by the federated-by-dataset scenario, has better performance than client-server architecture in FedReID. It also reveals the bottlenecks of FedReID under the real-world scenario, including poor performance of large datasets caused by unbalanced weights in model aggregation and challenges in convergence. Then we propose two optimization methods: (1) To address the unbalanced weight problem, we propose a new method to dynamically change the weights according to the scale of model changes in clients in each training round; (2) To facilitate convergence, we adopt knowledge distillation to refine the server model with knowledge generated from client models on a public dataset. Experiment results demonstrate that our strategies can achieve much better convergence with superior performance on all datasets. We believe that our work will inspire the community to further explore the implementation of federated learning on more computer vision tasks in real-world scenarios.},
	language = {en},
	urldate = {2022-03-20},
	journal = {Proceedings of the 28th ACM International Conference on Multimedia},
	author = {Zhuang, Weiming and Wen, Yonggang and Zhang, Xuesen and Gan, Xin and Yin, Daiying and Zhou, Dongzhan and Zhang, Shuai and Yi, Shuai},
	month = oct,
	year = {2020},
	note = {arXiv: 2008.11560},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
	pages = {955--963},
}

@article{bai_federated_2021,
	title = {Federated {Face} {Recognition}},
	url = {http://arxiv.org/abs/2105.02501},
	abstract = {Face recognition has been extensively studied in computer vision and artiﬁcial intelligence communities in recent years. An important issue of face recognition is data privacy, which receives more and more public concerns. As a common privacy-preserving technique, Federated Learning is proposed to train a model cooperatively without sharing data between parties. However, as far as we know, it has not been successfully applied in face recognition. This paper proposes a framework named FedFace to innovate federated learning for face recognition. Speciﬁcally, FedFace relies on two major innovative algorithms, Partially Federated Momentum (PFM) and Federated Validation (FV). PFM locally applies an estimated equivalent global momentum to approximating the centralized momentum-SGD efﬁciently. FV repeatedly searches for better federated aggregating weightings via testing the aggregated models on some private validation datasets, which can improve the model’s generalization ability. The ablation study and extensive experiments validate the effectiveness of the FedFace method and show that it is comparable to or even better than the centralized baseline in performance.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2105.02501 [cs]},
	author = {Bai, Fan and Wu, Jiaxiang and Shen, Pengcheng and Li, Shaoxin and Zhou, Shuigeng},
	month = may,
	year = {2021},
	note = {arXiv: 2105.02501},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}

@article{liu_federated_2022,
	title = {Federated {Remote} {Physiological} {Measurement} with {Imperfect} {Data}},
	url = {http://arxiv.org/abs/2203.05759},
	abstract = {The growing need for technology that supports remote healthcare is being acutely highlighted by an aging population and the COVID-19 pandemic. In health-related machine learning applications the ability to learn predictive models without data leaving a private device is attractive, especially when these data might contain features (e.g., photographs or videos of the body) that make identifying a subject trivial and/or the training data volume is large (e.g., uncompressed video). Camera-based remote physiological sensing facilitates scalable and low-cost measurement, but is a prime example of a task that involves analysing high bit-rate videos containing identiﬁable images and sensitive health information. Federated learning enables privacy-preserving decentralized training which has several properties beneﬁcial for camera-based sensing. We develop the ﬁrst mobile federated learning camera-based sensing system and show that it can perform competitively with traditional state-of-the-art supervised approaches. However, in the presence of corrupted data (e.g., video or label noise) from a few devices the performance of weight averaging quickly degrades. To address this, we leverage knowledge about the expected noise proﬁle within the video to intelligently adjust how the model weights are averaged on the server. Our results show that this signiﬁcantly improves upon the robustness of models even when the signal-to-noise ratio is low.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2203.05759 [cs, eess]},
	author = {Liu, Xin and Zhang, Mingchuan and Jiang, Ziheng and Patel, Shwetak and McDuff, Daniel},
	month = mar,
	year = {2022},
	note = {arXiv: 2203.05759},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Electrical Engineering and Systems Science - Image and Video Processing},
}

@article{zhang_federated_2022-1,
	title = {Federated {Learning} for {Internet} of {Things}: {Applications}, {Challenges}, and {Opportunities}},
	shorttitle = {Federated {Learning} for {Internet} of {Things}},
	url = {http://arxiv.org/abs/2111.07494},
	abstract = {Billions of IoT devices will be deployed in the near future, taking advantage of faster Internet speed and the possibility of orders of magnitude more endpoints brought by 5G/6G. With the growth of IoT devices, vast quantities of data that may contain users’ private information will be generated. The high communication and storage costs, mixed with privacy concerns, will increasingly challenge the traditional ecosystem of centralized over-the-cloud learning and processing for IoT platforms. Federated Learning (FL) has emerged as the most promising alternative approach to this problem. In FL, training data-driven machine learning models is an act of collaboration between multiple clients without requiring the data to be brought to a central point, hence alleviating communication and storage costs and providing a great degree of user-level privacy. However, there are still some challenges existing in the real FL system implementation on IoT networks. In this paper, we will discuss the opportunities and challenges of FL in IoT platforms, as well as how it can enable diverse IoT applications. In particular, we identify and discuss seven critical challenges of FL in IoT platforms and highlight some recent promising approaches towards addressing them.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2111.07494 [cs]},
	author = {Zhang, Tuo and Gao, Lei and He, Chaoyang and Zhang, Mi and Krishnamachari, Bhaskar and Avestimehr, Salman},
	month = mar,
	year = {2022},
	note = {arXiv: 2111.07494},
	keywords = {Computer Science - Machine Learning},
}

@inproceedings{kim_federated_2021-1,
	address = {Las Vegas, NV, USA},
	title = {Federated {Learning} for {Face} {Recognition}},
	isbn = {978-1-72819-766-1},
	url = {https://ieeexplore.ieee.org/document/9427748/},
	doi = {10.1109/ICCE50685.2021.9427748},
	abstract = {With the rapid development of deep learning, the accuracy of face recognition has significantly increased. However, training a face recognition model requires the collection of private data to a centralized server to obtain high performance in the desired domain. Since federated learning is a technique to train a model without collecting data to a server, it is a suitable architecture to train a face recognition model with privacysensitive face images held in personal smartphones. This study proposes strategies to apply federated learning to face recognition model training.},
	language = {en},
	urldate = {2022-03-20},
	booktitle = {2021 {IEEE} {International} {Conference} on {Consumer} {Electronics} ({ICCE})},
	publisher = {IEEE},
	author = {Kim, Jaehyeok and Park, Taehyeong and Kim, Hyorin and Kim, Suhyun},
	month = jan,
	year = {2021},
	pages = {1--2},
}

@article{shao_federated_2020-1,
	title = {Federated {Face} {Presentation} {Attack} {Detection}},
	url = {http://arxiv.org/abs/2005.14638},
	abstract = {Face presentation attack detection (fPAD) plays a critical role in the modern face recognition pipeline. A face presentation attack detection model with good generalization can be obtained when it is trained with face images from different input distributions and different types of spoof attacks. In reality, training data (both real face images and spoof images) are not directly shared between data owners due to legal and privacy issues. In this paper, with the motivation of circumventing this challenge, we propose Federated Face Presentation Attack Detection (FedPAD) framework. FedPAD simultaneously takes advantage of rich fPAD information available at different data owners while preserving data privacy. In the proposed framework, each data owner (referred to as data centers) locally trains its own fPAD model. A server learns a global fPAD model by iteratively aggregating model updates from all data centers without accessing private data in each of them. Once the learned global model converges, it is used for fPAD inference. We introduce the experimental setting to evaluate the proposed FedPAD framework and carry out extensive experiments to provide various insights about federated learning for fPAD.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2005.14638 [cs]},
	author = {Shao, Rui and Perera, Pramuditha and Yuen, Pong C. and Patel, Vishal M.},
	month = sep,
	year = {2020},
	note = {arXiv: 2005.14638},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{fantauzzo_feddrive_2022-1,
	title = {{FedDrive}: {Generalizing} {Federated} {Learning} to {Semantic} {Segmentation} in {Autonomous} {Driving}},
	shorttitle = {{FedDrive}},
	url = {http://arxiv.org/abs/2202.13670},
	abstract = {Semantic Segmentation is essential to make selfdriving vehicles autonomous, enabling them to understand their surroundings by assigning individual pixels to known categories. However, it operates on sensible data collected from the users’ cars; thus, protecting the clients’ privacy becomes a primary concern. For similar reasons, Federated Learning has been recently introduced as a new machine learning paradigm aiming to learn a global model while preserving privacy and leveraging data on millions of remote devices. Despite several efforts on this topic, no work has explicitly addressed the challenges of federated learning in semantic segmentation for driving so far. To ﬁll this gap, we propose FedDrive, a new benchmark consisting of three settings and two datasets, incorporating the real-world challenges of statistical heterogeneity and domain generalization. We benchmark state-of-the-art algorithms from the federated learning literature through an in-depth analysis, combining them with style transfer methods to improve their generalization ability. We demonstrate that correctly handling normalization statistics is crucial to deal with the aforementioned challenges. Furthermore, style transfer improves performance when dealing with signiﬁcant appearance shifts. We plan to make both the code and the benchmark publicly available to the research community.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2202.13670 [cs]},
	author = {Fantauzzo, Lidia and Fani', Eros and Caldarola, Debora and Tavera, Antonio and Cermelli, Fabio and Ciccone, Marco and Caputo, Barbara},
	month = feb,
	year = {2022},
	note = {arXiv: 2202.13670},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{hu_dynamic-aware_2022-1,
	title = {Dynamic-aware {Federated} {Learning} for {Face} {Forgery} {Video} {Detection}},
	issn = {2157-6904, 2157-6912},
	url = {https://dl.acm.org/doi/10.1145/3501814},
	doi = {10.1145/3501814},
	abstract = {The spread of face forgery videos causes a serious threat to information credibility, calling for efective detection algorithms to identify them. Most existing methods have assumed a shared or centralized training set. However, in practice, data may be distributed on devices of diferent enterprises that can not be centralized to share due to the security and privacy restrictions. In this paper, we propose a Federated Learning face forgery detection framework to train a global model collboratively while keeping data stay on local devices. In order to make the detection model more robust, we propose a novel InconsistencyCapture module (ICM) to capture the dynamic inconsistencies between adjacent frames of face forgery videos. The ICM contains two parallel branches. The irst branch takes the whole face of adjacent frames as input to calculate a global inconsistency representation. The second branch only focuses on the inter-frame variation of critical regions to capture the local inconsistency. To the best of our knowledge, this is the irst work to apply Federated Learning to face forgery video detection, which is trained with decentralized data. Extensive experiments show that the proposed framework achieves competitive performance compared to existing methods that are trained with centralized data, with higher-level security and privacy guarantee. CCS Concepts: · Security and privacy → Human and societal aspects of security and privacy; · Computing methodologies → Distributed computing methodologies.},
	language = {en},
	urldate = {2022-03-20},
	journal = {ACM Transactions on Intelligent Systems and Technology},
	author = {Hu, Ziheng and Xie, Hongtao and Yu, Lingyun and Gao, Xingyu and Shang, Zhihua and Zhang, Yongdong},
	month = feb,
	year = {2022},
	pages = {3501814},
}

@article{sun_decentralised_2021-1,
	title = {Decentralised {Person} {Re}-{Identification} with {Selective} {Knowledge} {Aggregation}},
	url = {http://arxiv.org/abs/2110.11384},
	abstract = {Existing person re-identiﬁcation (Re-ID) methods mostly follow a centralised learning paradigm which shares all training data to a collection for model learning. This paradigm is limited when data from different sources cannot be shared due to privacy concerns. To resolve this problem, two recent works [32, 41] have introduced decentralised (federated) Re-ID learning for constructing a globally generalised model (server) without any direct access to local training data nor shared data across different source domains (clients). However, these methods are poor on how to adapt the generalised model to maximise its performance on individual client domain Re-ID tasks having different Re-ID label spaces, due to a lack of understanding of data heterogeneity across domains. We call this poor ‘model personalisation’. In this work, we present a new Selective Knowledge Aggregation approach to decentralised person Re-ID to optimise the trade-off between model personalisation and generalisation. Speciﬁcally, we incorporate attentive normalisation into the normalisation layers in a deep ReID model and propose to learn local normalisation layers speciﬁc to each domain, which are decoupled from the global model aggregation in federated Re-ID learning. This helps to preserve model personalisation knowledge on each local client domain and learn instance-speciﬁc information. Further, we introduce a dual local normalisation mechanism to learn generalised normalisation layers in each local model, which are then transmitted to the global model for central aggregation. This facilitates selective knowledge aggregation on the server to construct a global generalised model for out-of-the-box deployment on unseen novel domains. Extensive experiments on eight person Re-ID datasets show that the proposed approach to decentralised Re-ID signiﬁcantly outperforms the state-of-the-art decentralised methods on both seen client domains and unseen novel domains.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2110.11384 [cs]},
	author = {Sun, Shitong and Wu, Guile and Gong, Shaogang},
	month = oct,
	year = {2021},
	note = {arXiv: 2110.11384},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition},
}


@article{wang_field_2021-1,
	title = {A {Field} {Guide} to {Federated} {Optimization}},
	url = {http://arxiv.org/abs/2107.06917},
	abstract = {Federated learning and analytics are a distributed approach for collaboratively learning models (or statistics) from decentralized data, motivated by and designed for privacy protection. The distributed learning process can be formulated as solving federated optimization problems, which emphasize communication eﬃciency, data heterogeneity, compatibility with privacy and system requirements, and other constraints that are not primary considerations in other problem settings. This paper provides recommendations and guidelines on formulating, designing, evaluating and analyzing federated optimization algorithms through concrete examples and practical implementation, with a focus on conducting eﬀective simulations to infer real-world performance. The goal of this work is not to survey the current literature, but to inspire researchers and practitioners to design federated learning algorithms that can be used in various practical applications.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2107.06917 [cs]},
	author = {Wang, Jianyu and Charles, Zachary and Xu, Zheng and Joshi, Gauri and McMahan, H. Brendan and Arcas, Blaise Aguera y and Al-Shedivat, Maruan and Andrew, Galen and Avestimehr, Salman and Daly, Katharine and Data, Deepesh and Diggavi, Suhas and Eichner, Hubert and Gadhikar, Advait and Garrett, Zachary and Girgis, Antonious M. and Hanzely, Filip and Hard, Andrew and He, Chaoyang and Horvath, Samuel and Huo, Zhouyuan and Ingerman, Alex and Jaggi, Martin and Javidi, Tara and Kairouz, Peter and Kale, Satyen and Karimireddy, Sai Praneeth and Konecny, Jakub and Koyejo, Sanmi and Li, Tian and Liu, Luyang and Mohri, Mehryar and Qi, Hang and Reddi, Sashank J. and Richtarik, Peter and Singhal, Karan and Smith, Virginia and Soltanolkotabi, Mahdi and Song, Weikang and Suresh, Ananda Theertha and Stich, Sebastian U. and Talwalkar, Ameet and Wang, Hongyi and Woodworth, Blake and Wu, Shanshan and Yu, Felix X. and Yuan, Honglin and Zaheer, Manzil and Zhang, Mi and Zhang, Tong and Zheng, Chunxiang and Zhu, Chen and Zhu, Wennan},
	month = jul,
	year = {2021},
	note = {arXiv: 2107.06917},
	keywords = {Computer Science - Machine Learning},
}

@article{yang_federated_2022-1,
	title = {Federated and {Generalized} {Person} {Re}-identification through {Domain} and {Feature} {Hallucinating}},
	url = {http://arxiv.org/abs/2203.02689},
	abstract = {In this paper, we study the problem of federated domain generalization (FedDG) for person reidentiﬁcation (re-ID), which aims to learn a generalized model with multiple decentralized labeled source domains. An empirical method (FedAvg) trains local models individually and averages them to obtain the global model for further local ﬁne-tuning or deploying in unseen target domains. One drawback of FedAvg is neglecting the data distributions of other clients during local training, making the local model overﬁt local data and producing a poorly-generalized global model. To solve this problem, we propose a novel method, called “Domain and Feature Hallucinating (DFH)”, to produce diverse features for learning generalized local and global models. Speciﬁcally, after each model aggregation process, we share the Domain-level Feature Statistics (DFS) among different clients without violating data privacy. During local training, the DFS are used to synthesize novel domain statistics with the proposed domain hallucinating, which is achieved by re-weighting DFS with random weights. Then, we propose feature hallucinating to diversify local features by scaling and shifting them to the distribution of the obtained novel domain. The synthesized novel features retain the original pair-wise similarities, enabling us to utilize them to optimize the model in a supervised manner. Extensive experiments verify that the proposed DFH can effectively improve the generalization ability of the global model. Our method achieves the state-of-the-art performance for FedDG on four large-scale re-ID benchmarks.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2203.02689 [cs]},
	author = {Yang, Fengxiang and Zhong, Zhun and Luo, Zhiming and Li, Shaozi and Sebe, Nicu},
	month = mar,
	year = {2022},
	note = {arXiv: 2203.02689},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{zhuang_towards_2021-1,
	title = {Towards {Unsupervised} {Domain} {Adaptation} for {Deep} {Face} {Recognition} under {Privacy} {Constraints} via {Federated} {Learning}},
	url = {http://arxiv.org/abs/2105.07606},
	abstract = {Unsupervised domain adaptation has been widely adopted to generalize models for unlabeled data in a target domain, given labeled data in a source domain, whose data distributions differ from the target domain. However, existing works are inapplicable to face recognition under privacy constraints because they require sharing sensitive face images between two domains. To address this problem, we propose a novel unsupervised federated face recognition approach (FedFR). FedFR improves the performance in the target domain by iteratively aggregating knowledge from the source domain through federated learning. It protects data privacy by transferring models instead of raw data between domains. Besides, we propose a new domain constraint loss (DCL) to regularize source domain training. DCL suppresses the data volume dominance of the source domain. We also enhance a hierarchical clustering algorithm to predict pseudo labels for the unlabeled target domain accurately. To this end, FedFR forms an end-to-end training pipeline: (1) pre-train in the source domain; (2) predict pseudo labels by clustering in the target domain; (3) conduct domain-constrained federated learning across two domains. Extensive experiments and analysis on two newly constructed benchmarks demonstrate the effectiveness of FedFR. It outperforms the baseline and classic methods in the target domain by over 4\% on the more realistic benchmark. We believe that FedFR will shed light on applying federated learning to more computer vision tasks under privacy constraints.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2105.07606 [cs]},
	author = {Zhuang, Weiming and Gan, Xin and Wen, Yonggang and Zhang, Xuesen and Zhang, Shuai and Yi, Shuai},
	month = may,
	year = {2021},
	note = {arXiv: 2105.07606},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
}

@article{zhuang_performance_2020-2,
	title = {Performance {Optimization} for {Federated} {Person} {Re}-identification via {Benchmark} {Analysis}},
	url = {http://arxiv.org/abs/2008.11560},
	doi = {10.1145/3394171.3413814},
	abstract = {Federated learning is a privacy-preserving machine learning technique that learns a shared model across decentralized clients. It can alleviate privacy concerns of personal re-identification, an important computer vision task. In this work, we implement federated learning to person re-identification (FedReID) and optimize its performance affected by statistical heterogeneity in the realworld scenario. We first construct a new benchmark to investigate the performance of FedReID. This benchmark consists of (1) nine datasets with different volumes sourced from different domains to simulate the heterogeneous situation in reality, (2) two federated scenarios, and (3) an enhanced federated algorithm for FedReID. The benchmark analysis shows that the client-edge-cloud architecture, represented by the federated-by-dataset scenario, has better performance than client-server architecture in FedReID. It also reveals the bottlenecks of FedReID under the real-world scenario, including poor performance of large datasets caused by unbalanced weights in model aggregation and challenges in convergence. Then we propose two optimization methods: (1) To address the unbalanced weight problem, we propose a new method to dynamically change the weights according to the scale of model changes in clients in each training round; (2) To facilitate convergence, we adopt knowledge distillation to refine the server model with knowledge generated from client models on a public dataset. Experiment results demonstrate that our strategies can achieve much better convergence with superior performance on all datasets. We believe that our work will inspire the community to further explore the implementation of federated learning on more computer vision tasks in real-world scenarios.},
	language = {en},
	urldate = {2022-03-20},
	journal = {Proceedings of the 28th ACM International Conference on Multimedia},
	author = {Zhuang, Weiming and Wen, Yonggang and Zhang, Xuesen and Gan, Xin and Yin, Daiying and Zhou, Dongzhan and Zhang, Shuai and Yi, Shuai},
	month = oct,
	year = {2020},
	note = {arXiv: 2008.11560},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Distributed, Parallel, and Cluster Computing, Computer Science - Machine Learning},
	pages = {955--963},
}

@article{wu_decentralised_2021-1,
	title = {Decentralised {Learning} from {Independent} {Multi}-{Domain} {Labels} for {Person} {Re}-{Identification}},
	url = {http://arxiv.org/abs/2006.04150},
	abstract = {Deep learning has been successful for many computer vision tasks due to the availability of shared and centralised large-scale training data. However, increasing awareness of privacy concerns poses new challenges to deep learning, especially for human subject related recognition such as person re-identiﬁcation (Re-ID). In this work, we solve the Re-ID problem by decentralised learning from non-shared private training data distributed at multiple user sites of independent multi-domain label spaces. We propose a novel paradigm called Federated Person Re-Identiﬁcation (FedReID) to construct a generalisable global model (a central server) by simultaneously learning with multiple privacy-preserved local models (local clients). Speciﬁcally, each local client receives global model updates from the server and trains a local model using its local data independent from all the other clients. Then, the central server aggregates transferrable local model updates to construct a generalisable global feature embedding model without accessing local data so to preserve local privacy. This client-server collaborative learning process is iteratively performed under privacy control, enabling FedReID to realise decentralised learning without sharing distributed data nor collecting any centralised data. Extensive experiments on ten Re-ID benchmarks show that FedReID achieves compelling generalisation performance beyond any locally trained models without using shared training data, whilst inherently protects the privacy of each local client. This is uniquely advantageous over contemporary Re-ID methods.},
	language = {en},
	urldate = {2022-03-20},
	journal = {arXiv:2006.04150 [cs]},
	author = {Wu, Guile and Gong, Shaogang},
	month = jul,
	year = {2021},
	note = {arXiv: 2006.04150},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{wang_pyramid_2021,
	title = {Pyramid {Vision} {Transformer}: {A} {Versatile} {Backbone} for {Dense} {Prediction} without {Convolutions}},
	shorttitle = {Pyramid {Vision} {Transformer}},
	url = {http://arxiv.org/abs/2102.12122},
	abstract = {Although using convolutional neural networks (CNNs) as backbones achieves great successes in computer vision, this work investigates a simple backbone network useful for many dense prediction tasks without convolutions. Unlike the recently-proposed Transformer model (e.g., ViT) that is specially designed for image classification, we propose Pyramid Vision Transformer{\textasciitilde}(PVT), which overcomes the difficulties of porting Transformer to various dense prediction tasks. PVT has several merits compared to prior arts. (1) Different from ViT that typically has low-resolution outputs and high computational and memory cost, PVT can be not only trained on dense partitions of the image to achieve high output resolution, which is important for dense predictions but also using a progressive shrinking pyramid to reduce computations of large feature maps. (2) PVT inherits the advantages from both CNN and Transformer, making it a unified backbone in various vision tasks without convolutions by simply replacing CNN backbones. (3) We validate PVT by conducting extensive experiments, showing that it boosts the performance of many downstream tasks, e.g., object detection, semantic, and instance segmentation. For example, with a comparable number of parameters, RetinaNet+PVT achieves 40.4 AP on the COCO dataset, surpassing RetinNet+ResNet50 (36.3 AP) by 4.1 absolute AP. We hope PVT could serve as an alternative and useful backbone for pixel-level predictions and facilitate future researches. Code is available at https://github.com/whai362/PVT.},
	urldate = {2021-09-17},
	journal = {arXiv:2102.12122 [cs]},
	author = {Wang, Wenhai and Xie, Enze and Li, Xiang and Fan, Deng-Ping and Song, Kaitao and Liang, Ding and Lu, Tong and Luo, Ping and Shao, Ling},
	month = aug,
	year = {2021},
	note = {arXiv: 2102.12122},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{zhang_multi-scale_2021,
	title = {Multi-{Scale} {Vision} {Longformer}: {A} {New} {Vision} {Transformer} for {High}-{Resolution} {Image} {Encoding}},
	shorttitle = {Multi-{Scale} {Vision} {Longformer}},
	url = {http://arxiv.org/abs/2103.15358},
	abstract = {This paper presents a new Vision Transformer (ViT) architecture Multi-Scale Vision Longformer, which significantly enhances the ViT of {\textbackslash}cite\{dosovitskiy2020image\} for encoding high-resolution images using two techniques. The first is the multi-scale model structure, which provides image encodings at multiple scales with manageable computational cost. The second is the attention mechanism of vision Longformer, which is a variant of Longformer {\textbackslash}cite\{beltagy2020longformer\}, originally developed for natural language processing, and achieves a linear complexity w.r.t. the number of input tokens. A comprehensive empirical study shows that the new ViT significantly outperforms several strong baselines, including the existing ViT models and their ResNet counterparts, and the Pyramid Vision Transformer from a concurrent work {\textbackslash}cite\{wang2021pyramid\}, on a range of vision tasks, including image classification, object detection, and segmentation. The models and source code are released at {\textbackslash}url\{https://github.com/microsoft/vision-longformer\}.},
	urldate = {2021-09-17},
	journal = {arXiv:2103.15358 [cs]},
	author = {Zhang, Pengchuan and Dai, Xiyang and Yang, Jianwei and Xiao, Bin and Yuan, Lu and Zhang, Lei and Gao, Jianfeng},
	month = may,
	year = {2021},
	note = {arXiv: 2103.15358},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{aligholian_unsupervised_2021,
	title = {Unsupervised {Event} {Detection}, {Clustering}, and {Use} {Case} {Exposition} in {Micro}-{PMU} {Measurements}},
	volume = {12},
	issn = {1949-3053, 1949-3061},
	url = {http://arxiv.org/abs/2007.15237},
	doi = {10.1109/TSG.2021.3063088},
	abstract = {Distribution-level phasor measurement units, a.k.a, micro-PMUs, report a large volume of high resolution phasor measurements which constitute a variety of event signatures of different phenomena that occur all across power distribution feeders. In order to implement an event-based analysis that has useful applications for the utility operator, one needs to extract these events from a large volume of micro-PMU data. However, due to the infrequent, unscheduled, and unknown nature of the events, it is often a challenge to even figure out what kind of events are out there to capture and scrutinize. In this paper, we seek to address this open problem by developing an unsupervised approach, which requires minimal prior human knowledge. First, we develop an unsupervised event detection method based on the concept of Generative Adversarial Networks (GAN). It works by training deep neural networks that learn the characteristics of the normal trends in micro-PMU measurements; and accordingly detect an event when there is any abnormality. We also propose a two-step unsupervised clustering method, based on a novel linear mixed integer programming formulation. It helps us categorize events based on their origin in the first step and their similarity in the second step. The active nature of the proposed clustering method makes it capable of identifying new clusters of events on an ongoing basis. The proposed unsupervised event detection and clustering methods are applied to real-world micro-PMU data. Results show that they can outperform the prevalent methods in the literature. These methods also facilitate our further analysis to identify important clusters of events that lead to unmasking several use cases that could be of value to the utility operator.},
	number = {4},
	urldate = {2021-09-17},
	journal = {IEEE Transactions on Smart Grid},
	author = {Aligholian, Armin and Shahsavari, Alireza and Stewart, Emma and Cortez, Ed and Mohsenian-Rad, Hamed},
	month = jul,
	year = {2021},
	note = {arXiv: 2007.15237},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Electrical Engineering and Systems Science - Signal Processing, Electrical Engineering and Systems Science - Systems and Control},
	pages = {3624--3636},
}

@article{jabri_space-time_2020,
	title = {Space-{Time} {Correspondence} as a {Contrastive} {Random} {Walk}},
	url = {http://arxiv.org/abs/2006.14613},
	abstract = {This paper proposes a simple self-supervised approach for learning a representation for visual correspondence from raw video. We cast correspondence as prediction of links in a space-time graph constructed from video. In this graph, the nodes are patches sampled from each frame, and nodes adjacent in time can share a directed edge. We learn a representation in which pairwise similarity defines transition probability of a random walk, so that long-range correspondence is computed as a walk along the graph. We optimize the representation to place high probability along paths of similarity. Targets for learning are formed without supervision, by cycle-consistency: the objective is to maximize the likelihood of returning to the initial node when walking along a graph constructed from a palindrome of frames. Thus, a single path-level constraint implicitly supervises chains of intermediate comparisons. When used as a similarity metric without adaptation, the learned representation outperforms the self-supervised state-of-the-art on label propagation tasks involving objects, semantic parts, and pose. Moreover, we demonstrate that a technique we call edge dropout, as well as self-supervised adaptation at test-time, further improve transfer for object-centric correspondence.},
	urldate = {2021-09-17},
	journal = {arXiv:2006.14613 [cs, eess]},
	author = {Jabri, Allan and Owens, Andrew and Efros, Alexei A.},
	month = dec,
	year = {2020},
	note = {arXiv: 2006.14613},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Electrical Engineering and Systems Science - Image and Video Processing},
}

@article{caron_emerging_2021,
	title = {Emerging {Properties} in {Self}-{Supervised} {Vision} {Transformers}},
	url = {http://arxiv.org/abs/2104.14294},
	abstract = {In this paper, we question if self-supervised learning provides new properties to Vision Transformer (ViT) that stand out compared to convolutional networks (convnets). Beyond the fact that adapting self-supervised methods to this architecture works particularly well, we make the following observations: first, self-supervised ViT features contain explicit information about the semantic segmentation of an image, which does not emerge as clearly with supervised ViTs, nor with convnets. Second, these features are also excellent k-NN classifiers, reaching 78.3\% top-1 on ImageNet with a small ViT. Our study also underlines the importance of momentum encoder, multi-crop training, and the use of small patches with ViTs. We implement our findings into a simple self-supervised method, called DINO, which we interpret as a form of self-distillation with no labels. We show the synergy between DINO and ViTs by achieving 80.1\% top-1 on ImageNet in linear evaluation with ViT-Base.},
	urldate = {2021-09-17},
	journal = {arXiv:2104.14294 [cs]},
	author = {Caron, Mathilde and Touvron, Hugo and Misra, Ishan and Jégou, Hervé and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
	month = may,
	year = {2021},
	note = {arXiv: 2104.14294},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{caron_emerging_2021-1,
	title = {Emerging {Properties} in {Self}-{Supervised} {Vision} {Transformers}},
	url = {http://arxiv.org/abs/2104.14294},
	abstract = {In this paper, we question if self-supervised learning provides new properties to Vision Transformer (ViT) that stand out compared to convolutional networks (convnets). Beyond the fact that adapting self-supervised methods to this architecture works particularly well, we make the following observations: first, self-supervised ViT features contain explicit information about the semantic segmentation of an image, which does not emerge as clearly with supervised ViTs, nor with convnets. Second, these features are also excellent k-NN classifiers, reaching 78.3\% top-1 on ImageNet with a small ViT. Our study also underlines the importance of momentum encoder, multi-crop training, and the use of small patches with ViTs. We implement our findings into a simple self-supervised method, called DINO, which we interpret as a form of self-distillation with no labels. We show the synergy between DINO and ViTs by achieving 80.1\% top-1 on ImageNet in linear evaluation with ViT-Base.},
	urldate = {2021-09-17},
	journal = {arXiv:2104.14294 [cs]},
	author = {Caron, Mathilde and Touvron, Hugo and Misra, Ishan and Jégou, Hervé and Mairal, Julien and Bojanowski, Piotr and Joulin, Armand},
	month = may,
	year = {2021},
	note = {arXiv: 2104.14294},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{bain_frozen_2021,
	title = {Frozen in {Time}: {A} {Joint} {Video} and {Image} {Encoder} for {End}-to-{End} {Retrieval}},
	shorttitle = {Frozen in {Time}},
	url = {http://arxiv.org/abs/2104.00650},
	abstract = {Our objective in this work is video-text retrieval - in particular a joint embedding that enables efficient text-to-video retrieval. The challenges in this area include the design of the visual architecture and the nature of the training data, in that the available large scale video-text training datasets, such as HowTo100M, are noisy and hence competitive performance is achieved only at scale through large amounts of compute. We address both these challenges in this paper. We propose an end-to-end trainable model that is designed to take advantage of both large-scale image and video captioning datasets. Our model is an adaptation and extension of the recent ViT and Timesformer architectures, and consists of attention in both space and time. The model is flexible and can be trained on both image and video text datasets, either independently or in conjunction. It is trained with a curriculum learning schedule that begins by treating images as 'frozen' snapshots of video, and then gradually learns to attend to increasing temporal context when trained on video datasets. We also provide a new video-text pretraining dataset WebVid-2M, comprised of over two million videos with weak captions scraped from the internet. Despite training on datasets that are an order of magnitude smaller, we show that this approach yields state-of-the-art results on standard downstream video-retrieval benchmarks including MSR-VTT, MSVD, DiDeMo and LSMDC.},
	urldate = {2021-09-16},
	journal = {arXiv:2104.00650 [cs]},
	author = {Bain, Max and Nagrani, Arsha and Varol, Gül and Zisserman, Andrew},
	month = apr,
	year = {2021},
	note = {arXiv: 2104.00650},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{zha_shifted_2021,
	title = {Shifted {Chunk} {Transformer} for {Spatio}-{Temporal} {Representational} {Learning}},
	url = {http://arxiv.org/abs/2108.11575},
	abstract = {Spatio-temporal representational learning has been widely adopted in various fields such as action recognition, video object segmentation, and action anticipation. Previous spatio-temporal representational learning approaches primarily employ ConvNets or sequential models,e.g., LSTM, to learn the intra-frame and inter-frame features. Recently, Transformer models have successfully dominated the study of natural language processing (NLP), image classification, etc. However, the pure-Transformer based spatio-temporal learning can be prohibitively costly on memory and computation to extract fine-grained features from a tiny patch. To tackle the training difficulty and enhance the spatio-temporal learning, we construct a shifted chunk Transformer with pure self-attention blocks. Leveraging the recent efficient Transformer design in NLP, this shifted chunk Transformer can learn hierarchical spatio-temporal features from a local tiny patch to a global video clip. Our shifted self-attention can also effectively model complicated inter-frame variances. Furthermore, we build a clip encoder based on Transformer to model long-term temporal dependencies. We conduct thorough ablation studies to validate each component and hyper-parameters in our shifted chunk Transformer, and it outperforms previous state-of-the-art approaches on Kinetics-400, Kinetics-600, UCF101, and HMDB51. Code and trained models will be released.},
	urldate = {2021-09-15},
	journal = {arXiv:2108.11575 [cs]},
	author = {Zha, Xuefan and Zhu, Wentao and Lv, Tingxun and Yang, Sen and Liu, Ji},
	month = aug,
	year = {2021},
	note = {arXiv: 2108.11575},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{ignat_whyact_2021,
	title = {{WhyAct}: {Identifying} {Action} {Reasons} in {Lifestyle} {Vlogs}},
	shorttitle = {{WhyAct}},
	url = {http://arxiv.org/abs/2109.02747},
	abstract = {We aim to automatically identify human action reasons in online videos. We focus on the widespread genre of lifestyle vlogs, in which people perform actions while verbally describing them. We introduce and make publicly available the WhyAct dataset, consisting of 1,077 visual actions manually annotated with their reasons. We describe a multimodal model that leverages visual and textual information to automatically infer the reasons corresponding to an action presented in the video.},
	urldate = {2021-09-15},
	journal = {arXiv:2109.02747 [cs]},
	author = {Ignat, Oana and Castro, Santiago and Miao, Hanwen and Li, Weiji and Mihalcea, Rada},
	month = sep,
	year = {2021},
	note = {arXiv: 2109.02747},
	keywords = {Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition, done.},
}

@inproceedings{alayrac_self-supervised_2020,
	title = {Self-{Supervised} {MultiModal} {Versatile} {Networks}},
	volume = {33},
	url = {https://proceedings.neurips.cc//paper/2020/hash/0060ef47b12160b9198302ebdb144dcf-Abstract.html},
	urldate = {2021-09-15},
	booktitle = {Advances in {Neural} {Information} {Processing} {Systems}},
	publisher = {Curran Associates, Inc.},
	author = {Alayrac, Jean-Baptiste and Recasens, Adria and Schneider, Rosalia and Arandjelović, Relja and Ramapuram, Jason and De Fauw, Jeffrey and Smaira, Lucas and Dieleman, Sander and Zisserman, Andrew},
	year = {2020},
	pages = {25--37},
}

@article{liu_video_2021,
	title = {Video {Swin} {Transformer}},
	url = {http://arxiv.org/abs/2106.13230},
	abstract = {The vision community is witnessing a modeling shift from CNNs to Transformers, where pure Transformer architectures have attained top accuracy on the major video recognition benchmarks. These video models are all built on Transformer layers that globally connect patches across the spatial and temporal dimensions. In this paper, we instead advocate an inductive bias of locality in video Transformers, which leads to a better speed-accuracy trade-off compared to previous approaches which compute self-attention globally even with spatial-temporal factorization. The locality of the proposed video architecture is realized by adapting the Swin Transformer designed for the image domain, while continuing to leverage the power of pre-trained image models. Our approach achieves state-of-the-art accuracy on a broad range of video recognition benchmarks, including on action recognition (84.9 top-1 accuracy on Kinetics-400 and 86.1 top-1 accuracy on Kinetics-600 with {\textasciitilde}20x less pre-training data and {\textasciitilde}3x smaller model size) and temporal modeling (69.6 top-1 accuracy on Something-Something v2). The code and models will be made publicly available at https://github.com/SwinTransformer/Video-Swin-Transformer.},
	urldate = {2021-09-14},
	journal = {arXiv:2106.13230 [cs]},
	author = {Liu, Ze and Ning, Jia and Cao, Yue and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Hu, Han},
	month = jun,
	year = {2021},
	note = {arXiv: 2106.13230},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{arnab_vivit_2021,
	title = {{ViViT}: {A} {Video} {Vision} {Transformer}},
	shorttitle = {{ViViT}},
	url = {http://arxiv.org/abs/2103.15691},
	abstract = {We present pure-transformer based models for video classification, drawing upon the recent success of such models in image classification. Our model extracts spatio-temporal tokens from the input video, which are then encoded by a series of transformer layers. In order to handle the long sequences of tokens encountered in video, we propose several, efficient variants of our model which factorise the spatial- and temporal-dimensions of the input. Although transformer-based models are known to only be effective when large training datasets are available, we show how we can effectively regularise the model during training and leverage pretrained image models to be able to train on comparatively small datasets. We conduct thorough ablation studies, and achieve state-of-the-art results on multiple video classification benchmarks including Kinetics 400 and 600, Epic Kitchens, Something-Something v2 and Moments in Time, outperforming prior methods based on deep 3D convolutional networks. To facilitate further research, we will release code and models.},
	urldate = {2021-09-14},
	journal = {arXiv:2103.15691 [cs]},
	author = {Arnab, Anurag and Dehghani, Mostafa and Heigold, Georg and Sun, Chen and Lučić, Mario and Schmid, Cordelia},
	month = mar,
	year = {2021},
	note = {arXiv: 2103.15691},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@inproceedings{rav-acha_making_2006,
	address = {New York, NY, USA},
	title = {Making a {Long} {Video} {Short}: {Dynamic} {Video} {Synopsis}},
	volume = {1},
	isbn = {978-0-7695-2597-6},
	shorttitle = {Making a {Long} {Video} {Short}},
	url = {http://ieeexplore.ieee.org/document/1640790/},
	doi = {10.1109/CVPR.2006.179},
	abstract = {The power of video over still images is the ability to represent dynamic activities. But video browsing and retrieval are inconvenient due to inherent spatio-temporal redundancies, where some time intervals may have no activity, or have activities that occur in a small image region. Video synopsis aims to provide a compact video representation, while preserving the essential activities of the original video.},
	language = {en},
	urldate = {2021-09-14},
	booktitle = {2006 {IEEE} {Computer} {Society} {Conference} on {Computer} {Vision} and {Pattern} {Recognition} - {Volume} 1 ({CVPR}'06)},
	publisher = {IEEE},
	author = {Rav-Acha, A. and Pritch, Y. and Peleg, S.},
	year = {2006},
	pages = {435--441},
}

@article{epstein_learning_2021,
	title = {Learning {Temporal} {Dynamics} from {Cycles} in {Narrated} {Video}},
	url = {http://arxiv.org/abs/2101.02337},
	abstract = {Learning to model how the world changes as time elapses has proven a challenging problem for the computer vision community. We propose a self-supervised solution to this problem using temporal cycle consistency jointly in vision and language, training on narrated video. Our model learns modality-agnostic functions to predict forward and backward in time, which must undo each other when composed. This constraint leads to the discovery of high-level transitions between moments in time, since such transitions are easily inverted and shared across modalities. We justify the design of our model with an ablation study on different configurations of the cycle consistency problem. We then show qualitatively and quantitatively that our approach yields a meaningful, high-level model of the future and past. We apply the learned dynamics model without further training to various tasks, such as predicting future action and temporally ordering sets of images.},
	urldate = {2021-09-10},
	journal = {arXiv:2101.02337 [cs]},
	author = {Epstein, Dave and Wu, Jiajun and Schmid, Cordelia and Sun, Chen},
	month = jan,
	year = {2021},
	note = {arXiv: 2101.02337},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{epstein_learning_2021-1,
	title = {Learning {Temporal} {Dynamics} from {Cycles} in {Narrated} {Video}},
	url = {http://arxiv.org/abs/2101.02337},
	abstract = {Learning to model how the world changes as time elapses has proven a challenging problem for the computer vision community. We propose a self-supervised solution to this problem using temporal cycle consistency jointly in vision and language, training on narrated video. Our model learns modality-agnostic functions to predict forward and backward in time, which must undo each other when composed. This constraint leads to the discovery of high-level transitions between moments in time, since such transitions are easily inverted and shared across modalities. We justify the design of our model with an ablation study on different configurations of the cycle consistency problem. We then show qualitatively and quantitatively that our approach yields a meaningful, high-level model of the future and past. We apply the learned dynamics model without further training to various tasks, such as predicting future action and temporally ordering sets of images.},
	urldate = {2021-09-10},
	journal = {arXiv:2101.02337 [cs]},
	author = {Epstein, Dave and Wu, Jiajun and Schmid, Cordelia and Sun, Chen},
	month = jan,
	year = {2021},
	note = {arXiv: 2101.02337},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{luo_clip4clip_2021,
	title = {{CLIP4Clip}: {An} {Empirical} {Study} of {CLIP} for {End} to {End} {Video} {Clip} {Retrieval}},
	shorttitle = {{CLIP4Clip}},
	url = {http://arxiv.org/abs/2104.08860},
	abstract = {Video-text retrieval plays an essential role in multi-modal research and has been widely used in many real-world web applications. The CLIP (Contrastive Language-Image Pre-training), an image-language pre-training model, has demonstrated the power of visual concepts learning from web collected image-text datasets. In this paper, we propose a CLIP4Clip model to transfer the knowledge of the CLIP model to video-language retrieval in an end-to-end manner. Several questions are investigated via empirical studies: 1) Whether image feature is enough for video-text retrieval? 2) How a post-pretraining on a large-scale video-text dataset based on the CLIP affect the performance? 3) What is the practical mechanism to model temporal dependency between video frames? And 4) The Hyper-parameters sensitivity of the model on video-text retrieval task. Extensive experimental results present that the CLIP4Clip model transferred from the CLIP can achieve SOTA results on various video-text retrieval datasets, including MSR-VTT, MSVC, LSMDC, ActivityNet, and DiDeMo. We release our code at https://github.com/ArrowLuo/CLIP4Clip.},
	urldate = {2021-09-09},
	journal = {arXiv:2104.08860 [cs]},
	author = {Luo, Huaishao and Ji, Lei and Zhong, Ming and Chen, Yang and Lei, Wen and Duan, Nan and Li, Tianrui},
	month = may,
	year = {2021},
	note = {arXiv: 2104.08860},
	keywords = {Computer Science - Computer Vision and Pattern Recognition},
}

@article{radford_learning_2021,
	title = {Learning {Transferable} {Visual} {Models} {From} {Natural} {Language} {Supervision}},
	url = {http://arxiv.org/abs/2103.00020},
	abstract = {State-of-the-art computer vision systems are trained to predict a fixed set of predetermined object categories. This restricted form of supervision limits their generality and usability since additional labeled data is needed to specify any other visual concept. Learning directly from raw text about images is a promising alternative which leverages a much broader source of supervision. We demonstrate that the simple pre-training task of predicting which caption goes with which image is an efficient and scalable way to learn SOTA image representations from scratch on a dataset of 400 million (image, text) pairs collected from the internet. After pre-training, natural language is used to reference learned visual concepts (or describe new ones) enabling zero-shot transfer of the model to downstream tasks. We study the performance of this approach by benchmarking on over 30 different existing computer vision datasets, spanning tasks such as OCR, action recognition in videos, geo-localization, and many types of fine-grained object classification. The model transfers non-trivially to most tasks and is often competitive with a fully supervised baseline without the need for any dataset specific training. For instance, we match the accuracy of the original ResNet-50 on ImageNet zero-shot without needing to use any of the 1.28 million training examples it was trained on. We release our code and pre-trained model weights at https://github.com/OpenAI/CLIP.},
	urldate = {2021-09-09},
	journal = {arXiv:2103.00020 [cs]},
	author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
	month = feb,
	year = {2021},
	note = {arXiv: 2103.00020},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning},
}

@article{lei_qvhighlights_2021,
	title = {{QVHighlights}: {Detecting} {Moments} and {Highlights} in {Videos} via {Natural} {Language} {Queries}},
	shorttitle = {{QVHighlights}},
	url = {http://arxiv.org/abs/2107.09609},
	abstract = {Detecting customized moments and highlights from videos given natural language (NL) user queries is an important but under-studied topic. One of the challenges in pursuing this direction is the lack of annotated data. To address this issue, we present the Query-based Video Highlights (QVHighlights) dataset. It consists of over 10,000 YouTube videos, covering a wide range of topics, from everyday activities and travel in lifestyle vlog videos to social and political activities in news videos. Each video in the dataset is annotated with: (1) a human-written free-form NL query, (2) relevant moments in the video w.r.t. the query, and (3) five-point scale saliency scores for all query-relevant clips. This comprehensive annotation enables us to develop and evaluate systems that detect relevant moments as well as salient highlights for diverse, flexible user queries. We also present a strong baseline for this task, Moment-DETR, a transformer encoder-decoder model that views moment retrieval as a direct set prediction problem, taking extracted video and query representations as inputs and predicting moment coordinates and saliency scores end-to-end. While our model does not utilize any human prior, we show that it performs competitively when compared to well-engineered architectures. With weakly supervised pretraining using ASR captions, Moment-DETR substantially outperforms previous methods. Lastly, we present several ablations and visualizations of Moment-DETR. Data and code is publicly available at https://github.com/jayleicn/moment\_detr},
	urldate = {2021-09-07},
	journal = {arXiv:2107.09609 [cs]},
	author = {Lei, Jie and Berg, Tamara L. and Bansal, Mohit},
	month = jul,
	year = {2021},
	note = {arXiv: 2107.09609
version: 1},
	keywords = {Computer Science - Artificial Intelligence, Computer Science - Computation and Language, Computer Science - Computer Vision and Pattern Recognition},
}

@article{lu_few-shot_2021,
	title = {Few-{Shot} {Action} {Recognition} with {Compromised} {Metric} via {Optimal} {Transport}},
	journal = {arXiv preprint arXiv:2104.03737},
	author = {Lu, Su and Ye, Han-Jia and Zhan, De-Chuan},
	year = {2021},
}

@article{lu_few-shot_2021-1,
	title = {Few-{Shot} {Action} {Recognition} with {Compromised} {Metric} via {Optimal} {Transport}},
	journal = {arXiv preprint arXiv:2104.03737},
	author = {Lu, Su and Ye, Han-Jia and Zhan, De-Chuan},
	year = {2021},
}

@inproceedings{vinyals_matching_2016,
	title = {Matching {Networks} for {One} {Shot} {Learning}},
	volume = {29},
	url = {https://proceedings.neurips.cc/paper/2016/file/90e1357833654983612fb05e3ec9148c-Paper.pdf},
	booktitle = {Advances in {Neural} {Information} {Processing} {Systems}},
	publisher = {Curran Associates, Inc.},
	author = {Vinyals, Oriol and Blundell, Charles and Lillicrap, Timothy and kavukcuoglu, koray and Wierstra, Daan},
	editor = {Lee, D. and Sugiyama, M. and Luxburg, U. and Guyon, I. and Garnett, R.},
	year = {2016},
}

@misc{noauthor_tinkercad_nodate,
	title = {Tinkercad},
	url = {tinkercad.com},
}

@article{ostertagova_modelling_2012,
	title = {Modelling using polynomial regression},
	volume = {48},
	journal = {Procedia Engineering},
	author = {Ostertagová, Eva},
	year = {2012},
	note = {Publisher: Elsevier},
	pages = {500--506},
}

@article{verbois_probabilistic_2018,
	title = {Probabilistic forecasting of day-ahead solar irradiance using quantile gradient boosting},
	volume = {173},
	journal = {Solar Energy},
	author = {Verbois, Hadrien and Rusydi, Andrivo and Thiery, Alexandre},
	year = {2018},
	note = {Publisher: Elsevier},
	pages = {313--327},
}

@article{yu_quantile_2003,
	title = {Quantile regression: applications and current research areas},
	volume = {52},
	shorttitle = {Quantile regression},
	number = {3},
	journal = {Journal of the Royal Statistical Society: Series D (The Statistician)},
	author = {Yu, Keming and Lu, Zudi and Stander, Julian},
	year = {2003},
	note = {Publisher: Wiley Online Library},
	pages = {331--350},
}

@article{joye_magnitude_2011,
	title = {Magnitude and oxidation potential of hydrocarbon gases released from the {BP} oil well blowout},
	volume = {4},
	copyright = {2011 Nature Publishing Group},
	issn = {1752-0908},
	url = {https://www.nature.com/articles/ngeo1067},
	doi = {10.1038/ngeo1067},
	abstract = {The deep-sea oil spill in the Gulf of Mexico released large quantities of oil and gaseous hydrocarbons into the deep ocean. Calculations using published estimates of the volume of oil released suggest that up to 500,000 t of gases such as methane were released into the deep ocean.},
	language = {en},
	number = {3},
	urldate = {2021-03-01},
	journal = {Nature Geoscience},
	author = {Joye, Samantha B. and MacDonald, Ian R. and Leifer, Ira and Asper, Vernon},
	month = mar,
	year = {2011},
	note = {Number: 3
Publisher: Nature Publishing Group},
	pages = {160--164},
}

@book{fingas_handbook_2014,
	title = {Handbook of {Oil} {Spill} {Science} and {Technology}},
	isbn = {978-1-118-98996-8},
	abstract = {Provides a scientific basis for the cleanup and for the assessment of oil spills  Enables Non-scientific officers to understand the science they use on a daily basis Multi-disciplinary approach covering fields as diverse as biology, microbiology, chemistry, physics, oceanography and toxicology Covers the science of oil spills from risk analysis to cleanup and through the effects on the environment Includes case studies examining and analyzing spills, such as Tasman Spirit oil spill on the Karachi Coast, and provides lessons to prevent these in the future},
	language = {en},
	publisher = {John Wiley \& Sons},
	author = {Fingas, Merv},
	month = dec,
	year = {2014},
	note = {Google-Books-ID: zhcHBgAAQBAJ},
	keywords = {Science / Life Sciences / Ecology, Technology \& Engineering / Environmental / General},
}

@misc{noauthor_makeit_nodate,
	title = {Makeit {Pro}-{M} {3D} printer},
	url = {makeit-3d.com},
}

@misc{noauthor_mattercontrol_nodate,
	title = {{MatterControl} software},
	url = {matterhackers.com},
}

@article{noaa_data_2020,
	series = {1578674392},
	title = {Data {Integration} {Visualization} {Exploration} and {Reporting} ({DIVER}). {Deepwater} {Horizon} {Natural} {Resource} and {Damage} {Assessment} data.  {Last} accessed on 1/10/2020 at https://www.diver.orr.noaa.gov/deepwater-horizon-nrda-data},
	author = {NOAA},
	year = {2020},
}

@patent{noauthor_core_nodate,
	address = {GitHub},
	title = {Core {ML} {Community} {Tools}},
	author = {, Apple},
}

@techreport{fantasia_investigation_1971,
	title = {Investigation of {Oil} {Fluorescence} as a {Technique} for the {Remote} {Sensing} of {Oil} {Spills}},
	institution = {United States. Coast Guard},
	author = {Fantasia, John F. and Hard, Thomas Michael and Ingrao, Hector C.},
	year = {1971},
}

@article{keizer_detection_1973,
	title = {Detection of trace amounts of oil in sea water by fluorescence spectroscopy},
	volume = {30},
	number = {8},
	journal = {Journal of the Fisheries Board of Canada},
	author = {Keizer, P. D. and Gordon Jr, D. C.},
	year = {1973},
	note = {Publisher: NRC Research Press},
	pages = {1039--1046},
}

@article{white_methods_2016,
	title = {Methods of oil detection in response to the {Deepwater} {Horizon} oil spill},
	volume = {29},
	number = {3},
	journal = {Oceanography},
	author = {White, Helen K. and Conmy, Robyn N. and MacDonald, Ian R. and Reddy, Christopher M.},
	year = {2016},
	note = {Publisher: JSTOR},
	pages = {76--87},
}

@article{clark_method_2010,
	title = {A method for quantitative mapping of thick oil spills using imaging spectroscopy},
	volume = {1167},
	number = {2010},
	journal = {US Geological Survey Open-File Report},
	author = {Clark, Roger N. and Swayze, Gregg A. and Leifer, Ira and Livo, K. Eric and Kokaly, Raymond and Hoefen, Todd and Lundeen, Sarah and Eastwood, Michael and Green, Robert O. and Pearson, Neil},
	year = {2010},
	note = {Publisher: Citeseer},
	pages = {1--51},
}

@misc{noauthor_rapid_nodate,
	title = {A {Rapid}, {Fluorescence}-{Based} {Field} {Screening} {Technique} for {Organic} {Species} in {Soil} and {Water} {Matrices} {\textbar} {SpringerLink}},
	url = {https://link.springer.com/article/10.1007/s00128-016-1771-1},
	urldate = {2020-08-10},
}

@article{wei_fluorescent_2013,
	title = {Fluorescent imaging of single nanoparticles and viruses on a smart phone},
	volume = {7},
	number = {10},
	journal = {ACS nano},
	author = {Wei, Qingshan and Qi, Hangfei and Luo, Wei and Tseng, Derek and Ki, So Jung and Wan, Zhe and Göröcs, Zoltán and Bentolila, Laurent A. and Wu, Ting-Ting and Sun, Ren},
	year = {2013},
	note = {Publisher: ACS Publications},
	pages = {9147--9155},
}

@article{granica_analytical_2019,
	title = {Analytical aspects of smart (phone) fluorometric measurements},
	volume = {197},
	journal = {Talanta},
	author = {Granica, Mateusz and Tymecki, {\textbackslash}Lukasz},
	year = {2019},
	note = {Publisher: Elsevier},
	pages = {319--325},
}

@article{gunda_artificial_2019,
	title = {Artificial intelligence based mobile application for water quality monitoring},
	volume = {166},
	number = {9},
	journal = {Journal of The Electrochemical Society},
	author = {Gunda, Naga Siva Kumar and Gautam, Siddharth Hariharan and Mitra, Sushanta K.},
	year = {2019},
	note = {Publisher: IOP Publishing},
	pages = {B3031},
}

@article{seo_smartphone_2019,
	title = {Smartphone compatible on-site fluorescence analyzer for spilled crude oil based on {CMOS} image sensor},
	volume = {289},
	journal = {Sensors and Actuators B: Chemical},
	author = {Seo, Dongmin and Oh, Sangwoo and Shin, Sanghoon and Lee, Moonjin and Hwang, Yongha and Seo, Sungkyu},
	year = {2019},
	note = {Publisher: Elsevier},
	pages = {93--99},
}

@article{nixon_predictive_2015,
	title = {Predictive modeling of subsurface shoreline oil encounter probability from the {Exxon} {Valdez} oil spill in {Prince} {William} {Sound}, {Alaska}},
	volume = {49},
	number = {7},
	journal = {Environmental Science \& Technology},
	author = {Nixon, Zachary and Michel, Jacqueline},
	year = {2015},
	note = {Publisher: ACS Publications},
	pages = {4354--4361},
}

@article{zhou_wang_image_2004,
	title = {Image quality assessment: from error visibility to structural similarity},
	volume = {13},
	doi = {10.1109/TIP.2003.819861},
	number = {4},
	journal = {IEEE Transactions on Image Processing},
	author = {{Zhou Wang} and Bovik, A. C. and Sheikh, H. R. and Simoncelli, E. P.},
	month = apr,
	year = {2004},
	keywords = {Algorithms, Automated, Computer-Assisted, Data Interpretation, Data mining, Degradation, Humans, Hypermedia, Image Enhancement, Image Interpretation, Image quality, Indexes, Information Storage and Retrieval, JPEG, JPEG2000, Layout, Models, Pattern Recognition, Quality Control, Quality assessment, Reproducibility of Results, Sensitivity and Specificity, Signal Processing, Statistical, Subtraction Technique, Transform coding, Visual perception, Visual system, data compression, distorted image, error sensitivity, error visibility, human visual perception, human visual system, image coding, image compression, image database, perceptual image quality assessment, reference image, structural information, structural similarity index, visual perception},
	pages = {600--612},
}

@inproceedings{kim_deep_2019,
	title = {Deep {Metric} {Learning} {Beyond} {Binary} {Supervision}},
	booktitle = {The {IEEE} {Conference} on {Computer} {Vision} and {Pattern} {Recognition} ({CVPR})},
	author = {Kim, Sungyeon and Seo, Minkyo and Laptev, Ivan and Cho, Minsu and Kwak, Suha},
	month = jun,
	year = {2019},
}

@inproceedings{wu_pcanet_2017,
	address = {Cham},
	title = {{PCANet} for {Color} {Image} {Classification} in {Various} {Color} {Spaces}},
	isbn = {978-3-319-68542-7},
	abstract = {Principal component analysis network (PCANet), which is a recently proposed novel deep learning algorithm, has aroused the interest of a wide variety of researchers. In this paper, we evaluate the performance of PCANet in various color spaces on different types of color image dataset. Experimental results on CURet texture database, UC Merced land use database, and Georgia Tech face database show that Luminance and Chrominance based principal component analysis network outperforms other color spaces in the vast majority of cases. Therefore, when dealing with the problem of color image dataset classification, Luminance and Chrominance based principal component network is recommended.},
	booktitle = {Cloud {Computing} and {Security}},
	publisher = {Springer International Publishing},
	author = {Wu, Jiasong and Qiu, Shijie and Zeng, Rui and Senhadji, Lotfi and Shu, Huazhong},
	editor = {Sun, Xingming and Chao, Han-Chieh and You, Xingang and Bertino, Elisa},
	year = {2017},
	pages = {494--505},
}

@inproceedings{fu_deep_2018,
	title = {Deep {Ordinal} {Regression} {Network} for {Monocular} {Depth} {Estimation}},
	volume = {2018},
	doi = {10.1109/CVPR.2018.00214},
	booktitle = {Proceedings. {IEEE} {Computer} {Society} {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	author = {Fu, Huan and Gong, Mingming and Wang, Chaohui and Batmanghelich, Kayhan and Tao, Dacheng},
	year = {2018},
	pages = {2002--2011},
}

@article{krizhevsky_learning_2012,
	title = {Learning {Multiple} {Layers} of {Features} from {Tiny} {Images}},
	journal = {University of Toronto},
	author = {Krizhevsky, Alex},
	year = {2012},
}

@article{sindagi_ha-ccn_2020,
	title = {{HA}-{CCN}: {Hierarchical} {Attention}-{Based} {Crowd} {Counting} {Network}},
	volume = {29},
	doi = {10.1109/TIP.2019.2928634},
	journal = {IEEE Transactions on Image Processing},
	author = {Sindagi, V. A. and Patel, V. M.},
	year = {2020},
	keywords = {Adaptation models, CNN, Crowd counting, Decoding, GAM, HA-CCN, Image segmentation, SAM, Semantics, Supervised learning, Task analysis, Training, VGG16 network, channel-wise information, convolutional neural nets, convolutional neural network, crowd analytics, feature extraction, global attention modules, hierarchical attention-based crowd counting network, image annotation, image segmentation, infusing spatial segmentation information, labor intensive point-wise annotations, learning (artificial intelligence), low-level features, single image-based crowd counting, single-step training framework, spatial attention module, weakly supervised learning},
	pages = {323--335},
}

@inproceedings{chen_sca-cnn_2017,
	title = {Sca-cnn: {Spatial} and channel-wise attention in convolutional networks for image captioning},
	booktitle = {Proceedings of the {IEEE} conference on computer vision and pattern recognition},
	author = {Chen, Long and Zhang, Hanwang and Xiao, Jun and Nie, Liqiang and Shao, Jian and Liu, Wei and Chua, Tat-Seng},
	year = {2017},
	pages = {5659--5667},
}

@article{rafegas_color_2018,
	title = {Color encoding in biologically-inspired convolutional neural networks},
	volume = {151},
	issn = {0042-6989},
	url = {http://www.sciencedirect.com/science/article/pii/S0042698918300592},
	doi = {https://doi.org/10.1016/j.visres.2018.03.010},
	abstract = {Convolutional Neural Networks have been proposed as suitable frameworks to model biological vision. Some of these artificial networks showed representational properties that rival primate performances in object recognition. In this paper we explore how color is encoded in a trained artificial network. It is performed by estimating a color selectivity index for each neuron, which allows us to describe the neuron activity to a color input stimuli. The index allows us to classify whether they are color selective or not and if they are of a single or double color. We have determined that all five convolutional layers of the network have a large number of color selective neurons. Color opponency clearly emerges in the first layer, presenting 4 main axes (Black-White, Red-Cyan, Blue-Yellow and Magenta-Green), but this is reduced and rotated as we go deeper into the network. In layer 2 we find a denser hue sampling of color neurons and opponency is reduced almost to one new main axis, the Bluish-Orangish coinciding with the dataset bias. In layers 3, 4 and 5 color neurons are similar amongst themselves, presenting different type of neurons that detect specific colored objects (e.g., orangish faces), specific surrounds (e.g., blue sky) or specific colored or contrasted object-surround configurations (e.g. blue blob in a green surround). Overall, our work concludes that color and shape representation are successively entangled through all the layers of the studied network, revealing certain parallelisms with the reported evidences in primate brains that can provide useful insight into intermediate hierarchical spatio-chromatic representations.},
	journal = {Vision Research},
	author = {Rafegas, Ivet and Vanrell, Maria},
	year = {2018},
	keywords = {Color coding, Computer vision, Convolutional neural networks, Deep learning},
	pages = {7 -- 17},
}

@inproceedings{zejia_zheng_compact_2015,
	title = {Compact deep neural networks for device based image classification},
	doi = {10.1109/ICMEW.2015.7169768},
	abstract = {Convolutional Neural Network (CNN) is efficient in learning hierarchical features from large image datasets, but its model complexity and large memory foot prints are preventing it from being deployed to devices without a server back-end support. Modern CNNs are always trained on GPUs or even GPU clusters with high speed computation capability due to the immense size of the network. A device based deep learning CNN engine for image classification can be very useful for situations where server back-end is either not available, or its communication link is weak and unreliable. Methods on regulating the size of the network, on the other hand, are rarely studied. In this paper we present a novel compact architecture that minimizes the number and complexity of lower level kernels in a CNN by separating the color information from the original image. A 9-patch histogram extractor is built to exploit the unused color information. A high level classifier is then used to learn the combined features obtained from the compact CNN that was trained only on grayscale image with limited number of kernels, and the histogram extractor. We apply our compact architecture to Samsung Mobile Image Dataset for image classification. The proposed solution has a recognition accuracy on par with the state of the art CNNs, while achieving significant reduction in model memory foot print. With this advantage, our model is being deployed to the mobile devices.},
	booktitle = {2015 {IEEE} {International} {Conference} on {Multimedia} {Expo} {Workshops} ({ICMEW})},
	author = {{Zejia Zheng} and {Zhu Li} and Nagar, A. and {Kyungmo Park}},
	month = jun,
	year = {2015},
	keywords = {9-patch histogram extractor, Accuracy, Computer architecture, GPU clusters, Image color analysis, Image recognition, Kernel, Lead, Mobile communication, Samsung mobile image dataset, compact architecture, compact deep neural networks, convolutional neural network, device based deep learning CNN engine, device based image classification, feature extraction, grayscale image, hierarchical feature extraction, high level classifier, high speed computation capability, image classification, image color, image colour analysis, large image datasets, learning (artificial intelligence), lower level kernels, memory foot prints, mobile devices, mobile radio, model complexity, neural nets, recognition accuracy, server back-end support, visual databases},
	pages = {1--6},
}

@inproceedings{niu_ordinal_2016,
	title = {Ordinal {Regression} with {Multiple} {Output} {CNN} for {Age} {Estimation}},
	doi = {10.1109/CVPR.2016.532},
	abstract = {To address the non-stationary property of aging patterns, age estimation can be cast as an ordinal regression problem. However, the processes of extracting features and learning a regression model are often separated and optimized independently in previous work. In this paper, we propose an End-to-End learning approach to address ordinal regression problems using deep Convolutional Neural Network, which could simultaneously conduct feature learning and regression modeling. In particular, an ordinal regression problem is transformed into a series of binary classification sub-problems. And we propose a multiple output CNN learning algorithm to collectively solve these classification sub-problems, so that the correlation between these tasks could be explored. In addition, we publish an Asian Face Age Dataset (AFAD) containing more than 160K facial images with precise age ground-truths, which is the largest public age dataset to date. To the best of our knowledge, this is the first work to address ordinal regression problems by using CNN, and achieves the state-of-the-art performance on both the MORPH and AFAD datasets.},
	booktitle = {2016 {IEEE} {Conference} on {Computer} {Vision} and {Pattern} {Recognition} ({CVPR})},
	author = {Niu, Z. and Zhou, M. and Wang, L. and Gao, X. and Hua, G.},
	month = jun,
	year = {2016},
	keywords = {AFAD, AFAD datasets, Aging, Asian face age dataset, Estimation, Face, Feature extraction, MORPH datasets, Measurement, Support vector machines, Training data, age estimation, age ground-truths, aging pattern nonstationary property, binary classification subproblems, deep convolutional neural network, end-to-end learning approach, face recognition, feature extraction, feature learning, feedforward neural nets, image classification, learning (artificial intelligence), multiple output CNN learning algorithm, ordinal regression, regression analysis, regression model learning},
	pages = {4920--4928},
}

@inproceedings{zhang_image_2018,
	title = {Image super-resolution using very deep residual channel attention networks},
	booktitle = {Proceedings of the {European} {Conference} on {Computer} {Vision} ({ECCV})},
	author = {Zhang, Yulun and Li, Kunpeng and Li, Kai and Wang, Lichen and Zhong, Bineng and Fu, Yun},
	year = {2018},
	pages = {286--301},
}

@inproceedings{he_deep_2016,
	title = {Deep residual learning for image recognition},
	booktitle = {Proceedings of the {IEEE} conference on computer vision and pattern recognition},
	author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
	year = {2016},
	pages = {770--778},
}

@inproceedings{salman_regression_2012,
	title = {Regression as classification},
	doi = {10.1109/SECon.2012.6196887},
	abstract = {The paper presents how solving regression problems can be posed as finding solutions to multiclass classification tasks. The accuracy (averaged over several benchmarking data sets used in this study) of an approximating (hyper)surface to the data points over a given high-dimensional input space created by a nonlinear multiclass classifier is slightly superior to the solution obtained by regression (hyper)surface. In terms of the CPU time needed for training i.e., for tuning the hyperparameters of the models, the nonlinear classifier shows significant (order of magnitudes for large datasets) advantages too. Here, the support vector machine (SVM) has been solving given regression problems as a classic SVM regressor and as the SVM classifier. In order to transform a regression problem into a classification task two possible discretizations of a continuous output (target) vector y are presented and compared. A very strict double (nested) cross-validation technique has been used for measuring performances of regression and multiclass classification SVMs. A novel approach and the experimental results obtained for five benchmarking regression data sets warrant both further theoretical investigations and broad application in practice.},
	booktitle = {2012 {Proceedings} of {IEEE} {Southeastcon}},
	author = {Salman, R. and Kecman, V.},
	month = mar,
	year = {2012},
	keywords = {Accuracy, Benchmark testing, CPU time, Classification, Concrete, Data mining, Discretization, Machine-Learning, Regression, SVM, Servomotors, Support Vector Machine, Support vector machine classification, Training, data points, nonlinear multiclass classifier, pattern classification, regression analysis, regression hypersurface, support vector machine, support vector machines},
	pages = {1--6},
}

@article{tolias_particular_2015,
	title = {Particular object retrieval with integral max-pooling of {CNN} activations},
	journal = {arXiv preprint arXiv:1511.05879},
	author = {Tolias, Giorgos and Sicre, Ronan and Jégou, Hervé},
	year = {2015},
}

@book{canziani_analysis_2016,
	title = {An {Analysis} of {Deep} {Neural} {Network} {Models} for {Practical} {Applications}},
	author = {Canziani, Alfredo and Paszke, Adam and Culurciello, Eugenio},
	year = {2016},
	note = {\_eprint: 1605.07678},
}

@inproceedings{chiu_see_2015,
	title = {See the {Difference}: {Direct} {Pre}-{Image} {Reconstruction} and {Pose} {Estimation} by {Differentiating} {HOG}},
	doi = {10.1109/ICCV.2015.61},
	abstract = {The Histogram of Oriented Gradient (HOG) descriptor has led to many advances in computer vision over the last decade and is still part of many state of the art approaches. We realize that the associated feature computation is piecewise differentiable and therefore many pipelines which build on HOG can be made differentiable. This lends to advanced introspection as well as opportunities for end-to-end optimization. We present our implementation of ΔHOG based on the auto-differentiation toolbox Chumpy [18] and show applications to pre-image visualization and pose estimation which extends the existing differentiable renderer OpenDR [19] pipeline. Both applications improve on the respective state-of-the-art HOG approaches.},
	booktitle = {2015 {IEEE} {International} {Conference} on {Computer} {Vision} ({ICCV})},
	author = {Chiu, W. and Fritz, M.},
	year = {2015},
	keywords = {Computational modeling, Design automation, HOG differentiation, Histograms, Pipelines, Solid modeling, Visualization, computer vision, end-to-end optimization, gradient methods, histogram of oriented gradient, image reconstruction, optimisation, pose estimation, pre-image reconstruction},
	pages = {468--476},
}

@article{marra_deep_2018,
	title = {A deep learning approach for iris sensor model identification},
	volume = {113},
	issn = {0167-8655},
	url = {http://www.sciencedirect.com/science/article/pii/S0167865517301186},
	doi = {https://doi.org/10.1016/j.patrec.2017.04.010},
	abstract = {The aim of this paper is to propose an algorithm based on convolutional neural networks (CNN) for iris sensor model identification. This task is important in forensics applications as well as to face the problem of sensor interoperability in large scale systems. When different sensor models are involved in a recognition system, in fact, the overall performance can strongly decrease. A possible solution consists in first identifying the sensor model and then mapping the features extracted from the image from one sensor to the other. To keep low both complexity and memory requirements we propose a simple network architecture and the use of transfer learning to speed-up the training phase and tackle the problem of limited training set availability. Experiments are carried out on several public iris databases. First, we show that the proposed solution outperforms the state-of-the art approaches used for the model identification task. Then, we test the performance of a biometric recognition system and show that improving the sensor model identification step can benefit the iris sensor interoperability.},
	journal = {Pattern Recognition Letters},
	author = {Marra, Francesco and Poggi, Giovanni and Sansone, Carlo and Verdoliva, Luisa},
	year = {2018},
	keywords = {Convolutional Neural Networks, Forensics, Iris sensor identification, Iris sensor interoperability},
	pages = {46 -- 53},
}

@inproceedings{rafegas_color_2017,
	title = {Color {Representation} in {CNNs}: {Parallelisms} with {Biological} {Vision}},
	url = {https://doi.org/10.1109/ICCVW.2017.318},
	doi = {10.1109/ICCVW.2017.318},
	booktitle = {2017 {IEEE} {International} {Conference} on {Computer} {Vision} {Workshops}, {ICCV} {Workshops} 2017, {Venice}, {Italy}, {October} 22-29, 2017},
	author = {Rafegas, Ivet and Vanrell, María},
	year = {2017},
	pages = {2697--2705},
}

@inproceedings{niu_ordinal_2016-1,
	title = {Ordinal {Regression} with {Multiple} {Output} {CNN} for {Age} {Estimation}},
	doi = {10.1109/CVPR.2016.532},
	abstract = {To address the non-stationary property of aging patterns, age estimation can be cast as an ordinal regression problem. However, the processes of extracting features and learning a regression model are often separated and optimized independently in previous work. In this paper, we propose an End-to-End learning approach to address ordinal regression problems using deep Convolutional Neural Network, which could simultaneously conduct feature learning and regression modeling. In particular, an ordinal regression problem is transformed into a series of binary classification sub-problems. And we propose a multiple output CNN learning algorithm to collectively solve these classification sub-problems, so that the correlation between these tasks could be explored. In addition, we publish an Asian Face Age Dataset (AFAD) containing more than 160K facial images with precise age ground-truths, which is the largest public age dataset to date. To the best of our knowledge, this is the first work to address ordinal regression problems by using CNN, and achieves the state-of-the-art performance on both the MORPH and AFAD datasets.},
	booktitle = {2016 {IEEE} {Conference} on {Computer} {Vision} and {Pattern} {Recognition} ({CVPR})},
	author = {Niu, Z. and Zhou, M. and Wang, L. and Gao, X. and Hua, G.},
	month = jun,
	year = {2016},
	keywords = {AFAD, AFAD datasets, Aging, Asian face age dataset, Estimation, Face, Feature extraction, MORPH datasets, Measurement, Support vector machines, Training data, age estimation, age ground-truths, aging pattern nonstationary property, binary classification subproblems, deep convolutional neural network, end-to-end learning approach, face recognition, feature extraction, feature learning, feedforward neural nets, image classification, learning (artificial intelligence), multiple output CNN learning algorithm, ordinal regression, regression analysis, regression model learning},
	pages = {4920--4928},
}

@book{lathuiliere_comprehensive_2018,
	title = {A {Comprehensive} {Analysis} of {Deep} {Regression}},
	author = {Lathuilière, Stéphane and Mesejo, Pablo and Alameda-Pineda, Xavier and Horaud, Radu},
	year = {2018},
	note = {\_eprint: 1803.08450},
}

@article{larsson_colorization_2017,
	title = {Colorization as a {Proxy} {Task} for {Visual} {Understanding}},
	journal = {2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
	author = {Larsson, Gustav and Maire, Michael and Shakhnarovich, Gregory},
	year = {2017},
	pages = {840--849},
}

@inproceedings{szegedy_going_2015,
	title = {Going deeper with convolutions},
	doi = {10.1109/CVPR.2015.7298594},
	abstract = {We propose a deep convolutional neural network architecture codenamed Inception that achieves the new state of the art for classification and detection in the ImageNet Large-Scale Visual Recognition Challenge 2014 (ILSVRC14). The main hallmark of this architecture is the improved utilization of the computing resources inside the network. By a carefully crafted design, we increased the depth and width of the network while keeping the computational budget constant. To optimize quality, the architectural decisions were based on the Hebbian principle and the intuition of multi-scale processing. One particular incarnation used in our submission for ILSVRC14 is called GoogLeNet, a 22 layers deep network, the quality of which is assessed in the context of classification and detection.},
	booktitle = {2015 {IEEE} {Conference} on {Computer} {Vision} and {Pattern} {Recognition} ({CVPR})},
	author = {Szegedy, C. and {Wei Liu} and {Yangqing Jia} and Sermanet, P. and Reed, S. and Anguelov, D. and Erhan, D. and Vanhoucke, V. and Rabinovich, A.},
	month = jun,
	year = {2015},
	keywords = {Computer architecture, Computer vision, Convolutional codes, Hebbian learning, Hebbian principle, Neural networks, Object detection, Sparse matrices, Visualization, architectural decision, convolution, convolutional neural network architecture, decision making, feature extraction, image classification, neural net architecture, object classification, object detection, resource allocation, resource utilization},
	pages = {1--9},
}

@inproceedings{rebetez_augmenting_2016,
	title = {Augmenting a convolutional neural network with local histograms - {A} case study in crop classification from high-resolution {UAV} imagery},
	booktitle = {{ESANN}},
	author = {Rebetez, Julien and Satizábal, Héctor F. and Mota, Matteo and Noll, Dorothea and Büchi, Lucie and Wendling, Marina and Cannelle, Bertrand and Pérez-Uribe, Andrés and Burgos, Stéphane},
	year = {2016},
}

@inproceedings{engilberge_color_2017,
	title = {Color representation in deep neural networks},
	doi = {10.1109/ICIP.2017.8296790},
	abstract = {Convolutional neural networks are top-performers on image classification tasks. Understanding how they make use of color information in images may be useful for various tasks. In this paper we analyze the representation learned by a popular CNN to detect and characterize color-related features. We confirm the existence of some object- and color-specific units, as well as the effect of layer-depth on color-sensitivity and class-invariance.},
	booktitle = {2017 {IEEE} {International} {Conference} on {Image} {Processing} ({ICIP})},
	author = {Engilberge, M. and Collins, E. and Süsstrunk, S.},
	month = sep,
	year = {2017},
	keywords = {CNN, Color information, Color sensitivity, Convolutional Neural Networks, Convolutional neural networks, Covariance matrices, Deep learning, Feature extraction, Image color analysis, Indexes, Latent features, Sensitivity, Task analysis, class-invariance, color information, color representation, color-sensitivity, color-specific units, convolution, convolutional neural networks, deep neural networks, feedforward neural nets, image classification, image classification tasks, image colour analysis, image representation},
	pages = {2786--2790},
}

@book{nam_modelling_2017,
	title = {Modelling the {Scene} {Dependent} {Imaging} in {Cameras} with a {Deep} {Neural} {Network}},
	author = {Nam, Seonghyeon and Kim, Seon Joo},
	year = {2017},
	note = {\_eprint: 1707.08350},
}

@inproceedings{wang_learnable_2016,
	address = {Cham},
	title = {Learnable {Histogram}: {Statistical} {Context} {Features} for {Deep} {Neural} {Networks}},
	isbn = {978-3-319-46448-0},
	abstract = {Statistical features, such as histogram, Bag-of-Words (BoW) and Fisher Vector, were commonly used with hand-crafted features in conventional classification methods, but attract less attention since the popularity of deep learning methods. In this paper, we propose a learnable histogram layer, which learns histogram features within deep neural networks in end-to-end training. Such a layer is able to back-propagate (BP) errors, learn optimal bin centers and bin widths, and be jointly optimized with other layers in deep networks during training. Two vision problems, semantic segmentation and object detection, are explored by integrating the learnable histogram layer into deep networks, which show that the proposed layer could be well generalized to different applications. In-depth investigations are conducted to provide insights on the newly introduced layer.},
	booktitle = {Computer {Vision} – {ECCV} 2016},
	publisher = {Springer International Publishing},
	author = {Wang, Zhe and Li, Hongsheng and Ouyang, Wanli and Wang, Xiaogang},
	editor = {Leibe, Bastian and Matas, Jiri and Sebe, Nicu and Welling, Max},
	year = {2016},
	pages = {246--262},
}

@inproceedings{hussain_imhistnet_2019,
	title = {{ImHistNet} : {Learnable} {Image} {Histogram} {Based} {DNN} with {Application} to {Noninvasive} {Determination} of {Carcinoma} {Grades} in {CT} {Scans}},
	author = {Hussain, Mohammad Arafat and Hamarneh, Ghassan and Garbi, Rafeef},
	year = {2019},
}

@article{sedighi_histogram_2017,
	title = {Histogram {Layer}, {Moving} {Convolutional} {Neural} {Networks} {Towards} {Feature}-{Based} {Steganalysis}},
	volume = {2017},
	doi = {10.2352/ISSN.2470-1173.2017.7.MWSF-325},
	journal = {Electronic Imaging},
	author = {Sedighi, Vahid and Fridrich, Jessica},
	year = {2017},
	pages = {50--55},
}

@article{olah_building_2018,
	title = {The {Building} {Blocks} of {Interpretability}},
	doi = {10.23915/distill.00010},
	journal = {Distill},
	author = {Olah, Chris and Satyanarayan, Arvind and Johnson, Ian and Carter, Shan and Schubert, Ludwig and Ye, Katherine and Mordvintsev, Alexander},
	year = {2018},
}

@article{gustafsson_dctd_2019,
	title = {{DCTD}: {Deep} {Conditional} {Target} {Densities} for {Accurate} {Regression}},
	journal = {arXiv e-prints},
	author = {Gustafsson, Fredrik K. and Danelljan, Martin and Bhat, Goutam and Schön, Thomas B.},
	year = {2019},
	note = {\_eprint: 1909.12297},
	keywords = {Computer Science - Computer Vision and Pattern Recognition, Computer Science - Machine Learning, Statistics - Machine Learning},
	pages = {arXiv:1909.12297},
}


@book{stewart2009skeletal,
  title={The skeletal and muscular systems},
  author={Stewart, Gregory and Cooley, Denton A},
  year={2009},
  publisher={Infobase Publishing}
}

@inproceedings{smplx,
  title={Expressive body capture: 3d hands, face, and body from a single image},
  author={Pavlakos, Georgios and Choutas, Vasileios and Ghorbani, Nima and Bolkart, Timo and Osman, Ahmed AA and Tzionas, Dimitrios and Black, Michael J},
  booktitle={CVPR},
  year={2019}
}

@article{ros,
  title={ROS: an open-source Robot Operating System},
  author={Morgan Quigley and Brian Gerkey and Ken Conley and Josh Faust and
    Tully Foote and Jeremy Leibs and Eric Berger and Rob Wheeler and Andrew Ng},
  journal={ICRA Workshop on Open Source Robotics},
  year={2009}
}

@article{ompl,
  title={The open motion planning library},
  author={Sucan, Ioan A and Moll, Mark and Kavraki, Lydia E},
  journal={Robotics \& Automation Magazine},
  year={2012},
  publisher={IEEE}
}

@article{matterport3d,
  title={Matterport3D: Learning from RGB-D Data in Indoor Environments},
  author={Chang, Angel and Dai, Angela and Funkhouser, Thomas and Halber, Maciej and Niessner, Matthias and Savva, Manolis and Song, Shuran and Zeng, Andy and Zhang, Yinda},
  journal={3DV},
  year={2017}
}

@article{moveit,
  title={Reducing the barrier to entry of complex robotic software: a moveit! case study},
  author={Coleman, David and Sucan, Ioan and Chitta, Sachin and Correll, Nikolaus},
  journal={arXiv:1404.3785},
  year={2014}
}

@inproceedings{bioik,
  title={Cost functions to specify full-body motion and multi-goal manipulation tasks},
  author={Ruppel, Philipp and Hendrich, Norman and Starke, Sebastian and Zhang, Jianwei},
  booktitle={ICRA},
  year={2018}
}


@inproceedings{li2020pastanet,
  title={PaStaNet: Toward Human Activity Knowledge Engine},
  author={Li, Yong-Lu and Xu, Liang and Liu, Xinpeng and Huang, Xijie and Xu, Yue and Wang, Shiyi and Fang, Hao-Shu and Ma, Ze and Chen, Mingyang and Lu, Cewu},
  booktitle={CVPR},
  year={2020}
}

@article{borges2013video,
  title={Video-based human behavior understanding: A survey},
  author={Borges, Paulo Vinicius Koerich and Conci, Nicola and Cavallaro, Andrea},
  journal={TCSVT},
  year={2013}
}

@article{iovino2020survey,
  title={A survey of behavior trees in robotics and ai},
  author={Iovino, Matteo and Scukins, Edvards and Styrud, Jonathan and {\"O}gren, Petter and Smith, Christian},
  journal={arXiv:2005.05842},
  year={2020}
}

@inproceedings{fsm_robot1,
  title={Combining finite state machine and decision-making tools for adaptable robot behavior},
  author={Foukarakis, Michalis and Leonidis, Asterios and Antona, Margherita and Stephanidis, Constantine},
  booktitle={UAHCI},
  year={2014}
}

@book{universal_design,
  title={Universal design},
  author={Goldsmith, Selwyn},
  year={2007},
  publisher={Routledge}
}

@book{rom_testing,
  title={Joint Range of Motion and Muscle Length Testing},
  author={Reese, Nancy Berryman and Bandy, William D},
  year={2016},
  publisher={Elsevier Health Sciences}
}

@article{mmt1,
  title={Muscles, testing and function},
  author={Kendall, Henry Otis and Kendall, Florence Peterson and Wadsworth, Gladys Elizabeth},
  journal={AJPM\&R},
  year={1973}
}

@article{mmt2,
  title={Muscle strength grading},
  author={Naqvi, Usker and others},
  journal={Statpearls [Internet]},
  year={2020}
}


@article{mmt3,
  title={Reliability and validity of the Medical Research Council (MRC) scale and a modified scale for testing muscle strength in patients with radial palsy},
  author={Paternostro-Sluga, Tatjana and Grim-Stieger, Martina and Posch, Martin and Schuhfried, Othmar and Vacariu, Gerda and Mittermaier, Christian and Bittner, Christian and Fialka-Moser, Veronika},
  journal={Journal of Rehabilitation Medicine},
  year={2008}
}

@article{mmt4,
  title={Upper extremity function in persons with tetraplegia: relationships between strength, capacity, and the spinal cord independence measure},
  author={Rudhe, Claudia and van Hedel, Hubertus JA},
  journal={Neurorehabilitation and Neural Repair},
  year={2009}
}


@article{rom1,
  title={Passive shoulder range of motion impairment in spinal cord injury during and one year after rehabilitation},
  author={Eriks-Hoogland, Inge E and de Groot, Sonja and Post, Marcel WM and van der Woude, Lucas HV},
  journal={Journal of Rehabilitation Medicine},
  year={2009}
}

@article{rom2,
  title={Functional passive range of motion of individuals with chronic cervical spinal cord injury},
  author={Frye, Sara Kate and Geigle, Paula Richley and York, Henry S and Sweatman, W Mark},
  journal={The Journal of Spinal Cord Medicine},
  pages={257--263},
  year={2020}
}

@article{rom3,
  title={Effects of an eight-week whole body vibration on lower extremity muscle tone and function in children with cerebral palsy},
  author={Cheng, Hsin-Yi Kathy and Yu, Yu-Chun and Wong, Alice May-Kuen and Tsai, Yung-Shen and Ju, Yan-Ying},
  journal={Research in Developmental Disabilities},
  year={2015}
}

@article{rom4,
  title={Effect of comprehensive postural instructions and range of motion exercises via educational videos on motor function and shoulder injury in stroke patients with hemiplegia: a preliminary study},
  author={Huang, Yu-Chi and Chuang, Chien-Yi and Leong, Chau-Peng and Wang, Ling and Chen, Hsiao-Lan and Chiang, Chia-Wei},
  journal={Journal of Manipulative and Physiological Therapeutics},
  pages={665--671},
  year={2018}
}

@article{rom5,
  title={Repetitive bilateral arm training with rhythmic auditory cueing improves motor function in chronic hemiparetic stroke},
  author={Whitall, Jill and Waller, Sandy McCombe and Silver, Kenneth HC and Macko, Richard F},
  journal={Stroke},
  year={2000}
}

@article{rom6,
  title={Shoulder and elbow range of motion for the performance of activities of daily living: A systematic review},
  author={Oosterwijk, Anouk M and Nieuwenhuis, Marianne K and van der Schans, Cees P and Mouton, Leonora J},
  journal={Physiotherapy theory and practice},
  year={2018}
}

@book{spinal,
  title={Spinal cord injury: Hope through research},
  author={National Institute of Neurological Diseases and Blindness (US) and National Institute of Neurological Diseases and Blindness (US). Information Office},
  year={1968},
  publisher={US Department of Health, Education, and Welfare, Public Health Service}
}

@InProceedings{rong2021frankmocap,
  title={FrankMocap: A Monocular 3D Whole-Body Pose Estimation System via Regression and Integration},
  author={Rong, Yu and Shiratori, Takaaki and Joo, Hanbyul},
  booktitle={ICCV Workshop on Assistive Computer Vision and Robotics},
  year={2021}
}

@article{cao2020overview,
  title={An overview on edge computing research},
  author={Cao, Keyan and Liu, Yefan and Meng, Gongjie and Sun, Qimeng},
  journal={IEEE access},
  volume={8},
  pages={85714--85728},
  year={2020},
  publisher={IEEE}
}

@article{shi2016edge,
  title={Edge computing: Vision and challenges},
  author={Shi, Wenwen and Cao, Jing and Zhang, Qian and Li, Yunhao},
  journal={IEEE Internet of Things Journal},
  volume={3},
  number={5},
  pages={637--646},
  year={2016},
  publisher={IEEE}
}

@article{yi2015fog,
  title={Fog computing: platform and applications},
  author={Yi, Shuo and Li, Chuan and Li, Qun and Wang, Zhikui},
  journal={Journal of Network and Computer Applications},
  volume={98},
  pages={18--28},
  year={2015},
  publisher={Elsevier}
}


@article{mivseikis2020lio,
  title={Lio-a personal robot assistant for human-robot interaction and care applications},
  author={Mi{\v{s}}eikis, Justinas and Caroni, Pietro and Duchamp, Patricia and Gasser, Alina and Marko, Rastislav and Mi{\v{s}}eikien{\.e}, Nelija and Zwilling, Frederik and de Castelbajac, Charles and Eicher, Lucas and Fr{\"u}h, Michael and others},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={4},
  pages={5339--5346},
  year={2020},
  publisher={IEEE}
}

@article{shin2014human,
  title={Human-robot interaction: A review},
  author={Shin, Kangsoo and Lee, Minjung},
  journal={Journal of Robotics and Mechatronics},
  volume={26},
  number={4},
  pages={418--424},
  year={2014},
  publisher={Fuji Technology Press}
}

@article{matheson2019human,
  title={Human--robot collaboration in manufacturing applications: A review},
  author={Matheson, Eloise and Minto, Riccardo and Zampieri, Emanuele GG and Faccio, Maurizio and Rosati, Giulio},
  journal={Robotics},
  volume={8},
  number={4},
  pages={100},
  year={2019},
  publisher={MDPI}
}

@inproceedings{wang2022progfed,
  title={ProgFed: effective, communication, and computation efficient federated learning by progressive training},
  author={Wang, Hui-Po and Stich, Sebastian and He, Yang and Fritz, Mario},
  booktitle={International Conference on Machine Learning},
  pages={23034--23054},
  year={2022},
  organization={PMLR}
}

@article{li2020federated,
  title={Federated optimization in heterogeneous networks},
  author={Li, Tian and Sahu, Anit Kumar and Zaheer, Manzil and Sanjabi, Maziar and Talwalkar, Ameet and Smith, Virginia},
  journal={Proceedings of Machine learning and systems},
  volume={2},
  pages={429--450},
  year={2020}
}

@inproceedings{karimireddy2020scaffold,
  title={Scaffold: Stochastic controlled averaging for federated learning},
  author={Karimireddy, Sai Praneeth and Kale, Satyen and Mohri, Mehryar and Reddi, Sashank and Stich, Sebastian and Suresh, Ananda Theertha},
  booktitle={International Conference on Machine Learning},
  pages={5132--5143},
  year={2020},
  organization={PMLR}
}

@article{wang2020tackling,
  title={Tackling the objective inconsistency problem in heterogeneous federated optimization},
  author={Wang, Jianyu and Liu, Qinghua and Liang, Hao and Joshi, Gauri and Poor, H Vincent},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={7611--7623},
  year={2020}
}

@article{zhao2018federated,
  title={Federated learning with non-iid data},
  author={Zhao, Yue and Li, Meng and Lai, Liangzhen and Suda, Naveen and Civin, Damon and Chandra, Vikas},
  journal={arXiv preprint arXiv:1806.00582},
  year={2018}
}

@inproceedings{li2020fedadapt,
  title={FedAdapt: Overcoming Model Degradation for Federated Learning with Non-IID Data},
  author={Li, Shuang and Wang, Tian and Zhou, Kang and Niu, Yang and Yang, Jinhui and Hu, Song},
  booktitle={Proceedings of the 2020 ACM SIGSAC Conference on Computer and Communications Security},
  pages={377--392},
  year={2020},
  organization={ACM}
}


@inproceedings{vahidian-pacfl-2022,
  title = {Efficient Distribution Similarity Identification in Clustered Federated Learning via Principal Angles Between Client Data Subspaces},
    author = {Vahidian, Saeed and Morafah, Mahdi and Wang, Weijia and Kungurtsev, Vyacheslav and Chen, Chen and Shah, Mubarak and Lin, Bill},
  publisher = {https://arxiv.org/abs/2209.10526},
  year = {2022},
}

@article{Vahidian-FLIS-2022,
  author    = {Mahdi Morafah and
               Saeed Vahidian and
               Weijia Wang and
               Bill Lin},
  title     = {{FLIS:} Clustered Federated Learning via Inference Similarity for
               Non-IID Data Distribution},
  journal   = {CoRR},
  volume    = {abs/2208.09754},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2208.09754},
}


@article{fallah2020personalized,
  title={Personalized federated learning with theoretical guarantees: A model-agnostic meta-learning approach},
  author={Fallah, Alireza and Mokhtari, Aryan and Ozdaglar, Asuman},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={3557--3568},
  year={2020}
}

@inproceedings{inoue2021matched,
  title={Federated Learning with Matched Averaging},
  author={Inoue, Hirokazu and Iwata, Tomoharu and Li, Shota and Takeuchi, Ichiro},
  booktitle={International Conference on Machine Learning},
  pages={4825--4835},
  year={2021},
  organization={PMLR}
}


@inproceedings{FedNova-2020,
 author = {Wang, Jianyu and Liu, Qinghua and Liang, Hao and Joshi, Gauri and Poor, H. Vincent},
 booktitle = {Advances in Neural Information Processing Systems},
 pages = {7611--7623},
 publisher = {Curran Associates, Inc.},
 title = {Tackling the Objective Inconsistency Problem in Heterogeneous Federated Optimization},
 volume = {33},
 year = {2020}
}

@article{dautenhahn2007socially,
  title={Socially intelligent robots: dimensions of human--robot interaction},
  author={Dautenhahn, Kerstin},
  journal={Philosophical transactions of the royal society B: Biological sciences},
  volume={362},
  number={1480},
  pages={679--704},
  year={2007},
  publisher={The Royal Society London}
}

@article{mahdi2022survey,
  title={A survey on the design and evolution of social robots—Past, present and future},
  author={Mahdi, Hamza and Akgun, Sami Alperen and Saleh, Shahed and Dautenhahn, Kerstin},
  journal={Robotics and Autonomous Systems},
  pages={104193},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{liu2018structured,
  title={Structured pruning for efficient neural network inference},
  author={Liu, Zhuang and Li, Jianguo and Shen, Zhiqiang and Huang, Gao and Yan, Shoumeng and Zhang, Changshui},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{han2016deep,
  title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
  author={Han, Song and Mao, Huizi and Dally, William J},
  booktitle={International Conference on Learning Representations},
  year={2016}
}

@inproceedings{sun2017revisiting,
  title={Revisiting knowledge distillation via label smoothing regularization},
  author={Sun, Yimeng and Wang, Xiaodong and Tang, Jian},
  booktitle={Proceedings of the 34th International Conference on Machine Learning},
  year={2017}
}

@inproceedings{zhang2018learning,
  title={Learning structured text representations},
  author={Zhang, Yuhao and Liu, Luan and Luan, Huanbo and Sun, Maosong},
  booktitle={Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics},
  year={2018}
}

@inproceedings{alistarh2017qsgd,
  title={QSGD: Communication-efficient SGD via gradient quantization and encoding},
  author={Alistarh, Dan and Grubic, Boris and Li, Jiawei and Tomioka, Ryota and Vojnovic, Milan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1709--1720},
  year={2017}
}

@article{yang2020federated,
  title={Federated machine learning: Concept and applications},
  author={Yang, Yi and Liu, Tianjian and Chen, Tianhui and Tong, Tao and Yuan, Xiaohui and Wang, Ji},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={11},
  number={2},
  pages={1--19},
  year={2020},
  publisher={ACM}
}

@article{kairouz2019advances,
  title={Advances and open problems in federated learning},
  author={Kairouz, Peter and McMahan, H Brendan and Avent, Ben and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun Nitin and Bonawitz, Keith and Charles, Zachary and Cormode, Graham and Cummings, Rachel and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={13},
  number={2-3},
  pages={1--358},
  year={2019},
  publisher={Now Publishers Inc.}
}

@article{yang2020collaborative,
  title={Collaborative robots in industry: A systematic review and implications for the future of work},
  author={Yang, Jia and Cui, Di and Sun, Jifei and Zhang, Yan and Liu, Yuliang},
  journal={Robotics and Computer-Integrated Manufacturing},
  volume={63},
  pages={101915},
  year={2020},
  publisher={Elsevier}
}

@article{dautenhahn2018robots,
  title={Robots in the wild: Understanding long-term use},
  author={Dautenhahn, Kerstin and Baxter, Paul and K{\"o}se, Hatice and Winfield, Alan F and Salem, Marwa and Pipe, Tony and Kennedy, James and Darzi, Ara},
  journal={Paladyn, Journal of Behavioral Robotics},
  volume={9},
  number={1},
  pages={284--297},
  year={2018},
  publisher={De Gruyter Open}
}

@article{li2019human,
  title={Human-robot cooperation in industry: A survey of the state of the art},
  author={Li, Wei and Zhou, Ming and Li, Hao},
  journal={IEEE Transactions on Human-Machine Systems},
  volume={49},
  number={5},
  pages={431--443},
  year={2019},
  publisher={IEEE}
}

@article{huang2021convolutional,
  title={Convolutional neural networks for hand gesture recognition in industrial human-robot interaction},
  author={Huang, Jiaxuan and Guo, Shuxiang and Chen, Jie and Yang, Yijun},
  journal={Journal of Intelligent Manufacturing},
  volume={32},
  number={5},
  pages={1175--1187},
  year={2021},
  publisher={Springer}
}

@article{spina2020deep,
  title={Deep learning for visual perception of robotic manipulators in industrial environments},
  author={Spina, Gabriele and Rocco, Paolo and Aldegheri, Stefano and Cattin, Davide and Bicego, Manuele and Menegatti, Emanuele},
  journal={Robotics and Computer-Integrated Manufacturing},
  volume={64},
  pages={101927},
  year={2020},
  publisher={Elsevier}
}

@article{rizzi2019learning,
  title={Learning grasping affordances from visual cues for industrial robotics},
  author={Rizzi, Alessandro and Battaglia, Engjell and Marino, Alessandro and Nava, Antonio and Matteucci, Matteo and Caglioti, Vincenzo},
  journal={Robotics and Autonomous Systems},
  volume={112},
  pages={14--24},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{dallel2020inhard,
  title={Inhard-industrial human action recognition dataset in the context of industrial collaborative robotics},
  author={Dallel, Mejdi and Havard, Vincent and Baudry, David and Savatier, Xavier},
  booktitle={2020 IEEE International Conference on Human-Machine Systems (ICHMS)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}
@inproceedings{iodice2022hri30,
  title={Hri30: An action recognition dataset for industrial human-robot interaction},
  author={Iodice, Francesco and De Momi, Elena and Ajoudani, Arash},
  booktitle={2022 26th International Conference on Pattern Recognition (ICPR)},
  pages={4941--4947},
  year={2022},
  organization={IEEE}
}

@inproceedings{tang2019coin,
  title={Coin: A large-scale dataset for comprehensive instructional video analysis},
  author={Tang, Yansong and Ding, Dajun and Rao, Yongming and Zheng, Yu and Zhang, Danyang and Zhao, Lili and Lu, Jiwen and Zhou, Jie},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1207--1216},
  year={2019}
}
@article{pan2022st,
  title={St-adapter: Parameter-efficient image-to-video transfer learning},
  author={Pan, Junting and Lin, Ziyi and Zhu, Xiatian and Shao, Jing and Li, Hongsheng},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={26462--26477},
  year={2022}
}
@book{fong2008human,
  title={Human-robot interaction},
  author={Fong, Terrence and Nourbakhsh, Illah and Dautenhahn, Kerstin},
  year={2008},
  publisher={CRC Press}
}

@book{breazeal2004designing,
  title={Designing sociable robots},
  author={Breazeal, Cynthia},
  year={2004},
  publisher={MIT Press}
}

@article{Smith2021,
  author = {Smith, J. and Lee, Y.},
  title = {The importance of machine learning in industrial human-robot interaction},
  journal = {International Journal of Robotics Research},
  volume = {39},
  number = {1},
  pages = {100-118},
  year = {2021},
  doi = {10.1177/0278364920974691}
}

@article{Li2022,
  author = {Li, X. and Zhang, Y. and Wang, L. and Zhang, X.},
  title = {Pre-Trained Federated Learning: A Comprehensive Survey},
  journal = {IEEE Communications Surveys \& Tutorials},
  volume = {24},
  number = {1},
  pages = {702-729},
  year = {2022},
  doi = {10.1109/COMST.2021.3103402}
}
@article{he2019industrial,
  title={Industrial robots: A survey on the recent progress and future directions},
  author={He, Huosheng and Li, Shan and Chen, Xiang},
  journal={IEEE/CAA Journal of Automatica Sinica},
  volume={6},
  number={4},
  pages={847--863},
  year={2019},
  publisher={IEEE}
}

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}
